LUK: Empowering Log Understanding with Expert Knowledge from Large Language Models

Logs play a critical role in providing essential information for system monitoring and troubleshooting. Recently, with the success of pre-trained language models (PLMs) and large language models (LLMs) in natural language processing (NLP), smaller PLMs (such as BERT) and LLMs (like GPT-4) have become the current mainstream approaches for log analysis. Despite the remarkable capabilities of LLMs, their higher cost and inefficient inference present significant challenges in leveraging the full potential of LLMs to analyze logs. In contrast, smaller PLMs can be fine-tuned for specific tasks even with limited computational resources, making them more practical. However, these smaller PLMs face challenges in understanding logs comprehensively due to their limited expert knowledge. To address the lack of expert knowledge and enhance log understanding for smaller PLMs, this paper introduces a novel and practical knowledge enhancement framework, called LUK, which acquires expert knowledge from LLMs automatically and then enhances the smaller PLM for log analysis with these expert knowledge. LUK can take full advantage of both types of models. Specifically, we design a multi-expert collaboration framework based on LLMs with different roles to acquire expert knowledge. In addition, we propose two novel pre-training tasks to enhance the log pre-training with expert knowledge. LUK achieves state-of-the-art results on different log analysis tasks and extensive experiments demonstrate expert knowledge from LLMs can be utilized more effectively to understand logs. Our source code and detailed experimental data are available at https://github.com/LeaperOvO/LUK.

==> response/review0.tex <==
\section{Response to Associate Editor}

\subsection{Original Comments}
The reviewers have recognized the contribution of the proposed knowledge enhancement framework to the SE field. However, the following issues highlighted by the reviewers affected the acceptance of the paper:

1. The authors need to clarify the relationship between the current submission and the previously published paper "KnowLog: Knowledge Enhanced Pre-trained Language Model for Log Understanding" at ICSE 2024. Is the current submission an extension of the prior work? (Emphasized by Reviewers A \& C)

2. The evaluation should encompass a more comprehensive range of baselines for comparison: (1) Language Models directly applied to log understanding; (2) Knowledge distillation; (3) GPT-4 or GPT-4o. (Raised by all three reviewers)

3. The authors have not adequately explained why "LLMs cannot be directly applied to log understanding." (Noted by all three reviewers)

4. The rigor of the approach description in the paper requires improvement. (Pointed out by all three reviewers)
It is advisable for the authors to consider the constructive comments from the three reviewers and further refine their approach to address these issues.

\subsection{Comments and Responses}

\textbf{Response:} Thanks for your valuable feedback on our paper.  We have carefully considered and addressed the list of must-fix issues. We also have addressed the reviewers' other comments and suggestions in the previous response. The manuscript has been revised thoroughly according to the reviewers' advice.

\textbf{C1:} The authors need to clarify the relationship between the current submission and the previously published paper "KnowLog: Knowledge Enhanced Pre-trained Language Model for Log Understanding" at ICSE 2024. Is the current submission an extension of the prior work? 

\textbf{R1:} Thanks for your reminder. LUK is a completely new approach, not an extension of KnowLog. 
First, LUK focuses on the challenge of the high cost and inefficiency of reasoning for Large Language Models (LLMs). It introduces a novel framework that reduces the computational overhead of LLMs by distilling knowledge into smaller models, enhancing practicality in log analysis contexts. In contrast, KnowLog's primary emphasis lies in leveraging existing domain knowledge to enhance log understanding.

Second, LUK has an advantage over KnowLog in terms of knowledge acquisition. KnowLog enhances the model based on existing documentation knowledge, however, most logs lack documentation, and the cost of manually constructing knowledge is extremely high, KnowLog cannot work in the absence of documentation. LUK, on the other hand, does not need to rely on existing documentation and obtains sufficient knowledge through the LLM, which is even of higher quality than the documentation knowledge, thus making LUK more practical. 

Third, LUK proposes a new pre-training task from the word level. KnowLog's abbreviation prediction task only recognizes the abbreviations that are already in the log. It cannot understand other key information within the log's tokens (such as parameters) and cannot perceive useful information from external knowledge to enhance the understanding of domain tokens. And LUK can adaptively perceive useful knowledge to understand tokens in logs, not limited to abbreviations. 

Finally, experimentally, we take KnowLog as the baseline in this revised manuscript, experimental results verify the LUK's superiority over KnowLog. Our experiments and case studies demonstrate that LUK consistently outperforms KnowLog across various metrics, substantiating the efficacy and advancement of our proposed approach.

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{new_fig/luk_knowledge_case.pdf}
   % \vspace{-6mm}
   \caption{\textcolor{blue}{Example of knowledge generated by GPT-4o and retrieved from documentation.}}
   % \vspace{-4mm}
   \label{fig:knowledge_case-r0}
\end{figure*}

\begin{figure}[]
\centering
    % \vspace{-2mm}
    \includegraphics[width=\columnwidth]{new_fig/LUK_percentage_1.pdf}    
    
    \caption{\textcolor{blue}{Proportion of unsatisfactory knowledge, where we employ the evaluation criteria of the MEC framework to evaluate the knowledge.}}
    
    % \vspace{-5mm}
    \label{fig:doc-knowledge-analysis-r0}
\end{figure}

\uline{Our main revisions are as follows:}
\begin{enumerate}
    \item We emphasize the focus of this paper in the introduction: \\ \uline{\textbf{Section I, Page 1-2:}} \textcolor{blue}{Despite the powerful performance of LLMs, limited accessibility
and higher costs present significant challenges in
leveraging the full potential of LLMs. These LLMs often
come with substantial usage fees and have restricted access
to data privacy and security. Even if the LLM is deployed
locally, it still may face resource constraints, making LLMs
less attainable for individuals and smaller organizations. In
addition, due to their complex autoregressive architectures
and a large number of parameters, LLM-based methods are computationally inefficient. Considering that modern software
systems can produce several petabytes per day [34, 35],
directly employing LLMs for log analysis is impractical due to
the significant overhead of querying LLMs, such as inference
time and network latency [29, 36]. In contrast, smaller PLMs
with smaller parameters, requiring limited resource costs,
are more efficient than LLMs [37]. Hence, we argue that
the smaller PLM is more practical in extensive log analysis
scenarios [23, 24, 25].}
    \item We modify the introduction of KnowLog in \textbf{Section I, Page 2:} \\
    \uline{\textbf{Section I, Page 2:}} \textcolor{blue}{This issue can be
attributed to the lack of rich sources for knowledge acquisition.
Although KnowLog proposes to acquire expert knowledge
from documentation [22], most logs lack professional documentation
(e.g. almost unable to find relevant documents for
logs coming from Loghub [38]) and the manual construction of
knowledge is costly and inefficient, which significantly hinders
the availability of the model.} \\
    \uline{\textbf{Section I, Page 2:}} \textcolor{blue}{In addition, KnowLog proposes an abbreviation
prediction task specialized for log understanding. However, its
ability only to enhance the knowledge of abbreviations in the
logs is limited. It cannot adaptively perceive other important
information from the knowledge to understand logs, such as
the parameter knowledge of logs.}
    \item We add KnowLog as the baseline in our experiments. \\
    \uline{\textbf{Section IV.D.2), Page 10:}} 
    \textcolor{blue}{In addition, KnowLog is the state-of-the-art log pre-trained model in log analysis not only due to pre-training on log corpus but also enhancing the pre-training with documentation knowledge. Referring to KnowLog, we collect the descriptions of logs from the Huawei and Cisco public documentation as background knowledge to enhance the log pre-training in the same way. For fairness, we reproduce Biglog and KnowLog with the same pre-training setting on our log corpus.} 
    \item We add the analysis of the experiments about KnowLog in \textbf{Section IV.E, Page 11-14:} \\
    \uline{\textbf{Section IV.E.RQ1, Page 11:}} \textcolor{blue}{To verify the effectiveness of the expert knowledge obtained
from the LLM, we compare it with the KnowLog, whose
knowledge is obtained from the documentation. Our experimental
findings demonstrate that MEC-based LUK surpasses
KnowLog in performance, more specifically, LUK (MECGPT4o)
improves the average Accuracy on the Cisco and
Huawei datasets regarding the MC and LDSM tasks by 2.38\%
and 1.15\%, respectively. It is noteworthy that Huawei’s documentation
provides more detailed log descriptions compared
to the relatively concise descriptions found in Cisco’s documentation.
This disparity underscores the LLM’s capability
to generate domain knowledge of equal or superior quality to that found in high-quality documentation. Given the scarcity of
documented descriptions for most logs in practice, obtaining
expert knowledge through KnowLog becomes impractical. For
instance, the challenge of sourcing relevant documents for
logs from sources like Loghub [38] significantly hampers
the effectiveness of KnowLog. Our approach, which operates
independently of documentation, consistently yields superior
results, and serves to diminish the reliance on human experts
for intricate knowledge construction processes, offering a more
feasible and practical alternative to traditional documentation-based
methodologies.} \\
    \uline{\textbf{Section IV.E.RQ2, Page 12:}} \textcolor{blue}{
    In comparison to KnowLog, LUK still has a clear advantage
over KnowLog, which takes knowledge from the documentation.
The domain knowledge derived from LLMs offers a deeper
level of comprehension and learning, enabling the PLM to
generalize more effectively to new log datasets. Conversely,
KnowLog, constrained by information within documents, may
not provide sufficiently profound domain insights to support
robust generalization of the PLM to unseen data.} \\
    \uline{\textbf{Section IV.E.RQ3, Page 13:}} \textcolor{blue}{In contrast, KnowLog’s reliance on knowledge
solely extracted from documentation may lead to limitations
in handling the evolving nature of log data.} \\
    \uline{\textbf{Section IV.E.RQ4, Page 14:}} \textcolor{blue}{KnowLog primarily relies on
knowledge extracted from documentation, which may be limited
in scope and quality, especially in low-resource settings.
In contrast, this proves that knowledge acquired by the LLM
has a wider scope and can provide a more comprehensive
and diverse range of information, rather than being limited to
some specific documentation.}
    \item To further verify our proposed word-level Token Prediction (TP) task,
we also compare it with other word-level pre-training tasks \textcolor{red}{Table \ref{tab:ablation-r0}},
including BERT’s Masked Language Modeling (MLM) task
and KnowLog’s Abbreviation Prediction (AP) task. \\
    \uline{\textbf{Section IV.F, Page 14:}} \textcolor{blue}{
    To further verify our proposed word-level Token Prediction (TP) task,
we also compare it with other word-level pre-training tasks,
including BERT’s Masked Language Modeling (MLM) task
and KnowLog’s Abbreviation Prediction (AP) task. The results
demonstrate the superior capability of our token prediction
task in integrating domain knowledge effectively. Unlike MLM
and Abbreviation Prediction tasks, our proposed pre-training
task requires models to not only predict tokens within the
log itself but also dynamically assimilate contextual insights
from domain-specific knowledge using the knowledge perception
module. This distinctive aspect sets our approach apart,
as BERT solely relies on internal information and cannot
leverage external knowledge. Conversely, KnowLog is limited
in its scope, focusing solely on abbreviations and failing to
comprehend other critical log elements such as parameters,
conditions, and more, which are essential for a comprehensive
understanding of domain-specific terminology.}
    \item We add the case study to analyze the quality of the expert knowledge from different sources in \textbf{Section V.B.2), Page 17:} \\
    \uline{\textbf{Section V.B.2), Page 17:}} \textcolor{blue}{Evaluation and refinement mechanism of the MEC
framework: To further intuitively analyze the quality of the expert knowledge constructed with the MEC framework, we compare it with the knowledge collected from documentation and the COT-based approach. As shown in \textcolor{red}{Fig. \ref{fig:knowledge_case-r0}}, we collect a Cisco log as the case and give the corresponding generated knowledge based on the COT and MEC methods.} \\
    \textcolor{blue}{
As can be seen from these cases, the knowledge provided by the documentation is too simple, which provides a generic and limited understanding of the log without delving into specific details or potential causes. Although COT-based knowledge offers a more detailed explanation of the log, compared to MEC-based knowledge, there is still the problem of inadequate knowledge and lack of insight.
In contrast, the knowledge derived from the MEC framework excels in its comprehensive analysis and insights. By explicitly outlining the specifics of the log error, including the MTS queue failure and the placeholders for queue and error message, the MEC-based knowledge provides a deeper understanding of the issue at hand. Furthermore, it goes beyond mere description to identify potential root causes such as network connectivity issues.
The comparison highlights the clear advantage of the MEC framework in expert knowledge generation. Its collaborative nature allows for the integration of diverse expertise and perspectives, resulting in a more comprehensive analysis of complex logs.} \\ 
\textcolor{blue}{
To quantify the differences among the various forms of knowledge, we employ the evaluation criteria of the MEC framework to evaluate the knowledge acquired by the documentation and the knowledge constructed based on COT in the network device logs. The evaluation results are shown in \textcolor{red}{Fig. \ref{fig:doc-knowledge-analysis-r0}}, revealing a notable contrast in quality between the different sources of knowledge. It is apparent from the analysis that a significant proportion of knowledge sourced from documentation falls short of meeting the evaluation requirements. This deficiency can be attributed to the inherent limitations of documentation-derived knowledge, which often lacks depth and detail, offering only the most straightforward description of the logs. Combined with Fig. 10a, this suggests that the knowledge acquired from MEC based on LLMs is comparable or even better than the documentation. Considering the lack of documentation support for most logs and the high cost of manually constructing knowledge, this provides a feasible way to gain a wealth of practical knowledge automatically.}

\end{enumerate}

\begin{table}[]
\centering
\color{blue}
\caption{\textcolor{blue}{Ablation studies for LUK, where TP and SA represent the pre-training tasks Token Prediction, and Semantic Alignment for LUK, respectively. MLM represents the pre-training task Masked Language Modeling of BERT and AP represents the pre-training task Abbreviation Prediction of KnowLog.}}
\label{tab:ablation-r0}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|cc}
\toprule[1.5pt]
\multirow{3}{*}{Methods}         & \multicolumn{2}{c|}{MC (Accuracy / Weighted-F1)} & \multicolumn{2}{c}{LDSM (Accuracy / Weighted-F1)} \\ \cmidrule{2-5} 
                                 & \multicolumn{2}{c|}{Huawei}                      & \multicolumn{2}{c}{Huawei}                        \\
                                 & Switches                & Routers                & Switches                & Routers                 \\ \midrule
BERT                             & 82.37 / 81.20           & 81.18 / 79.20          & 93.18 / 93.18           & 90.06 / 90.05           \\
LUK (MEC-GPT4o)                  & \textbf{85.51} / \textbf{85.26}           & \textbf{85.33} / \textbf{84.73}          & \textbf{97.66} / \textbf{97.66}           & \textbf{97.34} / \textbf{97.34}           \\ \midrule
$\vdash$ w/o Evaluator           & 83.77 / 83.26           & 82.30 / 81.08          & 96.57 / 96.57           & 95.53 / 95.53           \\
$\vdash$ w/o Evaluation Examples & 84.38 / 84.17           & 82.13 / 81.06          & 96.64 / 96.64           & 95.63 / 95.63           \\ \midrule
$\vdash$ w/o TP                  & 83.25 / 82.65           & 81.66 / 79.92          & 95.95 / 95.95           & 95.68 / 95.68           \\
$\vdash$ w/o SA                  & 83.77 / 83.19           & 84.14 / 82.92          & 95.25 / 95.25           & 94.68 / 94.68           \\ \midrule
$\vdash$ only with MLM           & 83.24 / 83.25           & 82.36 / 81.19          & 94.19 / 94.19           & 93.62 / 93.61           \\
$\vdash$ only with AP            & 83.60 / 82.89           & 82.72 / 81.68          & 94.39 / 94.39           & 93.97 / 93.97           \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\textbf{C2:} The evaluation should encompass a more comprehensive range of baselines for comparison: (1) Language Models directly applied to log understanding; (2) Knowledge distillation; (3) GPT-4 or GPT-4o. 

\textbf{R2:} Many thanks for your suggestions. As shown in \textcolor{red}{Table \ref{tab: software_results-r0} and \ref{tab: network_result2-r0}}, we have taken all three methods as the baselines in this revised manuscript.  First, we add three different LLMs as baselines, which
follow the in-context learning paradigm. Specifically,
we select top-5 similar examples from the training set
for each input log and use \textit{bge-large-en-v1.5} as the
embedding model to select examples. Considering the
recency bias of LLMs \cite{zhao2021calibrate}, we arrange these examples in
ascending order based on the cosine similarity.

Second, we add the existing distillation technique as
the baseline in the experiments. Specifically, we select Chain-of-Thought (COT)-based knowledge distillation \cite{hsieh2023distilling,shridhar2023distilling} as the baseline, which has
proven to be an effective knowledge distillation method
for the reasoning process in the field of NLP. The results
show that our framework is more advantageous.

Third, we employ the more powerful LLM (GPT-4o) as the
backbone to build the MEC framework in our experiments.


\begin{table}[]
\color{blue}
\centering
\caption{Results on AD and FI (software system logs).}
\label{tab: software_results-r0}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc|c}
\toprule[1.5pt]
\multirow{2}{*}{Methods} & AD (Precision / Recall / F1) & FI (Recall@1 / 2 / 3)                     \\
                         & BGL                          & OpenStack                                 \\ \midrule
CNN                      & \textbf{99.95} / 96.06 / 97.97        & 83.75 / 86.25 / 90.00                     \\
BiLSTM                   & \textbf{99.95} / 97.25 / 98.58        & 87.50 / 92.50 / 96.25                     \\
BERT                     & 99.70 / 98.48 / 99.09        & 87.50 / 92.50 / \textbf{98.75}                     \\
Biglog                   & 99.87 / 99.63 / 99.75        & 90.00 / 95.00 / \textbf{98.75}                     \\
KnowLog                  & 99.58 / 98.69 / 99.13        & 82.50 / 92.50 / 96.25                     \\ \midrule
T5-KD                    & 99.87 / 99.56 / 99.91        & 86.25 / 92.50 / 98.75                     \\ \midrule
LLama3-70B               & 46.87 / 95.23 / 71.05        & 85.00 / \textbf{96.25} / 96.25                     \\
ChatGPT                  & 42.73 / 95.23 / 68.98        & 83.75 / 95.00 / 96.25                     \\
GPT-4o                   & 46.85 / 95. 23 / 70.54       & 87.50 / \textbf{96.25} / 96.25                     \\ \midrule
LUK (COT-ChatGPT)        & 99.95 / 99.87 / 99.91        & 91.25 / 95.00 / \textbf{98.75}                     \\
LUK (COT-GPT4o)          & 99.67 / \textbf{100.0} / 99.83        & 91.25 / 95.00 / \textbf{98.75}                     \\ \midrule
LUK (MEC-LLama3)         & 99.87 / \textbf{100.0} / \textbf{99.93}        & \multicolumn{1}{l}{\textbf{92.50} / 95.00 / \textbf{98.75}} \\
LUK (MEC-ChatGPT)        & 99.95 / 99.91 / 99.93        & \multicolumn{1}{l}{\textbf{92.50} / 95.00 / \textbf{98.75}} \\
LUK (MEC-GPT4o)          & 99.87 / \textbf{100.0} / \textbf{99.93}       & \multicolumn{1}{l}{\textbf{92.50} / \textbf{96.25} / 96.25} \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\begin{table*}[]
\color{blue}
\centering
\caption{Results on MC and LDSM (network device logs).}
\label{tab: network_result-r0}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc|cccc}
\toprule[1.5pt]
\multirow{3}{*}{Methods} & \multicolumn{4}{c|}{MC (Accuracy / Weighted F1)}                                   & \multicolumn{4}{c}{LDSM (Accuracy / Weighted F1)}                                  \\ \cmidrule{2-9} 
                         & \multicolumn{2}{c|}{Cisco}                         & \multicolumn{2}{c|}{Huawei}   & \multicolumn{2}{c|}{Cisco}                         & \multicolumn{2}{c}{Huawei}    \\
                         & Switches      & \multicolumn{1}{c|}{Routers}       & Switches      & Routers       & Switches      & \multicolumn{1}{c|}{Routers}       & Switches      & Routers       \\ \midrule
CNN                      & 56.89 / 56.85 & \multicolumn{1}{c|}{57.46 / 54.92} & 74.52 / 73.95 & 72.78 / 72.23 & 84.04 / 84.04 & \multicolumn{1}{c|}{80.99 / 80.99} & 86.05 / 86.05 & 82.37 / 82.30 \\
BiLSTM                   & 55.74 / 55.63 & \multicolumn{1}{c|}{57.17 / 56.76} & 76.52 / 75.49 & 73.96 / 73.30 & 89.45 / 89.44 & \multicolumn{1}{c|}{85.42 / 85.41} & 87.85 / 87.85 & 84.43 / 84.40 \\
BERT                     & 62.67 / 61.38 & \multicolumn{1}{c|}{62.72 / 62.60} & 82.37 / 81.20 & 81.18 / 79.20 & 93.06 / 93.06 & \multicolumn{1}{c|}{90.01 / 90.00} & 93.18 / 93.18 & 90.06 / 90.05 \\
Biglog                   & 62.69 / 62.76 & \multicolumn{1}{c|}{63.15 / 61.17} & 83.24 / 83.25 & 82.36 / 81.19 & 93.32 / 93.32 & \multicolumn{1}{c|}{91.46 / 91.46} & 94.19 / 94.19 & 93.62 / 93.61 \\
KnowLog                  & 63.33 / 63.35 & \multicolumn{1}{c|}{63.65 / 63.12} & 84.11 / 83.65 & 83.55 / 82.41 & 95.05 / 95.05 & \multicolumn{1}{c|}{92.78 / 92.78} & 97.15 / 97.15 & 96.43 / 96.43 \\ \midrule
T5-KD                    & 62.96 / 62.36 & \multicolumn{1}{c|}{63.86 / 61.01} & 83.60 / 83.23 & 83.55 / 82.82 & 95.29 / 95.28 & \multicolumn{1}{c|}{93.20 / 93.20} & 95.25 / 95.25 & 93.97 / 93.97 \\ \midrule
LLama3-70B               & 61.61 / 60.95 & \multicolumn{1}{c|}{62.99 / 60.55} & 82.98 / 82.83 & 81.66 / 80.34 & 84.48 / 84.31 & \multicolumn{1}{c|}{88.32 / 88.24} & 95.49 / 95.49 & 95.57 / 95.57 \\
ChatGPT                  & 57.11 / 54.41 & \multicolumn{1}{c|}{57.99 / 54.56} & 79.14 / 77.19 & 78.22 / 75.51 & 82.14 / 81.96 & \multicolumn{1}{c|}{84.64 / 84.47} & 85.75 / 85.75 & 90.31 / 90.22 \\
GPT-4o                   & 62.12 / 61.62 & \multicolumn{1}{c|}{63.86 / 61.01} & 83.25 / 82.80 & 81.30 / 79.87 & 89.04 / 88.99 & \multicolumn{1}{c|}{93.12 / 93.11} & 97.23 / 97.23 & \textbf{97.79} / \textbf{97.79} \\ \midrule
LUK (COT-ChatGPT)        & 63.49 / 63.72 & \multicolumn{1}{c|}{64.51 / 63.33} & 83.42 / 82.70 & 83.19 / 82.34 & 94.93 / 94.92 & \multicolumn{1}{c|}{93.11 / 93.11} & 96.33 / 96.33 & 95.73 / 95.73 \\
LUK (COT-GPT4o)          & 63.47 / 63.51 & \multicolumn{1}{c|}{63.61 / 63.02} & 83.60 / 83.20 & 82.84 / 81.92 & 94.92 / 94.91 & \multicolumn{1}{c|}{93.18 / 93.18} & 96.46 / 96.46 & 95.93 / 95.93 \\ \midrule
LUK (MEC-LLama3)         & 65.67 / 65.27 & \multicolumn{1}{c|}{66.67 / 65.12} & 85.25 / 84.95 & 85.21 / 84.01 & 96.45 / 96.45 & \multicolumn{1}{c|}{94.13 / 94.13} & 97.66 / 97.66 & 97.39 / 97.39 \\
LUK (MEC-ChatGPT)        & 65.54 / 65.12 & \multicolumn{1}{c|}{66.29 / 64.27} & 84.64 / 84.47 & 85.09 / 83.82 & 96.32 / 96.32 & \multicolumn{1}{c|}{93.80 / 93.80} & 96.92 / 96.92 & 96.74 / 96.74 \\
LUK (MEC-GPT4o)          & \textbf{66.16} / \textbf{66.02} & \multicolumn{1}{c|}{\textbf{67.20} / \textbf{65.41}} & \textbf{85.51} / \textbf{85.26} & \textbf{85.33} / \textbf{84.73} & \textbf{96.63} / \textbf{96.63} & \multicolumn{1}{c|}{\textbf{94.32} / \textbf{94.32}} & \textbf{97.66} / \textbf{97.66} & 97.34 / 97.34 \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table*}


\begin{table}[]
\color{blue}
\centering
\caption{Results on LPCR and FPI (network device logs). Note: The results of proprietary LLMs on the FPI task cannot be compared due to data privacy issues.}
\label{tab: network_result2-r0}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|c}
\toprule[1.5pt]
\multirow{3}{*}{Methods} & \multicolumn{2}{c|}{LPCR (Precision@1 / 3 / MRR)} & FPI (Accuracy) \\ \cmidrule{2-4} 
                         & \multicolumn{2}{c|}{Huawei}                       & Huawei         \\
                         & Switches                & Routers                 & Switches       \\ \midrule
CNN                      & 54.30 / 77.26 / 67.99   & 53.45 / 75.77 / 67.35   & 69.00          \\
BiLSTM                   & 59.27 / 78.04 / 71.22   & 51.45 / 69.56 / 63.76   & 74.83          \\
BERT                     & 76.18 / 91.54 / 84.70   & 72.57 / 91.59 / 82.61   & 88.75          \\
Biglog                   & 83.33 / 94.02 / 89.38   & 82.98 / 95.59 / 89.49   & 89.58          \\
KnowLog                  & 87.50 / 93.01 / 91.84   & 89.68 / 96.59 / 93.99   & 94.17          \\ \midrule
T5-KD                    & 86.11 / 93.56 / 91.41   & 84.48 / 92.59 / 90.33   & -              \\ \midrule
LLama3-70B               & \textbf{95.61} / \textbf{98.04} / \textbf{97.27}   & \textbf{97.48} / \textbf{99.49} / \textbf{98.52}   & 88.83          \\
ChatGPT                  & 90.95 / 95.11 / 93.88   & 97.20 / 98.34 / 98.19   & -              \\
GPT-4o                   & 95.65 / 98.29 / 97.27   & 97.39 / 99.09 / 98.47   & -              \\ \midrule
LUK (COT-ChatGPT)        & 85.18 / 95.03 / 90.55   & 84.58 / 95.99 / 90.64   & 90.42          \\
LUK (COT-GPT4o)          & 86.34 / 93.79 / 91.37   & 87.88 / 95.19 / 92.75   & 92.50          \\ \midrule
LUK (MEC-LLama3)         & 90.45 / 95.81 / 94.06   & 90.49 / 96.99 / 94.52   & 95.83          \\
LUK (MEC-ChatGPT)        & 89.37 / 95.19 / 93.43   & 88.48 / 94.69 / 90.33   & 93.33          \\
LUK (MEC-GPT4o)          & 90.92 / 96.04 / 94.46   & 90.69 / 96.09 / 94.39   & \textbf{96.67}          \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\uline{Our main revisions are as follows:}
\begin{enumerate}
    \item We add the more powerful LLMs in our experiments and update all results in the revised manuscript. \\
    \uline{\textbf{Section IV.B, Page 7:}} \textcolor{blue}{As for expert knowledge acquisition, we explore different large language models for experiments, including two proprietary LLMs: \textit{gpt-3.5-turbo} (ChatGPT) and \textit{gpt-4o} (GPT-4o), and one open-source model: \textit{Llama-3.3-70B-Instruct } (LLama3-70B).} 

    \item We take the LLM following the ICL paradigm as the baseline. \\
    \uline{ \textbf{Section IV.D, Page 10:}} \textcolor{blue}{LLM-based log analysis methods follow the \textit{in-context learning} paradigm, where LLMs make predictions based on contexts augmented with a few examples without training.
Following previous LLM-based log analysis works [26,27,28,29], we select top-5 similar examples from the training set for each input log and use \textit{bge-large-en-v1.5} as the embedding model to select examples, due to its excellent performance among all open-source embedding models. Considering the recency bias of LLMs [87]{zhao2021calibrate}, we arrange these examples in ascending order based on the cosine similarity. We select two proprietary LLMs (\textbf{ChatGPT} and \textbf{GPT-4o}) and one powerful open-source LLM (\textbf{LLama3-70B [79]}) as baselines. We utilize HTTP requests to invoke the OpenAI APIs and interact with proprietary LLMs. For open-source LLM, we deploy \textit{Llama-3.3-70B-Instruct} in our environments to analyze logs.}

    \item  We add the existing distillation technique as
the baseline in the experiments. \\
\uline{\textbf{Section IV.D.3), Page 10:}} \textcolor{blue}{
    Knowledge distillation methods: In the era of LLMs,
data augmentation (DA) is the prevalent paradigm to achieve
knowledge distillation of LLMs, where it prompts the LLM to
generate more data tailored to train the student model in a targeted
skill or domain [85, 44]. This reasoning process-oriented
distillation method is more effective compared to obtaining
labels directly from the teacher model [45]. Considering the
lack of research on knowledge distillation in the field of log
analysis, we select Chain-of-Thought (COT)-based knowledge
distillation as the baseline, which has proven to be an effective
knowledge distillation method for the reasoning process in the
field of NLP [46, 47].} \\
    \textcolor{blue}{Specifically, we select T5 [86] (t5-base with 223M parameters) as the student model, and GPT-4o as the teacher model.
Given the specific log analysis task, we provide the inputs
and labels from the training set to the teacher model, then
utilize COT prompting to extract rationales from the teacher
model. Finally, the student model is trained with the inputs
and constructed rationales.}
\end{enumerate}

\textbf{C3:} The authors have not adequately explained why "LLMs cannot be directly applied to log understanding."

\textbf{R3:} We apologize for our non-rigorous discussions of the LLM. This paper's key motivation focuses on exploring the smaller PLM to analyze logs due to the challenge of employing LLMs. Following the ICL paradigm in our experiments, we find that LLMs obtain good performance in log analysis tasks. In fact, LLMs can be used for log analysis, there are just many challenges and smaller models are more practical.
    Hence, we reformulate the challenge of utilizing LLMs for log analysis as follows: 
    \textit{Despite the powerful performance of LLMs, limited accessibility and higher costs present significant challenges in
leveraging the full potential of LLMs. These LLMs often
come with substantial usage fees and have restricted access
to data privacy and security. Even if the LLM is deployed
locally, it still may face resource constraints, making LLMs
less attainable for individuals and smaller organizations. 
In addition, due to their complex autoregressive architectures
and a large number of parameters, LLM-based methods are computationally inefficient.
Hence, we argue that the smaller PLM is more practical in extensive log analysis 
scenarios. }

\uline{We modify the discussion of the challenge for employing LLMs in the introduction and related work. The details are illustrated below:}
\begin{enumerate}
    \item We modify the  discussion in the introduction (\textbf{Section I, Page 1-2:}) \\
    \uline{\textbf{Section I, Page 1-2:}} \textcolor{blue}{Despite the powerful performance of LLMs, limited accessibility and higher costs present significant challenges in
leveraging the full potential of LLMs. These LLMs often
come with substantial usage fees and have restricted access
to data privacy and security. Even if the LLM is deployed
locally, it still may face resource constraints, making LLMs
less attainable for individuals and smaller organizations. In
addition, due to their complex autoregressive architectures
and a large number of parameters, LLM-based methods are computationally inefficient. Considering that modern software
systems can produce several petabytes per day [34, 35],
directly employing LLMs for log analysis is impractical due to
the significant overhead of querying LLMs, such as inference
time and network latency [29, 36]. In contrast, smaller PLMs
with smaller parameters, requiring limited resource costs,
are more efficient than LLMs [37]. Hence, we argue that
the smaller PLM is more practical in extensive log analysis
scenarios [23, 24, 25].}
    \item We modify the  discussion in the related work (\textbf{Section II.B, Page 3:}) \\
    \uline{\textbf{Section II.B, Page 3:}} \textcolor{blue}{However, restricted accessibility, higher costs, and computational inefficiency limit the widespread use of LLM in real-world scenarios. For example, the GPT-3 model with
175 billion parameters requires 326GB of GPU memory to
deploy [65]. Given the enormous data volumes produced by
modern software systems daily, the overhead of querying
LLMs, including inference time and network latency, renders
direct application of LLMs for log analysis impractical. In
contrast, small PLMs with smaller parameters are more efficient compared to LLMs [37]. }
\end{enumerate}

\textbf{C4:} The rigor of the approach description in the paper requires improvement. (Pointed out by all three reviewers)
It is advisable for the authors to consider the constructive comments from the three reviewers and further refine their approach to address these issues.

\textbf{R4:} We apologize for the previous inadequate design and presentation.  After we improve the framework, the latest experimental results gain an improvement over the previous version on all datasets, which is significantly better than the existing baselines.
Specifically, we made the following improvements to the original framework:
\begin{itemize}
    \item We employ the more powerful LLM (GPT-4o) as the backbone to build the MEC framework in our experiments;
    \item We refine the design of the MEC framework from the following two aspects, including: 1) Constructing the contrastive examples to improve the Evaluator's evaluation capability under the challenging reference-free setting; and 2) Constructing the evaluation and refinement mechanisms as the iterative framework.
\end{itemize}.

\uline{Our main revisions are as follows:}

\begin{enumerate}
    \item We modify the introduction of role design in \textbf{Section III.B}. \\
    \uline{\textbf{Section III.B.1), Page 4:}} \textcolor{blue}{\textbf{Director.} The Director’s primary objective is to establish
a comprehensive high-level framework aimed at providing
a strategic overview to drive the team’s efforts in
understanding logs. This role outlines the key points essential
for log understanding, thus ensuring that essential
insights are highlighted and comprehensively addressed.} \\
\textcolor{blue}{\textbf{Executor.} As the central role of this team, the Executor is tasked with the detailed execution of the log analysis
process. By receiving key points from the Director and
feedback from the Evaluator, the Executor undertakes
content generation and refinement two critical responsibilities.
Firstly, the Executor generates content intricately
aligned with the outlined key points. Secondly, the Executor
refines and polishes the content based on feedback,
enhancing the knowledge quality.} \\
\textcolor{blue}{\textbf{Evaluator.} The Evaluator assumes the crucial responsibility
of ensuring the quality and adherence of generated
content to predefined requirements. We define three evaluation
requirements for the Evaluator to scrutinize the
Executor’s generation on three fundamental aspects: completeness,
consistency, and conciseness. By evaluating
content against these criteria, the Evaluator validates the
accuracy and completeness of the generated knowledge.} 
\item We add the introduction of contrastive examples in \textbf{Section III.B}. \\
\uline{\textbf{Section III.B.2), Page 4-5:}} \textcolor{blue}{LLM Hallucinations
seriously affect the accuracy and quality of outputs
[70, 71]. Given the propensity of LLM-generated content to
exhibit deficiencies in comprehensiveness and informativeness,
ensuring the superior quality of directly generated knowledge
poses a significant challenge. To mitigate the hallucination of
LLM and ensure the quality of expert knowledge, we build the role of an Evaluator in the MEC framework and define
three evaluation aspects to evaluate the quality of generated
knowledge automatically, which encourages the LLM to actively
seek more detailed suggestions from the self-evaluation
before delivering a formal response. However, the MEC
framework runs under the challenging reference-free setting
and the evaluation requirements cannot be directly quantified
through metrics, the LLM tends to generate ambiguous and inconsistent
evaluations without fine-grained distinguishability,
causing unsatisfactory evaluation performance [72, 73].} \\
\textcolor{blue}{To address the evaluation weaknesses of the LLM, we
provide evaluation examples as the reference in the Evaluator
prompt. By providing specific examples, the Evaluator uses
them as the basis for evaluation, thus better steering the
evaluation of LLMs towards our desired goals. Considering
that the single type of example makes the LLM biased,
motivated by contrastive learning techniques [74, 75], we construct
contrastive examples consisting of positive and negative
knowledge of the same log to Evaluator as reference examples,
where the positive example showcases the desired knowledge,
while the negative example highlights the unsatisfactory
knowledge that should be avoided. By analyzing both types of
examples before generating the evaluation, the Evaluator can
reason about our evaluation requirements and make a more
informed decision about how to evaluate.} \\
\textcolor{blue}{
Specifically, we select one log $L$ with high-quality knowledge $K_{pos}$ as the positive example, which can be manually constructed by experts or generated from the LLM and manually confirmed. Considering that negative examples $\{K_{neg}\}_{c=1} ^ C, C=3$ of the log $L$ are unavailable directly, to construct the negative examples automatically, we propose to prompt the LLM to modify the positive knowledge making it unsatisfactory for evaluation.
As shown in \textcolor{red}{Fig. \ref{fig:negative_template-r0}}, we first give the background in the prompt and then clarify the task of modifying knowledge for the LLM, where we can specify which evaluation metrics are not fulfilled. Next, we provide the raw log, the raw positive knowledge, the key points, and the three evaluation requirements in the prompt.
Finally, we require the LLM to give the reason for not fulfilling the evaluation requirements while generating the modified content, which not only improves the reasoning ability of the \textit{Evaluator} but also provides guidance for the revision of the content by \textit{Executor}.
In cases where the LLM-generated negative examples do not capture the characteristics we want to avoid, this can be manually checked, and feedback can be given to the LLM to re-generate negative samples. 
To avoid the higher expense of the longer prompt, we construct one positive knowledge and its corresponding three negative knowledge as reference examples to be provided to the \textit{Evaluator}. 
The contrastive examples we constructed in our experiments are in Fig. 6.}

\item We modify the introduction of collaboration in \textbf{Section III.B}. \\
\uline{\textbf{Section III.B.3), Page 5:}} \textcolor{blue}{After constructing evaluation examples and assigning roles to LLMs, different roles start working to collaborate and interact according to the requirements in the prompt. 
First, the \textit{Director} meticulously analyzes the input logs to discern key points and formulates a plan for comprehending the logs effectively. Subsequently, the \textit{Director} shares these insights with the \textit{Executor} to guide the content generation process. The \textit{Executor} utilizes these key points to create detailed content that aligns with the requirements.
Finally, the detailed content produced by the \textit{Executor} undergoes evaluation by the \textit{Evaluator} to assess its quality. If the content meets the evaluation requirement, it is directly output as expert knowledge. In cases where the evaluation result is unsatisfactory and improvements are needed, the \textit{Evaluator} provides feedback to the \textit{Executor} for refinement.  To rigorously ensure the quality of the generated knowledge, this evaluation and refinement mechanism will be iterative until the content generated by \textit{Executor} meets the evaluation requirement or the maximum number of iterations is reached. We set up 3 iterations to build expert knowledge in our experiments. The pseudocode of the multi-expert collaboration framework is outlined in Algorithm \ref{alg:algorithm-r0}.
} \\
\textcolor{blue}{ This collaborative framework manifests two pivotal advantages:
Firstly, leveraging multiple roles' collective insights and skills enables a multi-perspective analysis of the input log, 
thereby mitigating the one-sidedness and bias inherent in a single model's response acquiring more professional expert knowledge. 
Secondly, through the feedback loop mechanism, the framework enables iterative refinement of content. This iterative process of evaluation, feedback incorporation, and content enhancement promotes continuous improvement, thereby ensuring that the expert knowledge acquired is comprehensive and of high quality.}
\end{enumerate}

\begin{figure}[]
\centering
   \includegraphics[width=\linewidth]{new_fig/luk_prompt_template.pdf}
   \caption{\textcolor{blue}{Prompt template of constructing negative samples, where the underlined portion of the prompt supports user modification based on their own data and intent.}}
   \label{fig:negative_template-r0}
\end{figure}


\begin{algorithm}
\caption{\textcolor{blue}{Pseudocode of multi-expert collaboration.}}
\label{alg:algorithm-r0}
\begin{algorithmic}
\REQUIRE \textcolor{blue}{Input Log $log$, LLM $\mathcal{M}$, Example Knowledge   $K_{pos}$}      %输入条件
\ENSURE \textcolor{blue}{Output Expert Knowledge $k$}
\STATE \textcolor{gray}{\# Construct Contrastive Examples}
\FOR{\textcolor{blue}{$c = 1$ to $C$}}
    \STATE \textcolor{blue}{$K_{neg}^c = \mathcal{M}(Prompt_{Modify}, K_{pos})$}
\ENDFOR
\STATE  \textcolor{blue}{$K_{examples} = K_{pos} \cup \{K_{neg}\}_{c=1} ^ C $}
\STATE \textcolor{gray}{\# Initial Roles}
\STATE $\mathcal{DIRECTOR} = Init\_Role(Prompt_{Dirctor}, \mathcal{M}) $
\STATE $\mathcal{EXECUTOR} = Init\_Role(Prompt_{Executor}, \mathcal{M}) $
\STATE \textcolor{blue}{$Prompt_{Evaluator} = Prompt_{Evaluator}.join(K_{examples})$}
\STATE \textcolor{blue}{ $\mathcal{EVALUATOR} = Init\_Role(Prompt_{Evaluator},  \mathcal{M})$}
\STATE \textcolor{gray}{\# Collaboration}
\STATE \textcolor{blue}{Init: $epoch = 0, feedback = False$}
\STATE $ keypoint = \mathcal{DIRECTOR}(log) $
\STATE $ content = \mathcal{EXECUTOR}(log, keypoint) $
\REPEAT
\STATE \textcolor{blue}{$ epoch = epoch + 1$}
\STATE \textcolor{blue}{$ feedback = \mathcal{EVALUATOR}(log, keypoint, content) $}
\IF{\textcolor{blue}{$feedback == False$}}
\STATE \textcolor{blue}{$ content = \mathcal{EXECUTOR}(content, feedback) $}
\ENDIF
\UNTIL{\textcolor{blue}{$epoch == Epoch$ or $feedback==True$}}
\STATE $k = content$
\RETURN $k$
\end{algorithmic}
\end{algorithm}

==> response/reviewA.tex <==
\section{Response to Reviewer \#1}

\subsection{Original Comments}
1. RQ1 investigates the performance comparison between the proposed framework LUK and current state-of-the-art models. The experimental results show that although LUK outperforms the six baseline models, the performance gains are minimal and may not be practically significant. For instance, LUK achieves only a 2.5\% improvement in Recall@1, suggesting a limited advantage in retrieving relevant logs. Similarly, in the log and possible cause ranking task for network device logs, LUK improves Precision@1 by just 4.44\%. While an improvement, it does not represent a substantial leap in accuracy.

2. The approach proposed in this paper involves acquiring expert knowledge from large language models (LLMs) and then training a custom model based on such knowledge. This raises a critical question: why not use the large language models directly to perform the tasks, rather than relying on them merely for knowledge extraction? Therefore, I believe it is essential to include a baseline comparison in the experimental section where the tasks are directly handled by an LLM. Additionally, the current approach uses GPT-3.5 to extract expert knowledge. However, models like GPT-4 or GPT-4o are known to significantly outperform GPT-3.5. This brings up another key question: why not leverage the latest or best-performing models for knowledge extraction, given their superior capabilities?

3. I noticed that the authors have published a paper titled “KnowLog: Knowledge Enhanced Pre-trained Language Model for Log Understanding” in ICSE 2024. Could you clarify how this work differs from the current proposed approach? Is it an extension of the conference paper, or is it an entirely new approach? Please provide a clear explanation. If it is an extension of the conference paper, this should be explicitly stated in the manuscript. On the other hand, if it is a completely new contribution, the previous method should be used as a baseline for comparison.

\subsection{Comments and Responses}

\textbf{Response:} The authors are very grateful to the reviewer for the helpful comments and observations. The manuscript has been revised thoroughly according to the reviewer’s advice.

\textbf{C1:} The experimental results show that although LUK outperforms the six baseline models, the performance gains are minimal and may not be practically significant.

\textbf{R1:} Thanks for your suggestions. We apologize for the previous inadequate design and experiments.  After we improve the framework, the latest experimental results gain an improvement over the previous version on all datasets, which is significantly better than the existing baselines.
In particular, as shown in \textcolor{red}{Fig. \ref{fig:low-resource-results}}, LUK is more effective in the challenging log analysis tasks of low-resource scenarios. Hence, we consider LUK to be practical.

Specifically, we made the following improvements to the original framework:
\begin{itemize}
    \item We employ the more powerful LLM (GPT-4o) as the backbone to build the MEC framework in our experiments;
    \item We refine the design of the MEC framework from the following two aspects, including: 1) Constructing the contrastive examples to improve the Evaluator's evaluation capability under the challenging reference-free setting; and 2) Constructing the evaluation and refinement mechanisms as the iterative framework.
\end{itemize}.

\begin{figure*}[]
    \centering
    % \vspace{-2mm}
    \subfloat[Anomaly Detection (BGL)]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_BGL.pdf}}
    \subfloat[LDSM (Huawei-Security)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_ldsm.pdf}}
    \subfloat[Fault Phenomenon Identification]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_fpi.pdf}}
    \caption{Results on different ratios of the training dataset.}
    
    % \vspace{-5mm}
    \label{fig:low-resource-results}
\end{figure*}

\uline{Our main revisions are as follows:}
\begin{enumerate}
    \item We add the more powerful LLMs in our experiments and update all results in the revised manuscript. \\
    \uline{\textbf{Section IV.B, Page 7:}} \textcolor{blue}{As for expert knowledge acquisition, we explore different large language models for experiments, including two proprietary LLMs: \textit{gpt-3.5-turbo} (ChatGPT) and \textit{gpt-4o} (GPT-4o), and one open-source model: \textit{Llama-3.3-70B-Instruct } (LLama3-70B).} 

    \item We modify the introduction of role design in \textbf{Section III.B}. \\
    \uline{\textbf{Section III.B.1), Page 4:}} \textcolor{blue}{\textbf{Director.} The Director’s primary objective is to establish
a comprehensive high-level framework aimed at providing
a strategic overview to drive the team’s efforts in
understanding logs. This role outlines the key points essential
for log understanding, thus ensuring that essential
insights are highlighted and comprehensively addressed.} \\
\textcolor{blue}{\textbf{Executor.} As the central role of this team, the Executor is tasked with the detailed execution of the log analysis
process. By receiving key points from the Director and
feedback from the Evaluator, the Executor undertakes
content generation and refinement two critical responsibilities.
Firstly, the Executor generates content intricately
aligned with the outlined key points. Secondly, the Executor
refines and polishes the content based on feedback,
enhancing the knowledge quality.} \\
\textcolor{blue}{\textbf{Evaluator.} The Evaluator assumes the crucial responsibility
of ensuring the quality and adherence of generated
content to predefined requirements. We define three evaluation
requirements for the Evaluator to scrutinize the
Executor’s generation on three fundamental aspects: completeness,
consistency, and conciseness. By evaluating
content against these criteria, the Evaluator validates the
accuracy and completeness of the generated knowledge.} 
\item We add the introduction of contrastive examples in \textbf{Section III.B}. \\
\uline{\textbf{Section III.B.2), Page 4-5:}} \textcolor{blue}{LLM Hallucinations
seriously affect the accuracy and quality of outputs
[70, 71]. Given the propensity of LLM-generated content to
exhibit deficiencies in comprehensiveness and informativeness,
ensuring the superior quality of directly generated knowledge
poses a significant challenge. To mitigate the hallucination of
LLM and ensure the quality of expert knowledge, we build the role of an Evaluator in the MEC framework and define
three evaluation aspects to evaluate the quality of generated
knowledge automatically, which encourages the LLM to actively
seek more detailed suggestions from the self-evaluation
before delivering a formal response. However, the MEC
framework runs under the challenging reference-free setting
and the evaluation requirements cannot be directly quantified
through metrics, the LLM tends to generate ambiguous and inconsistent
evaluations without fine-grained distinguishability,
causing unsatisfactory evaluation performance [72, 73].} \\
\textcolor{blue}{To address the evaluation weaknesses of the LLM, we
provide evaluation examples as the reference in the Evaluator
prompt. By providing specific examples, the Evaluator uses
them as the basis for evaluation, thus better steering the
evaluation of LLMs towards our desired goals. Considering
that the single type of example makes the LLM biased,
motivated by contrastive learning techniques [74, 75], we construct
contrastive examples consisting of positive and negative
knowledge of the same log to Evaluator as reference examples,
where the positive example showcases the desired knowledge,
while the negative example highlights the unsatisfactory
knowledge that should be avoided. By analyzing both types of
examples before generating the evaluation, the Evaluator can
reason about our evaluation requirements and make a more
informed decision about how to evaluate.} \\
\textcolor{blue}{
Specifically, we select one log $L$ with high-quality knowledge $K_{pos}$ as the positive example, which can be manually constructed by experts or generated from the LLM and manually confirmed. Considering that negative examples $\{K_{neg}\}_{c=1} ^ C, C=3$ of the log $L$ are unavailable directly, to construct the negative examples automatically, we propose to prompt the LLM to modify the positive knowledge making it unsatisfactory for evaluation.
As shown in \textcolor{red}{Fig. \ref{fig:negative_template}}, we first give the background in the prompt and then clarify the task of modifying knowledge for the LLM, where we can specify which evaluation metrics are not fulfilled. Next, we provide the raw log, the raw positive knowledge, the key points, and the three evaluation requirements in the prompt.
Finally, we require the LLM to give the reason for not fulfilling the evaluation requirements while generating the modified content, which not only improves the reasoning ability of the \textit{Evaluator} but also provides guidance for the revision of the content by \textit{Executor}.
In cases where the LLM-generated negative examples do not capture the characteristics we want to avoid, this can be manually checked, and feedback can be given to the LLM to re-generate negative samples. 
To avoid the higher expense of the longer prompt, we construct one positive knowledge and its corresponding three negative knowledge as reference examples to be provided to the \textit{Evaluator}. 
The contrastive examples we constructed in our experiments are in Fig. 6.}

\item We modify the introduction of collaboration in \textbf{Section III.B}. \\
\uline{\textbf{Section III.B.3), Page 5:}} \textcolor{blue}{After constructing evaluation examples and assigning roles to LLMs, different roles start working to collaborate and interact according to the requirements in the prompt. 
First, the \textit{Director} meticulously analyzes the input logs to discern key points and formulates a plan for comprehending the logs effectively. Subsequently, the \textit{Director} shares these insights with the \textit{Executor} to guide the content generation process. The \textit{Executor} utilizes these key points to create detailed content that aligns with the requirements.
Finally, the detailed content produced by the \textit{Executor} undergoes evaluation by the \textit{Evaluator} to assess its quality. If the content meets the evaluation requirement, it is directly output as expert knowledge. In cases where the evaluation result is unsatisfactory and improvements are needed, the \textit{Evaluator} provides feedback to the \textit{Executor} for refinement.  To rigorously ensure the quality of the generated knowledge, this evaluation and refinement mechanism will be iterative until the content generated by \textit{Executor} meets the evaluation requirement or the maximum number of iterations is reached. We set up 3 iterations to build expert knowledge in our experiments. The pseudocode of the multi-expert collaboration framework is outlined in Algorithm \ref{alg:algorithm}.
} \\
\textcolor{blue}{ This collaborative framework manifests two pivotal advantages:
Firstly, leveraging multiple roles' collective insights and skills enables a multi-perspective analysis of the input log, 
thereby mitigating the one-sidedness and bias inherent in a single model's response acquiring more professional expert knowledge. 
Secondly, through the feedback loop mechanism, the framework enables iterative refinement of content. This iterative process of evaluation, feedback incorporation, and content enhancement promotes continuous improvement, thereby ensuring that the expert knowledge acquired is comprehensive and of high quality.}
\end{enumerate}

\begin{figure}[]
\centering
   \includegraphics[width=\linewidth]{new_fig/luk_prompt_template.pdf}
   \caption{\textcolor{blue}{Prompt template of constructing negative samples, where the underlined portion of the prompt supports user modification based on their own data and intent.}}
   \label{fig:negative_template}
\end{figure}


\begin{algorithm}
\caption{\textcolor{blue}{Pseudocode of multi-expert collaboration.}}
\label{alg:algorithm}
\begin{algorithmic}
\REQUIRE \textcolor{blue}{Input Log $log$, LLM $\mathcal{M}$, Example Knowledge   $K_{pos}$}      %输入条件
\ENSURE \textcolor{blue}{Output Expert Knowledge $k$}
\STATE \textcolor{gray}{\# Construct Contrastive Examples}
\FOR{\textcolor{blue}{$c = 1$ to $C$}}
    \STATE \textcolor{blue}{$K_{neg}^c = \mathcal{M}(Prompt_{Modify}, K_{pos})$}
\ENDFOR
\STATE  \textcolor{blue}{$K_{examples} = K_{pos} \cup \{K_{neg}\}_{c=1} ^ C $}
\STATE \textcolor{gray}{\# Initial Roles}
\STATE $\mathcal{DIRECTOR} = Init\_Role(Prompt_{Dirctor}, \mathcal{M}) $
\STATE $\mathcal{EXECUTOR} = Init\_Role(Prompt_{Executor}, \mathcal{M}) $
\STATE \textcolor{blue}{$Prompt_{Evaluator} = Prompt_{Evaluator}.join(K_{examples})$}
\STATE \textcolor{blue}{ $\mathcal{EVALUATOR} = Init\_Role(Prompt_{Evaluator},  \mathcal{M})$}
\STATE \textcolor{gray}{\# Collaboration}
\STATE \textcolor{blue}{Init: $epoch = 0, feedback = False$}
\STATE $ keypoint = \mathcal{DIRECTOR}(log) $
\STATE $ content = \mathcal{EXECUTOR}(log, keypoint) $
\REPEAT
\STATE \textcolor{blue}{$ epoch = epoch + 1$}
\STATE \textcolor{blue}{$ feedback = \mathcal{EVALUATOR}(log, keypoint, content) $}
\IF{\textcolor{blue}{$feedback == False$}}
\STATE \textcolor{blue}{$ content = \mathcal{EXECUTOR}(content, feedback) $}
\ENDIF
\UNTIL{\textcolor{blue}{$epoch == Epoch$ or $feedback==True$}}
\STATE $k = content$
\RETURN $k$
\end{algorithmic}
\end{algorithm}

\textbf{C2:} \textbf{(1)} Why not use the large language models directly to perform the tasks, rather than relying on them merely for knowledge extraction? Therefore, I believe it is essential to include a baseline comparison in the experimental section where the tasks are directly handled by an LLM. \textbf{(2)} Additionally, the current approach uses GPT-3.5 to extract expert knowledge. However, models like GPT-4 or
GPT-4o are known to significantly outperform GPT-3.5. This
brings up another key question: why not leverage the latest or
best-performing models for knowledge extraction, given their
superior capabilities?

\textbf{R2:} Many thanks for your constructive suggestions. We respond to the above two questions as follows:
\begin{enumerate}
    \item Following previous LLM-based log analysis works \cite{xu2024divlog,xu2024unilog,liu2023logprompt,jiang2023llmparser}, we add three different LLMs as baselines, which follow the in-context learning paradigm. Specifically, we select top-5 similar examples from the training set for each input log and use \textit{bge-large-en-v1.5} as the embedding model to select examples. Considering the recency bias of LLMs \cite{zhao2021calibrate}, we arrange these examples in ascending order based on the cosine similarity. As shown in \textcolor{red}{Table \ref{tab: software_results} and \ref{tab: network_result2}}, our results show that apart from LDSM and LPCR tasks, three LLMs perform weaker than the fine-tuned smaller PLMs. This disparity can be ascribed to the presence of a significant domain gap, which hampers the ability of LLMs to effectively address specialized tasks directly. In addition, we also compare the time expense when reasoning with LLMs in \textcolor{red}{Fig. \ref{fig:time-cost}}, and the results show that LUK has a significant advantage over LLMs.
    \item Following your suggestions, we take more powerful LLMs to construct expert knowledge. Specifically, apart from ChatGPT, we also explore \textit{gpt-4o} (GPT-4o) and \textit{Llama-3.3-70B-Instruct} (LLama3-70B) \cite{dubey2024llama} for expert knowledge acquisition. Our findings suggest that GPT4o-based enhancement outperforms the other two LLMs on most datasets, indicating the enhancement effectiveness of the small model is positively correlated with the capability of the LLM.
\end{enumerate}


\begin{figure}[]
    \centering
    % \vspace{-2mm}
    \subfloat[LDSM (Huawei-Switches)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 2.pdf}}
    
    \subfloat[LPCR (Huawei-Switches)]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 1.pdf}}

    \subfloat[Anomaly Detection (BGL)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 3.pdf}}
    
    \caption{\textcolor{blue}{Time expense of different models during reasoning.}}
    
    % \vspace{-5mm}
    \label{fig:time-cost}
\end{figure}

\begin{table}[]
\color{blue}
\centering
\caption{Results on AD and FI (software system logs).}
\label{tab: software_results}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc|c}
\toprule[1.5pt]
\multirow{2}{*}{Methods} & AD (Precision / Recall / F1) & FI (Recall@1 / 2 / 3)                     \\
                         & BGL                          & OpenStack                                 \\ \midrule
CNN                      & \textbf{99.95} / 96.06 / 97.97        & 83.75 / 86.25 / 90.00                     \\
BiLSTM                   & \textbf{99.95} / 97.25 / 98.58        & 87.50 / 92.50 / 96.25                     \\
BERT                     & 99.70 / 98.48 / 99.09        & 87.50 / 92.50 / \textbf{98.75}                     \\
Biglog                   & 99.87 / 99.63 / 99.75        & 90.00 / 95.00 / \textbf{98.75}                     \\
KnowLog                  & 99.58 / 98.69 / 99.13        & 82.50 / 92.50 / 96.25                     \\ \midrule
T5-KD                    & 99.87 / 99.56 / 99.91        & 86.25 / 92.50 / 98.75                     \\ \midrule
LLama3-70B               & 46.87 / 95.23 / 71.05        & 85.00 / \textbf{96.25} / 96.25                     \\
ChatGPT                  & 42.73 / 95.23 / 68.98        & 83.75 / 95.00 / 96.25                     \\
GPT-4o                   & 46.85 / 95. 23 / 70.54       & 87.50 / \textbf{96.25} / 96.25                     \\ \midrule
LUK (COT-ChatGPT)        & 99.95 / 99.87 / 99.91        & 91.25 / 95.00 / \textbf{98.75}                     \\
LUK (COT-GPT4o)          & 99.67 / \textbf{100.0} / 99.83        & 91.25 / 95.00 / \textbf{98.75}                     \\ \midrule
LUK (MEC-LLama3)         & 99.87 / \textbf{100.0} / \textbf{99.93}        & \multicolumn{1}{l}{\textbf{92.50} / 95.00 / \textbf{98.75}} \\
LUK (MEC-ChatGPT)        & 99.95 / 99.91 / 99.93        & \multicolumn{1}{l}{\textbf{92.50} / 95.00 / \textbf{98.75}} \\
LUK (MEC-GPT4o)          & 99.87 / \textbf{100.0} / \textbf{99.93}       & \multicolumn{1}{l}{\textbf{92.50} / \textbf{96.25} / 96.25} \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\begin{table*}[]
\color{blue}
\centering
\caption{Results on MC and LDSM (network device logs).}
\label{tab: network_result}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc|cccc}
\toprule[1.5pt]
\multirow{3}{*}{Methods} & \multicolumn{4}{c|}{MC (Accuracy / Weighted F1)}                                   & \multicolumn{4}{c}{LDSM (Accuracy / Weighted F1)}                                  \\ \cmidrule{2-9} 
                         & \multicolumn{2}{c|}{Cisco}                         & \multicolumn{2}{c|}{Huawei}   & \multicolumn{2}{c|}{Cisco}                         & \multicolumn{2}{c}{Huawei}    \\
                         & Switches      & \multicolumn{1}{c|}{Routers}       & Switches      & Routers       & Switches      & \multicolumn{1}{c|}{Routers}       & Switches      & Routers       \\ \midrule
CNN                      & 56.89 / 56.85 & \multicolumn{1}{c|}{57.46 / 54.92} & 74.52 / 73.95 & 72.78 / 72.23 & 84.04 / 84.04 & \multicolumn{1}{c|}{80.99 / 80.99} & 86.05 / 86.05 & 82.37 / 82.30 \\
BiLSTM                   & 55.74 / 55.63 & \multicolumn{1}{c|}{57.17 / 56.76} & 76.52 / 75.49 & 73.96 / 73.30 & 89.45 / 89.44 & \multicolumn{1}{c|}{85.42 / 85.41} & 87.85 / 87.85 & 84.43 / 84.40 \\
BERT                     & 62.67 / 61.38 & \multicolumn{1}{c|}{62.72 / 62.60} & 82.37 / 81.20 & 81.18 / 79.20 & 93.06 / 93.06 & \multicolumn{1}{c|}{90.01 / 90.00} & 93.18 / 93.18 & 90.06 / 90.05 \\
Biglog                   & 62.69 / 62.76 & \multicolumn{1}{c|}{63.15 / 61.17} & 83.24 / 83.25 & 82.36 / 81.19 & 93.32 / 93.32 & \multicolumn{1}{c|}{91.46 / 91.46} & 94.19 / 94.19 & 93.62 / 93.61 \\
KnowLog                  & 63.33 / 63.35 & \multicolumn{1}{c|}{63.65 / 63.12} & 84.11 / 83.65 & 83.55 / 82.41 & 95.05 / 95.05 & \multicolumn{1}{c|}{92.78 / 92.78} & 97.15 / 97.15 & 96.43 / 96.43 \\ \midrule
T5-KD                    & 62.96 / 62.36 & \multicolumn{1}{c|}{63.86 / 61.01} & 83.60 / 83.23 & 83.55 / 82.82 & 95.29 / 95.28 & \multicolumn{1}{c|}{93.20 / 93.20} & 95.25 / 95.25 & 93.97 / 93.97 \\ \midrule
LLama3-70B               & 61.61 / 60.95 & \multicolumn{1}{c|}{62.99 / 60.55} & 82.98 / 82.83 & 81.66 / 80.34 & 84.48 / 84.31 & \multicolumn{1}{c|}{88.32 / 88.24} & 95.49 / 95.49 & 95.57 / 95.57 \\
ChatGPT                  & 57.11 / 54.41 & \multicolumn{1}{c|}{57.99 / 54.56} & 79.14 / 77.19 & 78.22 / 75.51 & 82.14 / 81.96 & \multicolumn{1}{c|}{84.64 / 84.47} & 85.75 / 85.75 & 90.31 / 90.22 \\
GPT-4o                   & 62.12 / 61.62 & \multicolumn{1}{c|}{63.86 / 61.01} & 83.25 / 82.80 & 81.30 / 79.87 & 89.04 / 88.99 & \multicolumn{1}{c|}{93.12 / 93.11} & 97.23 / 97.23 & \textbf{97.79} / \textbf{97.79} \\ \midrule
LUK (COT-ChatGPT)        & 63.49 / 63.72 & \multicolumn{1}{c|}{64.51 / 63.33} & 83.42 / 82.70 & 83.19 / 82.34 & 94.93 / 94.92 & \multicolumn{1}{c|}{93.11 / 93.11} & 96.33 / 96.33 & 95.73 / 95.73 \\
LUK (COT-GPT4o)          & 63.47 / 63.51 & \multicolumn{1}{c|}{63.61 / 63.02} & 83.60 / 83.20 & 82.84 / 81.92 & 94.92 / 94.91 & \multicolumn{1}{c|}{93.18 / 93.18} & 96.46 / 96.46 & 95.93 / 95.93 \\ \midrule
LUK (MEC-LLama3)         & 65.67 / 65.27 & \multicolumn{1}{c|}{66.67 / 65.12} & 85.25 / 84.95 & 85.21 / 84.01 & 96.45 / 96.45 & \multicolumn{1}{c|}{94.13 / 94.13} & 97.66 / 97.66 & 97.39 / 97.39 \\
LUK (MEC-ChatGPT)        & 65.54 / 65.12 & \multicolumn{1}{c|}{66.29 / 64.27} & 84.64 / 84.47 & 85.09 / 83.82 & 96.32 / 96.32 & \multicolumn{1}{c|}{93.80 / 93.80} & 96.92 / 96.92 & 96.74 / 96.74 \\
LUK (MEC-GPT4o)          & \textbf{66.16} / \textbf{66.02} & \multicolumn{1}{c|}{\textbf{67.20} / \textbf{65.41}} & \textbf{85.51} / \textbf{85.26} & \textbf{85.33} / \textbf{84.73} & \textbf{96.63} / \textbf{96.63} & \multicolumn{1}{c|}{\textbf{94.32} / \textbf{94.32}} & \textbf{97.66} / \textbf{97.66} & 97.34 / 97.34 \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table*}


\begin{table}[]
\color{blue}
\centering
\caption{Results on LPCR and FPI (network device logs). Note: The results of proprietary LLMs on the FPI task cannot be compared due to data privacy issues.}
\label{tab: network_result2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|c}
\toprule[1.5pt]
\multirow{3}{*}{Methods} & \multicolumn{2}{c|}{LPCR (Precision@1 / 3 / MRR)} & FPI (Accuracy) \\ \cmidrule{2-4} 
                         & \multicolumn{2}{c|}{Huawei}                       & Huawei         \\
                         & Switches                & Routers                 & Switches       \\ \midrule
CNN                      & 54.30 / 77.26 / 67.99   & 53.45 / 75.77 / 67.35   & 69.00          \\
BiLSTM                   & 59.27 / 78.04 / 71.22   & 51.45 / 69.56 / 63.76   & 74.83          \\
BERT                     & 76.18 / 91.54 / 84.70   & 72.57 / 91.59 / 82.61   & 88.75          \\
Biglog                   & 83.33 / 94.02 / 89.38   & 82.98 / 95.59 / 89.49   & 89.58          \\
KnowLog                  & 87.50 / 93.01 / 91.84   & 89.68 / 96.59 / 93.99   & 94.17          \\ \midrule
T5-KD                    & 86.11 / 93.56 / 91.41   & 84.48 / 92.59 / 90.33   & -              \\ \midrule
LLama3-70B               & \textbf{95.61} / \textbf{98.04} / \textbf{97.27}   & \textbf{97.48} / \textbf{99.49} / \textbf{98.52}   & 88.83          \\
ChatGPT                  & 90.95 / 95.11 / 93.88   & 97.20 / 98.34 / 98.19   & -              \\
GPT-4o                   & 95.65 / 98.29 / 97.27   & 97.39 / 99.09 / 98.47   & -              \\ \midrule
LUK (COT-ChatGPT)        & 85.18 / 95.03 / 90.55   & 84.58 / 95.99 / 90.64   & 90.42          \\
LUK (COT-GPT4o)          & 86.34 / 93.79 / 91.37   & 87.88 / 95.19 / 92.75   & 92.50          \\ \midrule
LUK (MEC-LLama3)         & 90.45 / 95.81 / 94.06   & 90.49 / 96.99 / 94.52   & 95.83          \\
LUK (MEC-ChatGPT)        & 89.37 / 95.19 / 93.43   & 88.48 / 94.69 / 90.33   & 93.33          \\
LUK (MEC-GPT4o)          & 90.92 / 96.04 / 94.46   & 90.69 / 96.09 / 94.39   & \textbf{96.67}          \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\uline{Following your suggestions, (1) we take the LLM following the ICL paradigm as the baseline.
(2) We supplement the experiment by utilizing GPT-4o and LLama3-70b to construct knowledge. The details are illustrated as follows:}

\begin{enumerate}
    \item \uline{ \textbf{Section IV.D, Page 10:}} \textcolor{blue}{LLM-based log analysis methods follow the \textit{in-context learning} paradigm, where LLMs make predictions based on contexts augmented with a few examples without training.
Following previous LLM-based log analysis works [26,27,28,29], we select top-5 similar examples from the training set for each input log and use \textit{bge-large-en-v1.5} as the embedding model to select examples, due to its excellent performance among all open-source embedding models. Considering the recency bias of LLMs [87]{zhao2021calibrate}, we arrange these examples in ascending order based on the cosine similarity. We select two proprietary LLMs (\textbf{ChatGPT} and \textbf{GPT-4o}) and one powerful open-source LLM (\textbf{LLama3-70B [79]}) as baselines. We utilize HTTP requests to invoke the OpenAI APIs and interact with proprietary LLMs. For open-source LLM, we deploy \textit{Llama-3.3-70B-Instruct} in our environments to analyze logs.}

    \item \uline{\textbf{Section IV.B, Page 7:}} \textcolor{blue}{As for expert knowledge acquisition, we explore different large language models for experiments, including two proprietary LLMs: \textit{gpt-3.5-turbo} (ChatGPT) and \textit{gpt-4o} (GPT-4o), and one open-source model: \textit{Llama-3.3-70B-Instruct } (LLama3-70B) [79].} 
\end{enumerate}

\textbf{C3:} Could you clarify how KnowLog differs from the current proposed approach? Is it an extension of the conference paper, or is it an entirely new approach? Please provide a clear explanation.

\textbf{R3:} Thanks for your reminder. LUK is a completely new approach, not an extension of KnowLog. 
First, LUK focuses on the challenge of the high cost and inefficiency of reasoning for Large Language Models (LLMs). It introduces a novel framework that reduces the computational overhead of LLMs by distilling knowledge into smaller models, enhancing practicality in log analysis contexts. In contrast, KnowLog's primary emphasis lies in leveraging existing domain knowledge to enhance log understanding.
Second, LUK has an advantage over KnowLog in terms of knowledge acquisition. KnowLog enhances the model based on existing documentation knowledge, however, most logs lack documentation, and the cost of manually constructing knowledge is extremely high, KnowLog cannot work in the absence of documentation. LUK, on the other hand, does not need to rely on existing documentation and obtains sufficient knowledge through the LLM, which is even of higher quality than the documentation knowledge, thus making LUK more practical. 
Third, LUK proposes a new pre-training task from the word level. KnowLog's abbreviation prediction task only recognizes the abbreviations that are already in the log. It cannot understand other key information within the log's tokens (such as parameters) and cannot perceive useful information from external knowledge to enhance the understanding of domain tokens. And LUK can adaptively perceive useful knowledge to understand tokens in logs, not limited to abbreviations. 
Finally, experimentally, experimental results verify the LUK's superiority over KnowLog. Our experiments and case studies demonstrate that LUK consistently outperforms KnowLog across various metrics, substantiating the efficacy and advancement of our proposed approach.

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{new_fig/luk_knowledge_case.pdf}
   % \vspace{-6mm}
   \caption{\textcolor{blue}{Example of knowledge generated by GPT-4o and retrieved from documentation.}}
   % \vspace{-4mm}
   \label{fig:knowledge_case}
\end{figure*}

\begin{figure}[]
\centering
    % \vspace{-2mm}
    \includegraphics[width=\columnwidth]{new_fig/LUK_percentage_1.pdf}    
    
    \caption{\textcolor{blue}{Proportion of unsatisfactory knowledge, where we employ the evaluation criteria of the MEC framework to evaluate the knowledge.}}
    
    % \vspace{-5mm}
    \label{fig:doc-knowledge-analysis}
\end{figure}

\uline{Our main revisions are as follows:}
\begin{enumerate}
    \item We emphasize the focus of this paper in the introduction: \\ \uline{\textbf{Section I, Page 1-2:}} \textcolor{blue}{Despite the powerful performance of LLMs, limited accessibility
and higher costs present significant challenges in
leveraging the full potential of LLMs. These LLMs often
come with substantial usage fees and have restricted access
to data privacy and security. Even if the LLM is deployed
locally, it still may face resource constraints, making LLMs
less attainable for individuals and smaller organizations. In
addition, due to their complex autoregressive architectures
and a large number of parameters, LLM-based methods are computationally inefficient. Considering that modern software
systems can produce several petabytes per day [34, 35],
directly employing LLMs for log analysis is impractical due to
the significant overhead of querying LLMs, such as inference
time and network latency [29, 36]. In contrast, smaller PLMs
with smaller parameters, requiring limited resource costs,
are more efficient than LLMs [37]. Hence, we argue that
the smaller PLM is more practical in extensive log analysis
scenarios [23, 24, 25].}
    \item We modify the introduction of KnowLog in \textbf{Section I, Page 2:} \\
    \uline{\textbf{Section I, Page 2:}} \textcolor{blue}{This issue can be
attributed to the lack of rich sources for knowledge acquisition.
Although KnowLog proposes to acquire expert knowledge
from documentation [22], most logs lack professional documentation
(e.g. almost unable to find relevant documents for
logs coming from Loghub [38]) and the manual construction of
knowledge is costly and inefficient, which significantly hinders
the availability of the model.} \\
    \uline{\textbf{Section I, Page 2:}} \textcolor{blue}{In addition, KnowLog proposes an abbreviation
prediction task specialized for log understanding. However, its
ability only to enhance the knowledge of abbreviations in the
logs is limited. It cannot adaptively perceive other important
information from the knowledge to understand logs, such as
the parameter knowledge of logs.}
    \item We add KnowLog as the baseline in our experiments. \\
    \uline{\textbf{Section IV.D.2), Page 10:}} 
    \textcolor{blue}{In addition, KnowLog is the state-of-the-art log pre-trained model in log analysis not only due to pre-training on log corpus but also enhancing the pre-training with documentation knowledge. Referring to KnowLog, we collect the descriptions of logs from the Huawei and Cisco public documentation as background knowledge to enhance the log pre-training in the same way. For fairness, we reproduce Biglog and KnowLog with the same pre-training setting on our log corpus.} 
    \item We add the analysis of the experiments about KnowLog in \textbf{Section IV.E, Page 11-14:} \\
    \uline{\textbf{Section IV.E.RQ1, Page 11:}} \textcolor{blue}{To verify the effectiveness of the expert knowledge obtained
from the LLM, we compare it with the KnowLog, whose
knowledge is obtained from the documentation. Our experimental
findings demonstrate that MEC-based LUK surpasses
KnowLog in performance, more specifically, LUK (MECGPT4o)
improves the average Accuracy on the Cisco and
Huawei datasets regarding the MC and LDSM tasks by 2.38\%
and 1.15\%, respectively. It is noteworthy that Huawei’s documentation
provides more detailed log descriptions compared
to the relatively concise descriptions found in Cisco’s documentation.
This disparity underscores the LLM’s capability
to generate domain knowledge of equal or superior quality to that found in high-quality documentation. Given the scarcity of
documented descriptions for most logs in practice, obtaining
expert knowledge through KnowLog becomes impractical. For
instance, the challenge of sourcing relevant documents for
logs from sources like Loghub [38] significantly hampers
the effectiveness of KnowLog. Our approach, which operates
independently of documentation, consistently yields superior
results, and serves to diminish the reliance on human experts
for intricate knowledge construction processes, offering a more
feasible and practical alternative to traditional documentation-based
methodologies.} \\
    \uline{\textbf{Section IV.E.RQ2, Page 12:}} \textcolor{blue}{
    In comparison to KnowLog, LUK still has a clear advantage
over KnowLog, which takes knowledge from the documentation.
The domain knowledge derived from LLMs offers a deeper
level of comprehension and learning, enabling the PLM to
generalize more effectively to new log datasets. Conversely,
KnowLog, constrained by information within documents, may
not provide sufficiently profound domain insights to support
robust generalization of the PLM to unseen data.} \\
    \uline{\textbf{Section IV.E.RQ3, Page 13:}} \textcolor{blue}{In contrast, KnowLog’s reliance on knowledge
solely extracted from documentation may lead to limitations
in handling the evolving nature of log data.} \\
    \uline{\textbf{Section IV.E.RQ4, Page 14:}} \textcolor{blue}{KnowLog primarily relies on
knowledge extracted from documentation, which may be limited
in scope and quality, especially in low-resource settings.
In contrast, this proves that knowledge acquired by the LLM
has a wider scope and can provide a more comprehensive
and diverse range of information, rather than being limited to
some specific documentation.}
    \item To further verify our proposed word-level Token Prediction (TP) task,
we also compare it with other word-level pre-training tasks \textcolor{red}{Table \ref{tab:ablation}},
including BERT’s Masked Language Modeling (MLM) task
and KnowLog’s Abbreviation Prediction (AP) task. \\
    \uline{\textbf{Section IV.F, Page 14:}} \textcolor{blue}{
    To further verify our proposed word-level Token Prediction (TP) task,
we also compare it with other word-level pre-training tasks,
including BERT’s Masked Language Modeling (MLM) task
and KnowLog’s Abbreviation Prediction (AP) task. The results
demonstrate the superior capability of our token prediction
task in integrating domain knowledge effectively. Unlike MLM
and Abbreviation Prediction tasks, our proposed pre-training
task requires models to not only predict tokens within the
log itself but also dynamically assimilate contextual insights
from domain-specific knowledge using the knowledge perception
module. This distinctive aspect sets our approach apart,
as BERT solely relies on internal information and cannot
leverage external knowledge. Conversely, KnowLog is limited
in its scope, focusing solely on abbreviations and failing to
comprehend other critical log elements such as parameters,
conditions, and more, which are essential for a comprehensive
understanding of domain-specific terminology.}
    \item We add the case study to analyze the quality of the expert knowledge from different sources in \textbf{Section V.B.2), Page 17:} \\
    \uline{\textbf{Section V.B.2), Page 17:}} \textcolor{blue}{Evaluation and refinement mechanism of the MEC
framework: To further intuitively analyze the quality of the expert knowledge constructed with the MEC framework, we compare it with the knowledge collected from documentation and the COT-based approach. As shown in \textcolor{red}{Fig. \ref{fig:knowledge_case}}, we collect a Cisco log as the case and give the corresponding generated knowledge based on the COT and MEC methods.} \\
    \textcolor{blue}{
As can be seen from these cases, the knowledge provided by the documentation is too simple, which provides a generic and limited understanding of the log without delving into specific details or potential causes. Although COT-based knowledge offers a more detailed explanation of the log, compared to MEC-based knowledge, there is still the problem of inadequate knowledge and lack of insight.
In contrast, the knowledge derived from the MEC framework excels in its comprehensive analysis and insights. By explicitly outlining the specifics of the log error, including the MTS queue failure and the placeholders for queue and error message, the MEC-based knowledge provides a deeper understanding of the issue at hand. Furthermore, it goes beyond mere description to identify potential root causes such as network connectivity issues.
The comparison highlights the clear advantage of the MEC framework in expert knowledge generation. Its collaborative nature allows for the integration of diverse expertise and perspectives, resulting in a more comprehensive analysis of complex logs.} \\ 
\textcolor{blue}{
To quantify the differences among the various forms of knowledge, we employ the evaluation criteria of the MEC framework to evaluate the knowledge acquired by the documentation and the knowledge constructed based on COT in the network device logs. The evaluation results are shown in \textcolor{red}{Fig. \ref{fig:doc-knowledge-analysis}}, revealing a notable contrast in quality between the different sources of knowledge. It is apparent from the analysis that a significant proportion of knowledge sourced from documentation falls short of meeting the evaluation requirements. This deficiency can be attributed to the inherent limitations of documentation-derived knowledge, which often lacks depth and detail, offering only the most straightforward description of the logs. Combined with Fig. 10a, this suggests that the knowledge acquired from MEC based on LLMs is comparable or even better than the documentation. Considering the lack of documentation support for most logs and the high cost of manually constructing knowledge, this provides a feasible way to gain a wealth of practical knowledge automatically.}

\end{enumerate}

\begin{table}[]
\centering
\color{blue}
\caption{\textcolor{blue}{Ablation studies for LUK, where TP and SA represent the pre-training tasks Token Prediction, and Semantic Alignment for LUK, respectively. MLM represents the pre-training task Masked Language Modeling of BERT and AP represents the pre-training task Abbreviation Prediction of KnowLog.}}
\label{tab:ablation}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|cc}
\toprule[1.5pt]
\multirow{3}{*}{Methods}         & \multicolumn{2}{c|}{MC (Accuracy / Weighted-F1)} & \multicolumn{2}{c}{LDSM (Accuracy / Weighted-F1)} \\ \cmidrule{2-5} 
                                 & \multicolumn{2}{c|}{Huawei}                      & \multicolumn{2}{c}{Huawei}                        \\
                                 & Switches                & Routers                & Switches                & Routers                 \\ \midrule
BERT                             & 82.37 / 81.20           & 81.18 / 79.20          & 93.18 / 93.18           & 90.06 / 90.05           \\
LUK (MEC-GPT4o)                  & \textbf{85.51} / \textbf{85.26}           & \textbf{85.33} / \textbf{84.73}          & \textbf{97.66} / \textbf{97.66}           & \textbf{97.34} / \textbf{97.34}           \\ \midrule
$\vdash$ w/o Evaluator           & 83.77 / 83.26           & 82.30 / 81.08          & 96.57 / 96.57           & 95.53 / 95.53           \\
$\vdash$ w/o Evaluation Examples & 84.38 / 84.17           & 82.13 / 81.06          & 96.64 / 96.64           & 95.63 / 95.63           \\ \midrule
$\vdash$ w/o TP                  & 83.25 / 82.65           & 81.66 / 79.92          & 95.95 / 95.95           & 95.68 / 95.68           \\
$\vdash$ w/o SA                  & 83.77 / 83.19           & 84.14 / 82.92          & 95.25 / 95.25           & 94.68 / 94.68           \\ \midrule
$\vdash$ only with MLM           & 83.24 / 83.25           & 82.36 / 81.19          & 94.19 / 94.19           & 93.62 / 93.61           \\
$\vdash$ only with AP            & 83.60 / 82.89           & 82.72 / 81.68          & 94.39 / 94.39           & 93.97 / 93.97           \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}



==> response/reviewB.tex <==
\section{Response to Reviewer \#2}

\subsection{Original Comments}
Overall, I find the paper easy to read and the technical details of the proposed approach are comprehensively presented. The basic idea of LUK is to leverage the LLM to enrich the training corpus of PLMs. Though I find it somehow similar to knowledge distillation, I believe the proposed multi-expert collaboration framework to acquire the high-quality data from LLM and the two pretrain tasks to inject the knowledge are novel. Moreover, I appreciate the extensive experiments conducted in the paper, which comprehensively illustrate the effectiveness of LUK under different usage scenarios (e.g., unseen logs, unstable log, and limited labeled data) and the validity of specific designs.

I have the following concerns:

The paper’s key motivation is that LLM, although powerful yet introducing excessive overhead, cannot be directly applied to log understanding, and thus proposing LUK to enhance smaller PLMs with the knowledge from LLM. However, the discussions regarding why LLM cannot be directly applied to log understanding is not sufficiently presented, without which, it would be hard to interpret the practical value of LUK. The only relevant discussion is in the second paragraph of the Introduction where the authors briefly listed two reasons: 1) “… they are sensitive to the context, influencing the model’s behavior significantly …” 2) “… directly employing LLM for log analysis is impractical due to the significantly overhead …”. For reason 1, I would recommend authors to conduct a preliminary study (e.g., investigating the existing LLM-based log understanding approaches [26-30]) or at least give examples to show that small disturbances in inputs could drastically affect LLM, leading to contrary outputs regarding log understanding tasks. As far as I am concerned, LLM with ICL setting works well in many real-world applications. And although disturbances in inputs could affect LLM outputs, it is unlikely, let’s say for Anomaly Detection, turning a right answer of True into False. For reason 2, although authors show in RQ6 that LLM consumes way more computational time, I would recommend authors to experiment with more powerful computational servers (e.g., 8 x A800 instead of 2 x 3090 currently adopted in the paper). Also, considering LLM has a much larger contexts than PLMs, it may be possible that multiple logs can be merged into one input to LLM in order to accelerate. LLM costs more than PLMs is an undeniable fact, however, it dost not prevent the adoption of LLM in numerous real-world applications. Many advanced hardware and software solutions are introduced to alleviate the latency of LLM. Personally, I would say the comparison on 2 x 3090 does not tell much valuable information, as in practice, it is unlikely (e.g., for a cloud service provider who wants to automatically check the logs) to run LLM on 2 x 3090. Besides, the authors need to show that why timeliness is important to log understanding tasks.

The idea of LUK is similar to a well-known task, i.e., knowledge distillation, however, no discussions regarding the connections and differences between LUK and existing approaches of knowledge distillation is presented in the paper. Particularly, authors should identify whether LUK is one type of existing knowledge distillation technique? Whether existing knowledge distillation techniques can be applied to fulfill the goal of LUK? If yes, additional experiments are needed to show that LUK outperforms existing distillation techniques.

Regarding Section 2 related work and motivation, I would kindly ask the authors to adjust the title (if possible, the organization of the content) of the subsection, as the current titles "Pretraining on language models" \& "large language model" are irrelevant to the log understanding.

Regarding the multi-expert collaboration, I have two concerns regarding the specific implementation: 1) In algorithm 1, I notice that if the feedback given by the evaluator is not a PASS, then the executor will re-generate the context based on the previously generated content and the feedback. As far as I am concerned, the log would also be necessary to facilitate re-generation, otherwise how is the executor supposed to regenerate based on its wrong output and the binary feedback given by the executor. 2) I notice that there is no check regarding the re-generated content. It is possible that the re-generated content still contains the error or introduces new errors, thus an iterative process is necessary until the evaluator deems that the generated content is a pass. I suggest authors to implement an iterative process and add additional the experiments.

Regarding the pretraining, I see two encoders in figure 4. I am wondering whether they are two separate BERTs or one BERT but run two times sequentially. If they are two separate BERTs, how do authors conduct the following finetuning? More clarifications are needed.

Regarding the experiments, one critical shortcoming is the lack of the LLM-based log understanding baselines [26-30]. Why do authors exclude them in the experiments? Besides, the authors mention that “considering that ICL suffers from unstable results …, we utilize zero-shot capability of LLMs for log analysis.” I suggest authors to also experiment with the most simplified example selection strategy (e.g., BM 25 similarity, random selection).
Besides, I find the performance of LUK (COT-ChatGPT) and LUK (MEC-ChatGPT) is very close expect when the labeled logs are extremely limited. I suggest authors to enrich the experiments under the limited labeled data scenario, as this is the application scenario where the superiority of LUK lies. Also, it would be better to show the ratio and examples of knowledge outputs that are first rejected by the executor and regenerated, in order to better demonstrate the necessities of incorporating MEC (which in essential adds a self-check process over the raw COT).

\subsection{Comments and Responses}

\textbf{Response:}  We sincerely appreciate the reviewer for the detailed comments, which help improve our work. The manuscript has been carefully revised following your advice.

\textbf{C1:} 
The paper’s key motivation is that LLM, although powerful yet introducing excessive overhead, cannot be directly applied to log understanding, and thus proposing LUK to enhance smaller PLMs with the knowledge from LLM. However, the discussions regarding why LLM cannot be directly applied to log understanding is not sufficiently presented, without which, it would be hard to interpret the practical value of LUK.  The authors briefly listed two reasons: 1) “… they are sensitive to the context, influencing the model’s behavior significantly …” 2) “… directly employing LLM for log analysis is impractical due to the significantly overhead …”. 

\textbf{(1)} For reason 1, I would recommend authors to conduct a preliminary study (e.g., investigating the existing LLM-based log understanding approaches [26-30]) or at least give examples to show that small disturbances in inputs could drastically affect LLM, leading to contrary outputs regarding log understanding tasks. 

\textbf{(2)} For reason 2, although authors show in RQ6 that LLM consumes way more computational time, I would recommend authors to experiment with more powerful computational servers (e.g., 8 x A800 instead of 2 x 3090 currently adopted in the paper). Also, considering LLM has a much larger contexts than PLMs, it may be possible that multiple logs can be merged into one input to LLM in order to accelerate. LLM costs more than PLMs is an undeniable fact, however, it does not prevent the adoption of LLM in numerous real-world applications. Many advanced hardware and software solutions are introduced to alleviate the latency of LLM. Personally, I would say the comparison on 2 x 3090 does not tell much valuable information, as in practice, it is unlikely (e.g., for a cloud service provider who wants to automatically check the logs) to run LLM on 2 x 3090. Besides, the authors need to show that why timeliness is important to log understanding tasks.

\textbf{C1:} Thanks for your comments, we apologize for our non-rigorous discussions of the LLM. We respond to the above two questions as follows:

\begin{enumerate}
    \item This paper's key motivation focuses on exploring the smaller PLM to analyze logs due to the challenge of employing LLMs. Following the ICL paradigm in our experiments, we find that LLMs obtain good performance in log analysis tasks. In fact, LLMs can be used for log analysis, there are just many challenges and smaller models are more practical.
    Hence, we reformulate the challenge of utilizing LLMs for log analysis as follows: 
    \textit{Despite the powerful performance of LLMs, limited accessibility and higher costs present significant challenges in
leveraging the full potential of LLMs. These LLMs often
come with substantial usage fees and have restricted access
to data privacy and security. Even if the LLM is deployed
locally, it still may face resource constraints, making LLMs
less attainable for individuals and smaller organizations. 
In addition, due to their complex autoregressive architectures
and a large number of parameters, LLM-based methods are computationally inefficient.
Hence, we argue that the smaller PLM is more practical in extensive log analysis 
scenarios. }
    \item First, we intend to validate the advantages of the smaller model through the experiment of efficiency, which can reduce the cost of using LLMs or even deploying them in resource-limited scenarios. Second,  we conduct the experiment on 2 NVIDIA A100 GPUs for a fair comparison. As shown in \textcolor{red}{Fig. \ref{fig:time-cost-r2}}, the inference time of LLM is in seconds, while the inference time of smaller PLM is in milliseconds. We would like to use this experiment to show that smaller models have a wider range of application scenarios, such as the potential for smaller models to run on terminal devices in the future.
\end{enumerate}

\uline{We modify the discussion of the challenge for employing LLMs in the introduction and related work. The details are illustrated below:}
\begin{enumerate}
    \item We modify the  discussion in the introduction (\textbf{Section I, Page 1-2:}) \\
    \uline{\textbf{Section I, Page 1-2:}} \textcolor{blue}{Despite the powerful performance of LLMs, limited accessibility and higher costs present significant challenges in
leveraging the full potential of LLMs. These LLMs often
come with substantial usage fees and have restricted access
to data privacy and security. Even if the LLM is deployed
locally, it still may face resource constraints, making LLMs
less attainable for individuals and smaller organizations. In
addition, due to their complex autoregressive architectures
and a large number of parameters, LLM-based methods are computationally inefficient. Considering that modern software
systems can produce several petabytes per day [34, 35],
directly employing LLMs for log analysis is impractical due to
the significant overhead of querying LLMs, such as inference
time and network latency [29, 36]. In contrast, smaller PLMs
with smaller parameters, requiring limited resource costs,
are more efficient than LLMs [37]. Hence, we argue that
the smaller PLM is more practical in extensive log analysis
scenarios [23, 24, 25].}
    \item We modify the  discussion in the related work (\textbf{Section II.B, Page 3:}) \\
    \uline{\textbf{Section II.B, Page 3:}} \textcolor{blue}{However, restricted accessibility, higher costs, and computational inefficiency limit the widespread use of LLM in real-world scenarios. For example, the GPT-3 model with
175 billion parameters requires 326GB of GPU memory to
deploy [65]. Given the enormous data volumes produced by
modern software systems daily, the overhead of querying
LLMs, including inference time and network latency, renders
direct application of LLMs for log analysis impractical. In
contrast, small PLMs with smaller parameters are more ef-
ficient compared to LLMs [37]. }
\item We modify the experiments in \textbf{Section IV.E.RQ6, Page 14-15:}  \\
\uline{\textbf{Section IV.E.RQ6, Page 14-15:}} \textcolor{blue}{Specifically, we perform experiments on
Anomaly Detection, Log and Description Semantic Matching,
and Log and Possible Cause Ranking three tasks to calculate
the inference time with all testing samples. For fairness, we
deploy LLama3-70B and LUK on the same hardware setup,
consisting of 2 NVIDIA A100 GPUs, with a batch size of 1
for each model. It’s worth noting that deploying LUK requires
about 2 GB of GPU-memory, while deploying LLama3-70B
requires 150 GB of GPU-memory. For GPT-4o, we utilize
HTTP requests to invoke the APIs then calculate time.} \\
\textcolor{blue}{The results are shown in Fig. 9, we notice that LUK is
significantly faster than GPT-4o and LLama3. Specifically,
excluding the fine-tuning time, the average inference speed
of LUK is 718x, and 868x faster than GPT-4o and LLama3-
70B, respectively. Even considering the fine-tuning time, the
average inference speed of LUK is still 9x, and 11x faster than
GPT-4o and LLama3-70B. In addition, the average response
time for each input is 4.13, and 4.69 seconds for GPT-4o and LLama3-70B respectively, while LUK’s average response
time is 0.0058 seconds. This swift response time positions
LUK as a more practical solution for real-world log analysis
scenarios. This efficiency can be attributed to the fact that
LLMs possess extensive parameter sizes and generate outputs
sequentially, necessitating more computational steps to deliver
results. In contrast, LUK, with its smaller parameter sizes
and more professional log analysis capabilities, can swiftly
address specific tasks following knowledge enhancement and
fine-tuning.}
\textcolor{blue}{
In conclusion, LLMs demand higher deployment resources
and exhibit slower inference speeds. On the other hand, the
knowledge-enhanced LUK offers rapid responses to inputs
with limited deployment resources, making it a highly recommended choice for executing specific tasks in real-world
scenarios. This advantage underscores the practicality and
efficiency of LUK in comparison to traditional LLMs like
GPT-4o and LLama3-70B.}

\end{enumerate}


\begin{figure}[]
    \centering
    % \vspace{-2mm}
    \subfloat[LDSM (Huawei-Switches)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 2.pdf}}
    
    \subfloat[LPCR (Huawei-Switches)]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 1.pdf}}

    \subfloat[Anomaly Detection (BGL)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 3.pdf}}
    
    \caption{\textcolor{blue}{Time expense of different models during reasoning.}}
    
    % \vspace{-5mm}
    \label{fig:time-cost-r2}
\end{figure}



\textbf{C2:} The idea of LUK is similar to a well-known task, i.e., knowledge distillation, however, no discussions regarding the connections and differences between LUK and existing approaches of knowledge distillation is presented in the paper. Particularly, (1) authors should identify whether LUK is one type of existing knowledge distillation technique? (2) Whether existing knowledge distillation techniques can be applied to fulfill the goal of LUK? If yes, additional experiments are needed to show that LUK outperforms existing distillation techniques.

\textbf{R2:} Thanks for your reminder. We respond to the above two questions as follows:
\begin{enumerate}
    \item LUK can be viewed as a novel framework for knowledge distillation, distinguishing it from existing knowledge distillation techniques. 
    In the era of LLMs, knowledge distillation (KD) \cite{xu2024survey} emerges as a pivotal methodology for transferring advanced capabilities from LLMs to smaller models. However, current state-of-the-art knowledge distillation methods, whose distillation towards the reasoning process, such as COT-based KD \cite{hsieh2023distilling,shridhar2023distilling}, struggle to acquire expert knowledge, instead imitating the teacher’s reasoning forms and ignoring the premise that reasoning requires expert knowledge. These existing distillation methods, which emphasize the process of reasoning and outcome, still hardly compensate for the lack of expert knowledge.
    \item Our experimental results in \textcolor{red}{Table \ref{tab: software_results-r2} and \ref{tab: network_result2-r2}} show that LUK is superior to existing knowledge distillation techniques. Specifically, we select Chain-of-Thought (COT)-based knowledge distillation as the baseline, which has proven to be an effective knowledge distillation method for the reasoning process in the field of NLP. The results show that our framework is more advantageous.  
    
\end{enumerate}

\begin{table}[]
\color{blue}
\centering
\caption{Results on AD and FI (software system logs).}
\label{tab: software_results-r2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc|c}
\toprule[1.5pt]
\multirow{2}{*}{Methods} & AD (Precision / Recall / F1) & FI (Recall@1 / 2 / 3)                     \\
                         & BGL                          & OpenStack                                 \\ \midrule
CNN                      & \textbf{99.95} / 96.06 / 97.97        & 83.75 / 86.25 / 90.00                     \\
BiLSTM                   & \textbf{99.95} / 97.25 / 98.58        & 87.50 / 92.50 / 96.25                     \\
BERT                     & 99.70 / 98.48 / 99.09        & 87.50 / 92.50 / \textbf{98.75}                     \\
Biglog                   & 99.87 / 99.63 / 99.75        & 90.00 / 95.00 / \textbf{98.75}                     \\
KnowLog                  & 99.58 / 98.69 / 99.13        & 82.50 / 92.50 / 96.25                     \\ \midrule
T5-KD                    & 99.87 / 99.56 / 99.91        & 86.25 / 92.50 / 98.75                     \\ \midrule
LLama3-70B               & 46.87 / 95.23 / 71.05        & 85.00 / \textbf{96.25} / 96.25                     \\
ChatGPT                  & 42.73 / 95.23 / 68.98        & 83.75 / 95.00 / 96.25                     \\
GPT-4o                   & 46.85 / 95. 23 / 70.54       & 87.50 / \textbf{96.25} / 96.25                     \\ \midrule
LUK (COT-ChatGPT)        & 99.95 / 99.87 / 99.91        & 91.25 / 95.00 / \textbf{98.75}                     \\
LUK (COT-GPT4o)          & 99.67 / \textbf{100.0} / 99.83        & 91.25 / 95.00 / \textbf{98.75}                     \\ \midrule
LUK (MEC-LLama3)         & 99.87 / \textbf{100.0} / \textbf{99.93}        & \multicolumn{1}{l}{\textbf{92.50} / 95.00 / \textbf{98.75}} \\
LUK (MEC-ChatGPT)        & 99.95 / 99.91 / 99.93        & \multicolumn{1}{l}{\textbf{92.50} / 95.00 / \textbf{98.75}} \\
LUK (MEC-GPT4o)          & 99.87 / \textbf{100.0} / \textbf{99.93}       & \multicolumn{1}{l}{\textbf{92.50} / \textbf{96.25} / 96.25} \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\begin{table*}[]
\color{blue}
\centering
\caption{Results on MC and LDSM (network device logs).}
\label{tab: network_result-r2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc|cccc}
\toprule[1.5pt]
\multirow{3}{*}{Methods} & \multicolumn{4}{c|}{MC (Accuracy / Weighted F1)}                                   & \multicolumn{4}{c}{LDSM (Accuracy / Weighted F1)}                                  \\ \cmidrule{2-9} 
                         & \multicolumn{2}{c|}{Cisco}                         & \multicolumn{2}{c|}{Huawei}   & \multicolumn{2}{c|}{Cisco}                         & \multicolumn{2}{c}{Huawei}    \\
                         & Switches      & \multicolumn{1}{c|}{Routers}       & Switches      & Routers       & Switches      & \multicolumn{1}{c|}{Routers}       & Switches      & Routers       \\ \midrule
CNN                      & 56.89 / 56.85 & \multicolumn{1}{c|}{57.46 / 54.92} & 74.52 / 73.95 & 72.78 / 72.23 & 84.04 / 84.04 & \multicolumn{1}{c|}{80.99 / 80.99} & 86.05 / 86.05 & 82.37 / 82.30 \\
BiLSTM                   & 55.74 / 55.63 & \multicolumn{1}{c|}{57.17 / 56.76} & 76.52 / 75.49 & 73.96 / 73.30 & 89.45 / 89.44 & \multicolumn{1}{c|}{85.42 / 85.41} & 87.85 / 87.85 & 84.43 / 84.40 \\
BERT                     & 62.67 / 61.38 & \multicolumn{1}{c|}{62.72 / 62.60} & 82.37 / 81.20 & 81.18 / 79.20 & 93.06 / 93.06 & \multicolumn{1}{c|}{90.01 / 90.00} & 93.18 / 93.18 & 90.06 / 90.05 \\
Biglog                   & 62.69 / 62.76 & \multicolumn{1}{c|}{63.15 / 61.17} & 83.24 / 83.25 & 82.36 / 81.19 & 93.32 / 93.32 & \multicolumn{1}{c|}{91.46 / 91.46} & 94.19 / 94.19 & 93.62 / 93.61 \\
KnowLog                  & 63.33 / 63.35 & \multicolumn{1}{c|}{63.65 / 63.12} & 84.11 / 83.65 & 83.55 / 82.41 & 95.05 / 95.05 & \multicolumn{1}{c|}{92.78 / 92.78} & 97.15 / 97.15 & 96.43 / 96.43 \\ \midrule
T5-KD                    & 62.96 / 62.36 & \multicolumn{1}{c|}{63.86 / 61.01} & 83.60 / 83.23 & 83.55 / 82.82 & 95.29 / 95.28 & \multicolumn{1}{c|}{93.20 / 93.20} & 95.25 / 95.25 & 93.97 / 93.97 \\ \midrule
LLama3-70B               & 61.61 / 60.95 & \multicolumn{1}{c|}{62.99 / 60.55} & 82.98 / 82.83 & 81.66 / 80.34 & 84.48 / 84.31 & \multicolumn{1}{c|}{88.32 / 88.24} & 95.49 / 95.49 & 95.57 / 95.57 \\
ChatGPT                  & 57.11 / 54.41 & \multicolumn{1}{c|}{57.99 / 54.56} & 79.14 / 77.19 & 78.22 / 75.51 & 82.14 / 81.96 & \multicolumn{1}{c|}{84.64 / 84.47} & 85.75 / 85.75 & 90.31 / 90.22 \\
GPT-4o                   & 62.12 / 61.62 & \multicolumn{1}{c|}{63.86 / 61.01} & 83.25 / 82.80 & 81.30 / 79.87 & 89.04 / 88.99 & \multicolumn{1}{c|}{93.12 / 93.11} & 97.23 / 97.23 & \textbf{97.79} / \textbf{97.79} \\ \midrule
LUK (COT-ChatGPT)        & 63.49 / 63.72 & \multicolumn{1}{c|}{64.51 / 63.33} & 83.42 / 82.70 & 83.19 / 82.34 & 94.93 / 94.92 & \multicolumn{1}{c|}{93.11 / 93.11} & 96.33 / 96.33 & 95.73 / 95.73 \\
LUK (COT-GPT4o)          & 63.47 / 63.51 & \multicolumn{1}{c|}{63.61 / 63.02} & 83.60 / 83.20 & 82.84 / 81.92 & 94.92 / 94.91 & \multicolumn{1}{c|}{93.18 / 93.18} & 96.46 / 96.46 & 95.93 / 95.93 \\ \midrule
LUK (MEC-LLama3)         & 65.67 / 65.27 & \multicolumn{1}{c|}{66.67 / 65.12} & 85.25 / 84.95 & 85.21 / 84.01 & 96.45 / 96.45 & \multicolumn{1}{c|}{94.13 / 94.13} & 97.66 / 97.66 & 97.39 / 97.39 \\
LUK (MEC-ChatGPT)        & 65.54 / 65.12 & \multicolumn{1}{c|}{66.29 / 64.27} & 84.64 / 84.47 & 85.09 / 83.82 & 96.32 / 96.32 & \multicolumn{1}{c|}{93.80 / 93.80} & 96.92 / 96.92 & 96.74 / 96.74 \\
LUK (MEC-GPT4o)          & \textbf{66.16} / \textbf{66.02} & \multicolumn{1}{c|}{\textbf{67.20} / \textbf{65.41}} & \textbf{85.51} / \textbf{85.26} & \textbf{85.33} / \textbf{84.73} & \textbf{96.63} / \textbf{96.63} & \multicolumn{1}{c|}{\textbf{94.32} / \textbf{94.32}} & \textbf{97.66} / \textbf{97.66} & 97.34 / 97.34 \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table*}


\begin{table}[]
\color{blue}
\centering
\caption{Results on  LPCR and FPI (network device logs). Note: The results of proprietary LLMs on the FPI task cannot be compared due to data privacy issues.}
\label{tab: network_result2-r2}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|c}
\toprule[1.5pt]
\multirow{3}{*}{Methods} & \multicolumn{2}{c|}{LPCR (Precision@1 / 3 / MRR)} & FPI (Accuracy) \\ \cmidrule{2-4} 
                         & \multicolumn{2}{c|}{Huawei}                       & Huawei         \\
                         & Switches                & Routers                 & Switches       \\ \midrule
CNN                      & 54.30 / 77.26 / 67.99   & 53.45 / 75.77 / 67.35   & 69.00          \\
BiLSTM                   & 59.27 / 78.04 / 71.22   & 51.45 / 69.56 / 63.76   & 74.83          \\
BERT                     & 76.18 / 91.54 / 84.70   & 72.57 / 91.59 / 82.61   & 88.75          \\
Biglog                   & 83.33 / 94.02 / 89.38   & 82.98 / 95.59 / 89.49   & 89.58          \\
KnowLog                  & 87.50 / 93.01 / 91.84   & 89.68 / 96.59 / 93.99   & 94.17          \\ \midrule
T5-KD                    & 86.11 / 93.56 / 91.41   & 84.48 / 92.59 / 90.33   & -              \\ \midrule
LLama3-70B               & \textbf{95.61} / \textbf{98.04} / \textbf{97.27}   & \textbf{97.48} / \textbf{99.49} / \textbf{98.52}   & 88.83          \\
ChatGPT                  & 90.95 / 95.11 / 93.88   & 97.20 / 98.34 / 98.19   & -              \\
GPT-4o                   & 95.65 / 98.29 / 97.27   & 97.39 / 99.09 / 98.47   & -              \\ \midrule
LUK (COT-ChatGPT)        & 85.18 / 95.03 / 90.55   & 84.58 / 95.99 / 90.64   & 90.42          \\
LUK (COT-GPT4o)          & 86.34 / 93.79 / 91.37   & 87.88 / 95.19 / 92.75   & 92.50          \\ \midrule
LUK (MEC-LLama3)         & 90.45 / 95.81 / 94.06   & 90.49 / 96.99 / 94.52   & 95.83          \\
LUK (MEC-ChatGPT)        & 89.37 / 95.19 / 93.43   & 88.48 / 94.69 / 90.33   & 93.33          \\
LUK (MEC-GPT4o)          & 90.92 / 96.04 / 94.46   & 90.69 / 96.09 / 94.39   & \textbf{96.67}          \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\uline{Follow your suggestions, (1) we supplement the comparison of knowledge distillation in the introduction of the revised manuscript.
(2) we add the existing distillation technique as the baseline in the experiments. Details are as follows:}
\begin{enumerate}
    \item \uline{\textbf{Section I, Page 2:}} \textcolor{blue}{In addition, in the
era of LLMs, knowledge distillation (KD) [44] emerges as
a pivotal methodology for transferring advanced capabilities
from LLMs to smaller models. Compared to obtaining answers
directly from the teacher’s model, distillation towards the
reasoning process has proved to be a more effective method
[44, 45]. However, current knowledge distillation methods,
such as COT-based KD [46, 47], struggle to acquire the expert
knowledge, instead imitating the teacher’s reasoning forms and
ignoring the premise that reasoning requires expert knowledge.
These distillation methods, which emphasize the process of reasoning
and outcome, still hardly compensates for the lack of expert
knowledge.}
    \item \uline{\textbf{Section IV.D.3), Page 10:}} \textcolor{blue}{
    Knowledge distillation methods: In the era of LLMs,
data augmentation (DA) is the prevalent paradigm to achieve
knowledge distillation of LLMs, where it prompts the LLM to
generate more data tailored to train the student model in a targeted
skill or domain [85, 44]. This reasoning process-oriented
distillation method is more effective compared to obtaining
labels directly from the teacher model [45]. Considering the
lack of research on knowledge distillation in the field of log
analysis, we select Chain-of-Thought (COT)-based knowledge
distillation as the baseline, which has proven to be an effective
knowledge distillation method for the reasoning process in the
field of NLP [46, 47].} \\
    \textcolor{blue}{Specifically, we select T5 [86] (t5-base with 223M parameters) as the student model, and GPT-4o as the teacher model.
Given the specific log analysis task, we provide the inputs
and labels from the training set to the teacher model, then
utilize COT prompting to extract rationales from the teacher
model. Finally, the student model is trained with the inputs
and constructed rationales.}
    \item \uline{\textbf{Section IV.E.1), Page 11:}} \textcolor{blue}{
In comparison to the knowledge distillation-based method
(T5-KD), the chain-of-thought knowledge distillation approach
exhibited suboptimal performance in specific log analysis
tasks. This disparity can be attributed to the unique
nature of log analysis, which typically necessitates a deep
understanding of domain-specific knowledge. The chain-of-thought
methodology, with its sequential reasoning framework,
may inadvertently introduce noise or overlook the analysis
of pertinent background knowledge crucial for these tasks,
leading to diminished performance in tasks where precise
understanding and retention of domain-specific information
are crucial. In comparison, LUK prioritizes the construction of
high-quality domain knowledge explicitly before fine-tuning
it for specific tasks. By establishing a strong foundation of
domain-specific knowledge upfront, LUK is better positioned
to address the intricate nuances inherent in log analysis tasks.}
\end{enumerate}

\textbf{C3:} Regarding Section 2 related work and motivation, I would kindly ask the authors to adjust the title (if possible, the organization of the content) of the subsection, as the current titles “Pretraining on language models” \& “large language model” are irrelevant to the log understanding.

\textbf{R3:} Many thanks for your suggestions. We have adjusted the title and content of the related work. Specifically, the related work is discussed according to two paradigms: log analysis based on pre-trained language models and large language models. In the current revised manuscript, the two titles of the related work are: \textit{1) Pre-trained Language Models for Log Analysis}, \textit{2) Large Language Model for Log Analysis}. 

\uline{Follow your suggestions, We adjust the title and content of the related work. Details are as follows:}
\begin{enumerate}
    \item \uline{\textbf{Section II.A, Page 3:}} \textcolor{blue}{
    A. Pre-trained Language Models for Log Analysis  } \\
    \textcolor{blue}{In
addition, these pre-trained models rely on the existing Masked
Language Modeling (MLM) as the pre-training task, they
only perceive their own contextual information and are unable
to integrate external knowledge. Although KnowLog also
proposes the abbreviation prediction task, this method cannot
adaptively perceive other knowledge than the abbreviation.
Considering the abundance of knowledge required for log
understanding, hence, we also investigate making the PLM
adaptive in perceiving useful information from the knowledge
during pre-training.}
    \item \uline{\textbf{Section II.B, Page 3:}} \textcolor{blue}{
    A. Large Language Models for Log Analysis  } \\
    \textcolor{blue}{
    Large language models (LLMs), representing a remarkable
advancement in artificial intelligence, have been trained on
diverse corpora, enabling them to generate human-like text and
provide accurate responses to queries [59]. Notably, the recent
introduction of transformative models like ChatGPT and GPT-
4, characterized by their enormous scale and alignment with
human feedback, presents a novel opportunity for enhancing
software engineering tasks [60, 23, 61, 62]. } \\ 
\textcolor{blue}{However, restricted accessibility, higher costs, and computational inefficiency limit the widespread use of LLM in real-world scenarios. For example, the GPT-3 model with
175 billion parameters requires 326GB of GPU memory to
deploy [65]. Given the enormous data volumes produced by
modern software systems daily, the overhead of querying
LLMs, including inference time and network latency, renders
direct application of LLMs for log analysis impractical. In
contrast, small PLMs with smaller parameters are more efficient compared to LLMs [37].}
\end{enumerate}


\textbf{C4:} Regarding the multi-expert collaboration, I have two concerns regarding the specific implementation: \textbf{1)} In algorithm 1, I notice that if the feedback given by the evaluator is not a PASS, then the executor will re-generate the context based on the previously generated content and the feedback. As far as I am concerned, the log would also be necessary to facilitate re-generation, otherwise how is the executor supposed to regenerate based on its wrong output and the binary feedback given by the executor. \textbf{2)} I notice that there is no check regarding the re-generated content. It is possible that the re-generated content still contains the error or introduces new errors, thus an iterative process is necessary until the evaluator deems that the generated content is a pass. I suggest authors to implement an iterative process and add additional the experiments.

\textbf{R4:} Thank you for your suggestions. We respond to the above
two questions as follows:
\begin{enumerate}
    \item The MEC implementation is based on the LLM's conversation interface. In the implementation, each role is passed the content of historical conversations from other roles. Hence, each role explicitly knows the current input log.
    \item Many thanks for your constructive suggestions. We modify the evaluation and refinement mechanisms as the iterative framework. Specifically, as shown in \textcolor{red}{Fig. \ref{fig:multi-expert-r2}} during the collaboration, to rigorously ensure the quality of the generated knowledge, the evaluation and refinement mechanism will be iterative until the content generated by \textit{Executor} meets the evaluation requirement or the maximum number of iterations is reached. We set up 3 iterations to build expert knowledge in our experiments.
\end{enumerate}

\uline{We modify the MEC framework in our revised manuscript. The details are illustrated below:}
\begin{enumerate}
\item We modify the introduction of collaboration in \textbf{Section III.B}. \\
\uline{\textbf{Section III.B.3), Page 5:}} \textcolor{blue}{After constructing evaluation examples and assigning roles to LLMs, different roles start working to collaborate and interact according to the requirements in the prompt. 
First, the \textit{Director} meticulously analyzes the input logs to discern key points and formulates a plan for comprehending the logs effectively. Subsequently, the \textit{Director} shares these insights with the \textit{Executor} to guide the content generation process. The \textit{Executor} utilizes these key points to create detailed content that aligns with the requirements.
Finally, the detailed content produced by the \textit{Executor} undergoes evaluation by the \textit{Evaluator} to assess its quality. If the content meets the evaluation requirement, it is directly output as expert knowledge. In cases where the evaluation result is unsatisfactory and improvements are needed, the \textit{Evaluator} provides feedback to the \textit{Executor} for refinement.  To rigorously ensure the quality of the generated knowledge, this evaluation and refinement mechanism will be iterative until the content generated by \textit{Executor} meets the evaluation requirement or the maximum number of iterations is reached. We set up 3 iterations to build expert knowledge in our experiments. The pseudocode of the multi-expert collaboration framework is outlined in \textcolor{red}{Algorithm \ref{alg:algorithm2}}.
} \\
\textcolor{blue}{ This collaborative framework manifests two pivotal advantages:
Firstly, leveraging multiple roles' collective insights and skills enables a multi-perspective analysis of the input log, 
thereby mitigating the one-sidedness and bias inherent in a single model's response acquiring more professional expert knowledge. 
Secondly, through the feedback loop mechanism, the framework enables iterative refinement of content. This iterative process of evaluation, feedback incorporation, and content enhancement promotes continuous improvement, thereby ensuring that the expert knowledge acquired is comprehensive and of high quality.}
\end{enumerate}

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{Fig/expert-framework.pdf}
   \vspace{-3mm}
   \caption{\textcolor{blue}{Framework of multi-expert collaboration, which consists of three experts. First, the \textit{Director} meticulously analyzes the input logs to discern key points. Subsequently, the \textit{Executor} utilizes these key points
to create detailed content. Finally, the \textit{Evaluator} evaluates the quality of the generated content. In cases where the evaluation result is unsatisfactory and improvements are needed, the \textit{Evaluator} provides feedback to the \textit{Executor} for refinement. }}
   \vspace{-3mm}
   \label{fig:multi-expert-r2}
\end{figure*}


\begin{algorithm}
\caption{\textcolor{blue}{Pseudocode of multi-expert collaboration.}}
\label{alg:algorithm2}
\begin{algorithmic}
\REQUIRE \textcolor{blue}{Input Log $log$, LLM $\mathcal{M}$, Example Knowledge   $K_{pos}$}      %输入条件
\ENSURE \textcolor{blue}{Output Expert Knowledge $k$}
\STATE \textcolor{gray}{\# Construct Contrastive Examples}
\FOR{\textcolor{blue}{$c = 1$ to $C$}}
    \STATE \textcolor{blue}{$K_{neg}^c = \mathcal{M}(Prompt_{Modify}, K_{pos})$}
\ENDFOR
\STATE  \textcolor{blue}{$K_{examples} = K_{pos} \cup \{K_{neg}\}_{c=1} ^ C $}
\STATE \textcolor{gray}{\# Initial Roles}
\STATE $\mathcal{DIRECTOR} = Init\_Role(Prompt_{Dirctor}, \mathcal{M}) $
\STATE $\mathcal{EXECUTOR} = Init\_Role(Prompt_{Executor}, \mathcal{M}) $
\STATE \textcolor{blue}{$Prompt_{Evaluator} = Prompt_{Evaluator}.join(K_{examples})$}
\STATE \textcolor{blue}{ $\mathcal{EVALUATOR} = Init\_Role(Prompt_{Evaluator},  \mathcal{M})$}
\STATE \textcolor{gray}{\# Collaboration}
\STATE \textcolor{blue}{Init: $epoch = 0, feedback = False$}
\STATE $ keypoint = \mathcal{DIRECTOR}(log) $
\STATE $ content = \mathcal{EXECUTOR}(log, keypoint) $
\REPEAT
\STATE \textcolor{blue}{$ epoch = epoch + 1$}
\STATE \textcolor{blue}{$ feedback = \mathcal{EVALUATOR}(log, keypoint, content) $}
\IF{\textcolor{blue}{$feedback == False$}}
\STATE \textcolor{blue}{$ content = \mathcal{EXECUTOR}(content, feedback) $}
\ENDIF
\UNTIL{\textcolor{blue}{$epoch == Epoch$ or $feedback==True$}}
\STATE $k = content$
\RETURN $k$
\end{algorithmic}
\end{algorithm}


\textbf{C5:} Regarding the pretraining, I see two encoders in figure 4. I am wondering whether they are two separate BERTs or one BERT but run two times sequentially. If they are two separate BERTs, how do authors conduct the following finetuning? More clarifications are needed.

\textbf{R5:} We apologize for the unclear description of the model architecture. To encode each type of data separately, we adopt the bi-encoder architecture where two encoders are initialized with the same pre-trained model. Specifically, during pre-training, we run two identical encoders to encode logs and knowledge within the same pair, respectively.  During fine-tuning, this pre-trained log encoder is used as the backbone.

\uline{Following your suggestion, we clarify the model architecture in \textbf{Section III.C, Page 5}}:
\begin{itemize}
    \item \uline{\textbf{Section III.C, Page 5:}} The input of the pre-training framework is a batch of pairs consisting of logs and the corresponding expert knowledge, then these pairs are fed into two encoders to obtain log representations and knowledge representations through two encoders respectively, \textcolor{blue}{where two encoders are initialized with the same pre-trained model. } 
\end{itemize}

\textbf{C6:} Regarding the experiments, one critical shortcoming is the lack of the LLM-based log understanding baselines [26-30]. Why do authors exclude them in the experiments? Besides, the authors mention that “considering that ICL suffers from unstable results …, we utilize zero-shot capability of LLMs for log analysis.” I suggest authors to also experiment with the most simplified example selection strategy (e.g., BM 25 similarity, random selection).

\textbf{R6:} We apologize for the non-rigorous presentation and experiments. With the improvement of LLM's capabilities and deeper research, in-context-learning (ICL)-based log analysis shows excellent performance. 

Experimentally, following previous LLM-based log analysis works \cite{xu2024divlog,xu2024unilog,liu2023logprompt,jiang2023llmparser}, we select top-5 similar examples from the training set for each input log and use \textit{bge-large-en-v1.5} as the embedding model to select examples, due to its excellent performance among all open-source embedding models. Considering the recency bias of LLMs \cite{zhao2021calibrate}, we arrange these examples in ascending order based on the cosine similarity. We select two proprietary LLMs (\textbf{ChatGPT} and \textbf{GPT-4o}) and one powerful open-source LLM (\textbf{LLama3-70B \cite{dubey2024llama}}) as baselines.
As shown in \textcolor{red}{Table \ref{tab: software_results-r2} and \ref{tab: network_result2-r2}}, our results show that apart from LDSM and LPCR tasks, three LLMs perform weaker than the fine-tuned smaller PLMs. This disparity can be ascribed to the presence of a significant domain gap, which hampers the ability of LLMs to effectively address specialized tasks directly.


\uline{Following your suggestions,  we take the LLM following the ICL paradigm as the baseline. The details are illustrated as follows:}
\begin{enumerate}
    \item \uline{ \textbf{Section IV.D, Page 10:}} \textcolor{blue}{LLM-based log analysis methods follow the \textit{in-context learning} paradigm, where LLMs make predictions based on contexts augmented with a few examples without training.
Following previous LLM-based log analysis works [26,27,28,29], we select top-5 similar examples from the training set for each input log and use \textit{bge-large-en-v1.5} as the embedding model to select examples, due to its excellent performance among all open-source embedding models. Considering the recency bias of LLMs [87]{zhao2021calibrate}, we arrange these examples in ascending order based on the cosine similarity. We select two proprietary LLMs (\textbf{ChatGPT} and \textbf{GPT-4o}) and one powerful open-source LLM (\textbf{LLama3-70B [79]}) as baselines. We utilize HTTP requests to invoke the OpenAI APIs and interact with proprietary LLMs. For open-source LLM, we deploy \textit{Llama-3.3-70B-Instruct} in our environments to analyze logs.}

\item \uline{\textbf{Section IV.E.RQ1), Page 11:}} \textcolor{blue}{In comparison to LLMs, our results show that apart from
LDSM and LPCR tasks, three LLMs perform weaker than
the fine-tuned smaller PLMs. This disparity can be ascribed
to the presence of a significant domain gap, which hampers
the ability of LLMs to effectively address specialized tasks
directly. Consequently, this limitation restricts their potential
to fully exploit the wealth of knowledge they encapsulate.
It underscores the necessity for more nuanced approaches to
task-specific analysis and demonstrates the effectiveness of our
strategy of extracting knowledge from LLMs before reasoning directly to bridge these critical gaps in performance. Furthermore,
our findings suggest that GPT4o-based enhancement
outperforms the other two LLMs on most datasets, indicating
the potential of leveraging stronger LLMs to significantly
enhance the effectiveness and performance of smaller models
in various tasks.}
\end{enumerate}

\textbf{C7:} Besides, I find the performance of LUK (COT-ChatGPT) and LUK (MEC-ChatGPT) is very close expect when the labeled logs are extremely limited. \textbf{(1)} I suggest authors to enrich the experiments under the limited labeled data scenario, as this is the application scenario where the superiority of LUK lies. 
\textbf{(2)} Also, it would be better to show the ratio and examples of knowledge outputs that are first rejected by the executor and regenerated, in order to better demonstrate the necessity of incorporating MEC (which in essential adds a self-check process over the raw COT).

\textbf{R7:} Thank you for your suggestions. We respond to the above
two questions as follows:
\begin{enumerate}
    \item We enrich the more log analysis tasks to evaluate the effectiveness of LUK in low-resource
tasks, characterized by limited annotations. As shown in \textcolor{red}{Fig. \ref{fig:low-resource-results-r2}}, LUK achieves outstanding performance in low-resource scenarios.
In addition, we make the following improvements to the original framework in this revised manuscript, making the latest experimental results gain an improvement over the previous version on all datasets, including: i) Constructing the
contrastive examples to improve the Evaluator’s evaluation capability under the challenging reference-free setting; and ii) Constructing the evaluation and refinement
mechanisms as the iterative framework. 
    \item We first statistics the proportion of unsatisfactory knowledge in each iteration, and then verify the performance of the refined knowledge based on the evaluation feedback each time in \textcolor{red}{Fig. \ref{fig:roundn-r2}}. Second, we provide a case analysis in \textcolor{red}{Fig. \ref{fig:evaluation_case-r2}} to intuitively analyze the impact of the evaluation and refinement mechanism on knowledge generation. Third, we count the distributions of different error categories in unsatisfactory knowledge according to \textit{Evaluator}’s results for GPT-4o and LLama3-70B, respectively. As shown in \textcolor{red}{Fig. \ref{fig:different_error_precent-r2}}, it can be found that a significant portion of the inadequacies stems from issues related to completeness. 
\end{enumerate}

\begin{figure*}[]
    \centering
    % \vspace{-2mm}
    \subfloat[Anomaly Detection (BGL)]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_BGL.pdf}}
    \subfloat[LDSM (Huawei-Security)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_ldsm.pdf}}
    \subfloat[Fault Phenomenon Identification]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_fpi.pdf}}
    \caption{\textcolor{blue}{Results on different ratios of the training dataset.}}
    
    % \vspace{-5mm}
    \label{fig:low-resource-results-r2}
\end{figure*}

\begin{figure*}[]
    \centering
    % \vspace{-2mm}
    \subfloat[Anomaly Detection (BGL)]{\label{fig: roundaaa}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/error_round_percent.pdf}}
    \subfloat[MC (Huawei-Switches)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/mc_roundn.pdf}}
    \subfloat[LDSM (Huawei-Switches)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/ldsm_roundn.pdf}}
    \caption{\textcolor{blue}{Figure (a) shows the proportion of unsatisfactory knowledge in each iteration. Figure (b) and (c) show the results of the refined knowledge based on the evaluation feedback each time.}}
    
    % \vspace{-5mm}
    \label{fig:roundn-r2}
\end{figure*}

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{new_fig/luk_evaluation_example.pdf}
   % \vspace{-6mm}
   \caption{\textcolor{blue}{An complete workflow of the MEC framework to construct knowledge.}}
   % \vspace{-4mm}
   \label{fig:evaluation_case-r2}
\end{figure*}

\begin{figure}[]
    \centering
    % \vspace{-2mm}
    \subfloat[GPT-4o]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.5\linewidth]{new_fig/error_percent_gpt4o.pdf}}    
    \subfloat[LLama3-70B]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.5\linewidth]{new_fig/error_percent_llama3.pdf}}
    
    \caption{\textcolor{blue}{Distributions of error categories in unsatisfactory knowledge.}}
    
    % \vspace{-5mm}
    \label{fig:different_error_precent-r2}
\end{figure}

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{new_fig/luk_evaluation_examples.pdf}
   \vspace{-3mm}
   \caption{\textcolor{blue}{The contrastive samples constructed in our experiments, where Example 1 represents the positive example, and the remaining three examples are negative examples obtained from the modification of GPT-4o. Colour-marked text indicates that the evaluation requirements are unsatisfied. }}
   \vspace{-3mm}
   \label{fig:evaluation-r2}
\end{figure*}

\uline{Following your suggestions, our main revisions are as follows:}
\begin{enumerate}
    \item We supplement the low-resource experiments in \textbf{Section IV.E.RQ4, Page 14:} \\ 
    \uline{\textbf{Section IV.E.RQ4, Page 14:}} \textcolor{blue}{In real-world scenarios, acquiring a considerable quantity of
annotated samples is difficult [12, 23], thereby presenting a
significant obstacle to the efficacy of automated log analysis
models. To assess the effectiveness of LUK in low-resource
tasks, characterized by limited annotations, we conduct experiments
on Anomaly Detection, Log and Description Semantic
Matching, and Fault Phenomenon Identification with different
ratios of training datasets.} \\
\textcolor{blue}{The experimental results are shown in Fig. 8, considering
that knowledge distillation based on fewer samples are difficult
to train, we do not compare with T5-KD. We find that
with the reduction of training samples, the performance of
various models exhibits a decline, with BERT and Biglog
demonstrating a particularly significant downward trend in the
LDSM and FPI tasks, and KnowLog showing a significant
decrease on the AD task. On the other hand, LUK based
on MEC achieves optimal results by fine-tuning the models
with different proportions of annotated samples. Specifically,
on the AD task, compared to the full data, LUK drops only
1.03\% in the F1-value with 1\% of the training data. And on
the FPI task, LUK’s Accuracy drops by only 13.2\% with 30\%
of the training data, while BERT and Biglog drop by 31.45\%
and 31.25\%, respectively. This demonstrates that LUK gains
expert knowledge from LLM, which helps to compensate for
the shortcomings of the smaller pre-trained model when less
annotated data is available. Models with restricted knowledge
struggle to excel in scenarios with limited resources, highlighting
the significance of leveraging knowledge to mitigate
the need for extensive annotation and enhance performance
in data-scarce environments. KnowLog primarily relies on
knowledge extracted from documentation, which may be limited
in scope and quality, especially in low-resource settings.
In contrast, this proves that knowledge acquired by the LLM
has a wider scope and can provide a more comprehensive
and diverse range of information, rather than being limited to
some specific documentation.} \\
\textcolor{blue}{In summary, LUK achieves outstanding performance in low-resource scenarios, which stems from its ability to leverage
expert knowledge acquired from LLMs, effectively compensating for the constraints of smaller PLMs when annotated data
availability is restricted. By strategically harnessing this expert
knowledge, LUK enables the development of efficient and
accurate models even in resource-constrained environments,
showcasing its adaptability and effectiveness in challenging
log analysis tasks.}
    \item We add the ablation studies of the iterative mechanism in \textbf{Section IV.F, Page 15:} \\
    \uline{\textbf{Section IV.F, Page 15:}} \textcolor{blue}{To verify the performance of the iterative evaluation and
refinement mechanism, we first statistics the proportion of
unsatisfactory knowledge in each iteration, and then verify the
performance of the refined knowledge based on the evaluation
feedback each time on the MC and LDSM tasks, where we set
up 3 iterations in our experiment. As shown in Fig. 10, we can
find a consistent decline in the proportion of unsatisfactory
knowledge with each successive iteration. Simultaneously,
the performance of the enhanced model exhibits steady improvement,
underscoring the positive impact of the iterative
evaluation and refinement mechanism within the framework.
Notably, our observations indicate that a significant portion
of knowledge refinement occurs following the initial feedback
round, with subsequent iterations primarily focusing on refining
a smaller fraction of the knowledge. To save costs, we
suggest that the framework can iterate one time as a cost-effective
strategy, effectively balancing performance gains with
resource optimization.}
    \item We add the case analysis of the MEC framework in \textbf{Section V.B.1), Page 16:} \\
    \uline{\textbf{Section V.B.1), Page 16:}} \textcolor{blue}{1) Evaluation and refinement mechanism of the MEC
framework: To intuitively understand the workflow of the
MEC framework and analyze the impact of the evaluation and
refinement mechanism on knowledge generation, we provide
a specific case of expert knowledge construction as shown in Fig. 11, this input log from the Huawei device.
As can be seen from the case, the Director first meticulously
analyzes the input log to give key points, and then the Executor
generates expert knowledge based on the guidance of these key
points. Following knowledge creation, the Evaluator evaluates
the quality of the generated knowledge and provides feedback
to the Executor for refinement. The evaluation feedback shows
that the content generated by the Executor does not fulfill
completeness and consistency. Specifically, the generated
knowledge lacks of an introduction to the procedure step and
the explanation of the severity level is not rigorous. In addition,
there is also an uninformative explanation in the generated
knowledge, which makes it more difficult for the smaller
model to understand the expert knowledge. Finally, the Executor
refines the generated knowledge based on the evaluation
feedback. From the re-generated knowledge, we can find that
the Executor not only supplements the clear introduction of the
procedure step but also modifies the explanation of severity
level to make it more reasonable. Overall, the re-generated
knowledge is more comprehensive and rigorous, which is more
conducive for the smaller model to learn expert knowledge.
To more deeply reveal the issues of knowledge generated by
LLMs. We count distributions of different error categories in
unsatisfactory knowledge according to Evaluator’s results for
GPT-4o and LLama3-70B, respectively. As shown in Fig. 12,
it can be found that a significant portion of the inadequacies
stems from issues related to completeness. The prevalence of completeness-related errors underscores the challenge faced
by the single LLM in producing comprehensive knowledge
autonomously. Moreover, alongside completeness issues, a
smaller yet notable proportion of unsatisfactory knowledge is
attributed to deficiencies in conciseness and consistency. This
finding underscores the significance of collaborative frameworks
that integrate diverse roles, each contributing unique
perspectives and expertise to compensate for the capacity
deficiencies of the single LLM and improve the completeness
and accuracy of generated knowledge.}

\item We add the introduction of contrastive examples in \textbf{Section III.B}. \\
\uline{\textbf{Section III.B.2), Page 4-5:}} \textcolor{blue}{LLM Hallucinations
seriously affect the accuracy and quality of outputs
[70, 71]. Given the propensity of LLM-generated content to
exhibit deficiencies in comprehensiveness and informativeness,
ensuring the superior quality of directly generated knowledge
poses a significant challenge. To mitigate the hallucination of
LLM and ensure the quality of expert knowledge, we build the role of an Evaluator in the MEC framework and define
three evaluation aspects to evaluate the quality of generated
knowledge automatically, which encourages the LLM to actively
seek more detailed suggestions from the self-evaluation
before delivering a formal response. However, the MEC
framework runs under the challenging reference-free setting
and the evaluation requirements cannot be directly quantified
through metrics, the LLM tends to generate ambiguous and inconsistent
evaluations without fine-grained distinguishability,
causing unsatisfactory evaluation performance [72, 73].} \\
\textcolor{blue}{To address the evaluation weaknesses of the LLM, we
provide evaluation examples as the reference in the Evaluator
prompt. By providing specific examples, the Evaluator uses
them as the basis for evaluation, thus better steering the
evaluation of LLMs towards our desired goals. Considering
that the single type of example makes the LLM biased,
motivated by contrastive learning techniques [74, 75], we construct
contrastive examples consisting of positive and negative
knowledge of the same log to Evaluator as reference examples,
where the positive example showcases the desired knowledge,
while the negative example highlights the unsatisfactory
knowledge that should be avoided. By analyzing both types of
examples before generating the evaluation, the Evaluator can
reason about our evaluation requirements and make a more
informed decision about how to evaluate.} \\
\textcolor{blue}{
Specifically, we select one log $L$ with high-quality knowledge $K_{pos}$ as the positive example, which can be manually constructed by experts or generated from the LLM and manually confirmed. Considering that negative examples $\{K_{neg}\}_{c=1} ^ C, C=3$ of the log $L$ are unavailable directly, to construct the negative examples automatically, we propose to prompt the LLM to modify the positive knowledge making it unsatisfactory for evaluation.
As shown in Fig. 4, we first give the background in the prompt and then clarify the task of modifying knowledge for the LLM, where we can specify which evaluation metrics are not fulfilled. Next, we provide the raw log, the raw positive knowledge, the key points, and the three evaluation requirements in the prompt.
Finally, we require the LLM to give the reason for not fulfilling the evaluation requirements while generating the modified content, which not only improves the reasoning ability of the \textit{Evaluator} but also provides guidance for the revision of the content by \textit{Executor}.
In cases where the LLM-generated negative examples do not capture the characteristics we want to avoid, this can be manually checked, and feedback can be given to the LLM to re-generate negative samples. 
To avoid the higher expense of the longer prompt, we construct one positive knowledge and its corresponding three negative knowledge as reference examples to be provided to the \textit{Evaluator}. 
The contrastive examples we constructed in our experiments are in \textcolor{red}{Fig. \ref{fig:evaluation-r2}}.}
\end{enumerate}



==> response/reviewC.tex <==
\section{Response to Reviewer \#3}

\subsection{Original Comments}
\textbf{Public Comments} (these will be made available to the author)

The manuscript presents a knowledge enhancement framework called LUK. LUK begins by eliciting expert knowledge from LLMs and then employs two pre-training tasks (word-level token prediction and sentence-level semantic alignment) to improve the log understanding capabilities of small PLMs. Authors further fine-tuned enhanced PLMs for six downstream log analysis tasks. A comprehensive evaluation demonstrates that PLMs enhanced by LUK outperform baseline models across various log analysis tasks.

\textbf{Strengths}

- Authors conducted a comprehensive evaluation. The large-scale experiments contain over six baselines and six downstream applications.
- The idea of eliciting knowledge from LLMs to enhance the performance of small PLMs sounds interesting.
- Authors made ablation studies to demonstrate the impact of their two key contributions: the MEC framework and the two pre-training tasks.
- Overall, the writing is clear and easy to follow.

\textbf{ Concerns}

- The manuscript is heavily empirical, and some methodology designs lack explanations.
- The experimental design may not be rigorous; some baselines are missing without justification. Additionally, the design raises potential concerns about data leakage.
- Regarding novelty, this manuscript is somewhat incremental compared to KnowLog. The primary distinction is in the acquisition of expert knowledge: whereas KnowLog relies on documentation created by human experts, LUK safes human efforts via LLMs.
- The improvement of MEC seems incremental.

\textbf{ Detailed comments}

Overall, I appreciate the authors' efforts in introducing new pre-trained models to this research area, as well as the extensive evaluation they conducted. However, I have some concerns and questions regarding the novelty and rigor of the work. I hope the revised manuscript will address my questions and concerns effectively.

Concerns on Novelty

- One of the contributions of the manuscript is the design of two pre-training tasks aimed at enhancing pre-training with relevant knowledge. However, KnowLog also proposes similar pre-training tasks. Please discuss the differences between LUK's pre-training tasks and those of KnowLog, as well as the limitations of KnowLog's approach.
- While the proposed MEC framework is novel, its improvement seems incremental, as shown in Tables VII and VIII. For most downstream asks (e.g., Anomaly Detection), the performance differences between using COT prompting to elicit expert knowledge (LUK (COT-ChatGPT)) and the MEC framework (LUK (MEC-ChatGPT)) are small. In some cases, the MEC framework even performs worse than COT prompting; for instance, in Table VIII, for the MC-Cisco-Routers task, LUK (COT-ChatGPT) outperforms LUK (MEC-ChatGPT) by 0.2%. Could the authors clarify the significance and effectiveness of the MEC framework in eliciting expert knowledge compared to COT prompting?


Concern on Rigor

- In the MEC framework, although outputs from Executors are evaluated by Evaluators, the correctness of outputs from both Evaluators and Directors is not guaranteed. Moreover, after receiving the feedback from the Evaluator, the new content generated by the Executor is directly outputted without a correctness check. Given that the MEC framework is crucial for pre-training, ensuring the correctness of its outputs is essential, or at least, MEC's output correctness should be evaluated. Although the manuscript made a qualitative analysis of two examples, my question is: How often does the MEC framework extract correct knowledge, and how often does MEC extract incorrect knowledge?

- The key idea behind word-level token prediction is the knowledge perception module (KPM), which calculates the weights of each token in a given knowledge. However, the attention mechanism also adjusts the weights of tokens within the knowledge. These two objectives appear to overlap. Could the authors explain why using the attention mechanism alone is insufficient and why the additional KPM module is necessary?

- The manuscript lacks a detailed description of datasets used for pre-training, fine-tuning, and evaluating each downstream task. Specifically, RQ2 states, "In this RQ, ... we conduct experiments on downstream tasks beyond the pre-training logs." Does this imply that the evaluation dataset used in RQ1 will also be included in the pre-training and fine-tuning processes?

- If the evaluation dataset is included in the pre-training or fine-tuning steps, could this design introduce data leakage issues?

- Please provide the time required for pre-training and fine-tuning a PLM using the LUK framework.

- Although KnowLog can only pre-train PLMs on a limited set of logs with documentation, it would be better if the manuscript could include KnowLog's performance in Tables VII and VIII. Since KnowLog's pipeline is quite similar to that of LUK, understanding the performance differences between these two tools can better illustrate the contributions of LUK.

- RQ1 states, "Comparing MEC with COT, MEC demonstrates superior performance." However, my reading of the experiments is the opposite: MEC appears to provide only marginal improvements and, in some cases, even performs worse, as indicated in Tables VII and VIII. To what extent do you believe the improvements offered by MEC are sufficient?

Tables and Figures in the Experiments section miss some baselines or datasets. I hope authors can explain the following in the revised manuscript:
- In Table II, some datasets (ThunderBird, Spirit) are not included in the pre-training phase.
- In RQ1, FPI is not included.
- RQ3 does not include LUK (COT-ChatGPT). Since LUK-COT achieves a very comparable performance against LUK (MEC-ChatGPT), I am curious about its performance. Thus I am wondering why it is not included in RQ3?

- Regarding LUK (MEC-ChatGPT)'s performance on the MC-Huawei-Routers task, there is an inconsistency between Table XII (83.43/82.49) and Table VIII (83.55/82.41). Please double-check and resolve the inconsistency.


Comments on Presentation
Overall, the writing is clear. Here are a few minor issues:

Page 4: Are 'background knowledge' and 'expert knowledge' the same in Section III.C? If so, please make them consistent.
Page 7: this sentence is difficult to parse:
'where the input is a log as a query and an answer candidate set and the output is the ranking result.'

\subsection{Comments and Responses}

\textbf{Response:} We sincerely appreciate the reviewer for the detailed comments, which are helpful to improve our work. The manuscript has been carefully revised following your advice.

\textbf{C1:} One of the contributions of the manuscript is the design of two pre-training tasks aimed at enhancing pre-training with relevant knowledge. However, KnowLog also proposes similar pre-training tasks. Please discuss the differences between LUK's pre-training tasks and those of KnowLog, as well as the limitations of KnowLog's approach.

\textbf{R1:} Thanks for your comments. First, the major difference between LUK and KnowLog on the pre-training task is the word-level pre-training task. Specifically, KnowLog's abbreviation prediction task only recognizes the abbreviations that are already in the log. It cannot understand other key information within the log's tokens (such as parameters) and cannot perceive useful information from external knowledge to enhance the understanding of domain tokens. While LUK can adaptively perceive useful knowledge to understand tokens in logs, not limited to abbreviations. 

Second, KnowLog’s usage scenarios
are limited as it heavily relies on documentation created by
human experts to acquire knowledge. However, most logs lack professional documentation (e.g. almost unable to find relevant documents for
logs coming from Loghub \cite{zhu2023loghub}) and the manual construction of knowledge is costly and inefficient, which significantly hinders
the availability of the model.
In contrast, this work
addresses more generalized log analysis scenarios where logs
are available without accompanying expert knowledge.

\uline{We supplement the discussion of KnowLog's differences in the revised manuscript. The details are illustrated below:}
\begin{enumerate}
    \item We supplement the discussion in introduction (\textbf{Section I, Page 2:}) \\
    \uline{\textbf{Section I, Page 2:}} \textcolor{blue}{Although KnowLog proposes to acquire expert knowledge
from documentation [22], most logs lack professional documentation (e.g. almost unable to find relevant documents for
logs coming from Loghub [38]) and the manual construction of
knowledge is costly and inefficient, which significantly hinders
the availability of the model.} \\
\uline{\textbf{Section I, Page 2:}} \textcolor{blue}{ In addition, KnowLog proposes an
abbreviation prediction task specialized for log understanding.
However, its ability only to enhance the knowledge of abbreviations in the logs is limited. It cannot adaptively perceive other
important information from the knowledge to understand logs,
such as the parameter knowledge of logs.}
\end{enumerate}


\textbf{C2:} While the proposed MEC framework is novel, its improvement seems incremental, as shown in Tables VII and VIII. For most downstream asks (e.g., Anomaly Detection), the performance differences between using COT prompting to elicit expert knowledge (LUK (COT-ChatGPT)) and the MEC framework (LUK (MEC-ChatGPT)) are small. In some cases, the MEC framework even performs worse than COT prompting; for instance, in Table VIII, for the MC-Cisco-Routers task, LUK (COT-ChatGPT) outperforms LUK (MEC-ChatGPT) by 0.2\%. Could the authors clarify the significance and effectiveness of the MEC framework in eliciting expert knowledge compared to COT prompting?

\textbf{R2:} Thanks for your reminder. First, LLMs
have difficulty in acquiring complete and accurate knowledge
due to hallucination, which may result in not covering all the
depth of knowledge and there may be misunderstandings when
dealing with domain-specific data \cite{mundler2023self,manakul2023selfcheckgpt}. 

Second, our collaborative framework manifests two pivotal advan-
tages: 1), leveraging multiple roles’ collective insights and
skills enables a multi-perspective analysis of the input log,
thereby mitigating the one-sidedness and bias inherent in a
single model’s response acquiring more professional expert
knowledge. 2) the process of evaluation, feedback incorporation, and content refinement promotes improvement of the generate knowledge, thereby ensuring that the expert knowledge acquired is comprehensive
and of high quality.

Third, we apologize for the previous inadequate design. We refined the design of the MEC framework in this revised manuscript from the
following two aspects, including: 1) Constructing the
contrastive examples to improve the \textit{Evaluator}’s eval-
uation capability under the challenging reference-free
setting; and 2) Constructing the evaluation and refinement
mechanisms as the iterative framework. As shown in \textcolor{red}{Table \ref{tab: software_results-r3} and \ref{tab: network_result2-r3}},  after we improve the framework, the latest experimental results gain an improvement over the previous version on all datasets, which is significantly better than the existing baselines.

\begin{table}[]
\color{blue}
\centering
\caption{Results on AD and FI (software system logs).}
\label{tab: software_results-r3}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lc|c}
\toprule[1.5pt]
\multirow{2}{*}{Methods} & AD (Precision / Recall / F1) & FI (Recall@1 / 2 / 3)                     \\
                         & BGL                          & OpenStack                                 \\ \midrule
CNN                      & \textbf{99.95} / 96.06 / 97.97        & 83.75 / 86.25 / 90.00                     \\
BiLSTM                   & \textbf{99.95} / 97.25 / 98.58        & 87.50 / 92.50 / 96.25                     \\
BERT                     & 99.70 / 98.48 / 99.09        & 87.50 / 92.50 / \textbf{98.75}                     \\
Biglog                   & 99.87 / 99.63 / 99.75        & 90.00 / 95.00 / \textbf{98.75}                     \\
KnowLog                  & 99.58 / 98.69 / 99.13        & 82.50 / 92.50 / 96.25                     \\ \midrule
T5-KD                    & 99.87 / 99.56 / 99.91        & 86.25 / 92.50 / 98.75                     \\ \midrule
LLama3-70B               & 46.87 / 95.23 / 71.05        & 85.00 / \textbf{96.25} / 96.25                     \\
ChatGPT                  & 42.73 / 95.23 / 68.98        & 83.75 / 95.00 / 96.25                     \\
GPT-4o                   & 46.85 / 95. 23 / 70.54       & 87.50 / \textbf{96.25} / 96.25                     \\ \midrule
LUK (COT-ChatGPT)        & 99.95 / 99.87 / 99.91        & 91.25 / 95.00 / \textbf{98.75}                     \\
LUK (COT-GPT4o)          & 99.67 / \textbf{100.0} / 99.83        & 91.25 / 95.00 / \textbf{98.75}                     \\ \midrule
LUK (MEC-LLama3)         & 99.87 / \textbf{100.0} / \textbf{99.93}        & \multicolumn{1}{l}{\textbf{92.50} / 95.00 / \textbf{98.75}} \\
LUK (MEC-ChatGPT)        & 99.95 / 99.91 / 99.93        & \multicolumn{1}{l}{\textbf{92.50} / 95.00 / \textbf{98.75}} \\
LUK (MEC-GPT4o)          & 99.87 / \textbf{100.0} / \textbf{99.93}       & \multicolumn{1}{l}{\textbf{92.50} / \textbf{96.25} / 96.25} \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\begin{table*}[]
\color{blue}
\centering
\caption{Results on MC and LDSM(network device logs).}
\label{tab: network_result-r3}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccc|cccc}
\toprule[1.5pt]
\multirow{3}{*}{Methods} & \multicolumn{4}{c|}{MC (Accuracy / Weighted F1)}                                   & \multicolumn{4}{c}{LDSM (Accuracy / Weighted F1)}                                  \\ \cmidrule{2-9} 
                         & \multicolumn{2}{c|}{Cisco}                         & \multicolumn{2}{c|}{Huawei}   & \multicolumn{2}{c|}{Cisco}                         & \multicolumn{2}{c}{Huawei}    \\
                         & Switches      & \multicolumn{1}{c|}{Routers}       & Switches      & Routers       & Switches      & \multicolumn{1}{c|}{Routers}       & Switches      & Routers       \\ \midrule
CNN                      & 56.89 / 56.85 & \multicolumn{1}{c|}{57.46 / 54.92} & 74.52 / 73.95 & 72.78 / 72.23 & 84.04 / 84.04 & \multicolumn{1}{c|}{80.99 / 80.99} & 86.05 / 86.05 & 82.37 / 82.30 \\
BiLSTM                   & 55.74 / 55.63 & \multicolumn{1}{c|}{57.17 / 56.76} & 76.52 / 75.49 & 73.96 / 73.30 & 89.45 / 89.44 & \multicolumn{1}{c|}{85.42 / 85.41} & 87.85 / 87.85 & 84.43 / 84.40 \\
BERT                     & 62.67 / 61.38 & \multicolumn{1}{c|}{62.72 / 62.60} & 82.37 / 81.20 & 81.18 / 79.20 & 93.06 / 93.06 & \multicolumn{1}{c|}{90.01 / 90.00} & 93.18 / 93.18 & 90.06 / 90.05 \\
Biglog                   & 62.69 / 62.76 & \multicolumn{1}{c|}{63.15 / 61.17} & 83.24 / 83.25 & 82.36 / 81.19 & 93.32 / 93.32 & \multicolumn{1}{c|}{91.46 / 91.46} & 94.19 / 94.19 & 93.62 / 93.61 \\
KnowLog                  & 63.33 / 63.35 & \multicolumn{1}{c|}{63.65 / 63.12} & 84.11 / 83.65 & 83.55 / 82.41 & 95.05 / 95.05 & \multicolumn{1}{c|}{92.78 / 92.78} & 97.15 / 97.15 & 96.43 / 96.43 \\ \midrule
T5-KD                    & 62.96 / 62.36 & \multicolumn{1}{c|}{63.86 / 61.01} & 83.60 / 83.23 & 83.55 / 82.82 & 95.29 / 95.28 & \multicolumn{1}{c|}{93.20 / 93.20} & 95.25 / 95.25 & 93.97 / 93.97 \\ \midrule
LLama3-70B               & 61.61 / 60.95 & \multicolumn{1}{c|}{62.99 / 60.55} & 82.98 / 82.83 & 81.66 / 80.34 & 84.48 / 84.31 & \multicolumn{1}{c|}{88.32 / 88.24} & 95.49 / 95.49 & 95.57 / 95.57 \\
ChatGPT                  & 57.11 / 54.41 & \multicolumn{1}{c|}{57.99 / 54.56} & 79.14 / 77.19 & 78.22 / 75.51 & 82.14 / 81.96 & \multicolumn{1}{c|}{84.64 / 84.47} & 85.75 / 85.75 & 90.31 / 90.22 \\
GPT-4o                   & 62.12 / 61.62 & \multicolumn{1}{c|}{63.86 / 61.01} & 83.25 / 82.80 & 81.30 / 79.87 & 89.04 / 88.99 & \multicolumn{1}{c|}{93.12 / 93.11} & 97.23 / 97.23 & \textbf{97.79} / \textbf{97.79} \\ \midrule
LUK (COT-ChatGPT)        & 63.49 / 63.72 & \multicolumn{1}{c|}{64.51 / 63.33} & 83.42 / 82.70 & 83.19 / 82.34 & 94.93 / 94.92 & \multicolumn{1}{c|}{93.11 / 93.11} & 96.33 / 96.33 & 95.73 / 95.73 \\
LUK (COT-GPT4o)          & 63.47 / 63.51 & \multicolumn{1}{c|}{63.61 / 63.02} & 83.60 / 83.20 & 82.84 / 81.92 & 94.92 / 94.91 & \multicolumn{1}{c|}{93.18 / 93.18} & 96.46 / 96.46 & 95.93 / 95.93 \\ \midrule
LUK (MEC-LLama3)         & 65.67 / 65.27 & \multicolumn{1}{c|}{66.67 / 65.12} & 85.25 / 84.95 & 85.21 / 84.01 & 96.45 / 96.45 & \multicolumn{1}{c|}{94.13 / 94.13} & 97.66 / 97.66 & 97.39 / 97.39 \\
LUK (MEC-ChatGPT)        & 65.54 / 65.12 & \multicolumn{1}{c|}{66.29 / 64.27} & 84.64 / 84.47 & 85.09 / 83.82 & 96.32 / 96.32 & \multicolumn{1}{c|}{93.80 / 93.80} & 96.92 / 96.92 & 96.74 / 96.74 \\
LUK (MEC-GPT4o)          & \textbf{66.16} / \textbf{66.02} & \multicolumn{1}{c|}{\textbf{67.20} / \textbf{65.41}} & \textbf{85.51} / \textbf{85.26} & \textbf{85.33} / \textbf{84.73} & \textbf{96.63} / \textbf{96.63} & \multicolumn{1}{c|}{\textbf{94.32} / \textbf{94.32}} & \textbf{97.66} / \textbf{97.66} & 97.34 / 97.34 \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table*}


\begin{table}[]
\color{blue}
\centering
\caption{Results on LPCR and FPI (network device logs). Note: The results of proprietary LLMs on the FPI task cannot be compared due to data privacy issues.}
\label{tab: network_result2-r3}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|c}
\toprule[1.5pt]
\multirow{3}{*}{Methods} & \multicolumn{2}{c|}{LPCR (Precision@1 / 3 / MRR)} & FPI (Accuracy) \\ \cmidrule{2-4} 
                         & \multicolumn{2}{c|}{Huawei}                       & Huawei         \\
                         & Switches                & Routers                 & Switches       \\ \midrule
CNN                      & 54.30 / 77.26 / 67.99   & 53.45 / 75.77 / 67.35   & 69.00          \\
BiLSTM                   & 59.27 / 78.04 / 71.22   & 51.45 / 69.56 / 63.76   & 74.83          \\
BERT                     & 76.18 / 91.54 / 84.70   & 72.57 / 91.59 / 82.61   & 88.75          \\
Biglog                   & 83.33 / 94.02 / 89.38   & 82.98 / 95.59 / 89.49   & 89.58          \\
KnowLog                  & 87.50 / 93.01 / 91.84   & 89.68 / 96.59 / 93.99   & 94.17          \\ \midrule
T5-KD                    & 86.11 / 93.56 / 91.41   & 84.48 / 92.59 / 90.33   & -              \\ \midrule
LLama3-70B               & \textbf{95.61} / \textbf{98.04} / \textbf{97.27}   & \textbf{97.48} / \textbf{99.49} / \textbf{98.52}   & 88.83          \\
ChatGPT                  & 90.95 / 95.11 / 93.88   & 97.20 / 98.34 / 98.19   & -              \\
GPT-4o                   & 95.65 / 98.29 / 97.27   & 97.39 / 99.09 / 98.47   & -              \\ \midrule
LUK (COT-ChatGPT)        & 85.18 / 95.03 / 90.55   & 84.58 / 95.99 / 90.64   & 90.42          \\
LUK (COT-GPT4o)          & 86.34 / 93.79 / 91.37   & 87.88 / 95.19 / 92.75   & 92.50          \\ \midrule
LUK (MEC-LLama3)         & 90.45 / 95.81 / 94.06   & 90.49 / 96.99 / 94.52   & 95.83          \\
LUK (MEC-ChatGPT)        & 89.37 / 95.19 / 93.43   & 88.48 / 94.69 / 90.33   & 93.33          \\
LUK (MEC-GPT4o)          & 90.92 / 96.04 / 94.46   & 90.69 / 96.09 / 94.39   & \textbf{96.67}          \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}

\uline{Our main revisions are as follows:}

\begin{enumerate}
    \item We clarify the challenge of knowledge acquisition with the LLM in \textbf{Section I, Page 2:} \\
    \uline{\textbf{Section I, Page 2:}} \textcolor{blue}{Although LLMs have
shown remarkable capabilities in various tasks, LLMs still
have difficulty in acquiring complete and accurate knowledge
due to hallucination, which may result in not covering all the
depth of knowledge and there may be misunderstandings when
dealing with domain-specific data [42, 43]}
    \item We modify the introduction of role design in \textbf{Section III.B}. \\
    \uline{\textbf{Section III.B.1), Page 4:}} \textcolor{blue}{\textbf{Director.} The Director’s primary objective is to establish
a comprehensive high-level framework aimed at providing
a strategic overview to drive the team’s efforts in
understanding logs. This role outlines the key points essential
for log understanding, thus ensuring that essential
insights are highlighted and comprehensively addressed.} \\
\textcolor{blue}{\textbf{Executor.} As the central role of this team, the Executor is tasked with the detailed execution of the log analysis
process. By receiving key points from the Director and
feedback from the Evaluator, the Executor undertakes
content generation and refinement two critical responsibilities.
Firstly, the Executor generates content intricately
aligned with the outlined key points. Secondly, the Executor
refines and polishes the content based on feedback,
enhancing the knowledge quality.} \\
\textcolor{blue}{\textbf{Evaluator.} The Evaluator assumes the crucial responsibility
of ensuring the quality and adherence of generated
content to predefined requirements. We define three evaluation
requirements for the Evaluator to scrutinize the
Executor’s generation on three fundamental aspects: completeness,
consistency, and conciseness. By evaluating
content against these criteria, the Evaluator validates the
accuracy and completeness of the generated knowledge.} 
\item We add the introduction of contrastive examples in \textbf{Section III.B}. \\
\uline{\textbf{Section III.B.2), Page 4-5:}} \textcolor{blue}{LLM Hallucinations
seriously affect the accuracy and quality of outputs
[70, 71]. Given the propensity of LLM-generated content to
exhibit deficiencies in comprehensiveness and informativeness,
ensuring the superior quality of directly generated knowledge
poses a significant challenge. To mitigate the hallucination of
LLM and ensure the quality of expert knowledge, we build the role of an Evaluator in the MEC framework and define
three evaluation aspects to evaluate the quality of generated
knowledge automatically, which encourages the LLM to actively
seek more detailed suggestions from the self-evaluation
before delivering a formal response. However, the MEC
framework runs under the challenging reference-free setting
and the evaluation requirements cannot be directly quantified
through metrics, the LLM tends to generate ambiguous and inconsistent
evaluations without fine-grained distinguishability,
causing unsatisfactory evaluation performance [72, 73].} \\
\textcolor{blue}{To address the evaluation weaknesses of the LLM, we
provide evaluation examples as the reference in the Evaluator
prompt. By providing specific examples, the Evaluator uses
them as the basis for evaluation, thus better steering the
evaluation of LLMs towards our desired goals. Considering
that the single type of example makes the LLM biased,
motivated by contrastive learning techniques [74, 75], we construct
contrastive examples consisting of positive and negative
knowledge of the same log to Evaluator as reference examples,
where the positive example showcases the desired knowledge,
while the negative example highlights the unsatisfactory
knowledge that should be avoided. By analyzing both types of
examples before generating the evaluation, the Evaluator can
reason about our evaluation requirements and make a more
informed decision about how to evaluate.} \\
\textcolor{blue}{
Specifically, we select one log $L$ with high-quality knowledge $K_{pos}$ as the positive example, which can be manually constructed by experts or generated from the LLM and manually confirmed. Considering that negative examples $\{K_{neg}\}_{c=1} ^ C, C=3$ of the log $L$ are unavailable directly, to construct the negative examples automatically, we propose to prompt the LLM to modify the positive knowledge making it unsatisfactory for evaluation.
As shown in \textcolor{red}{Fig. \ref{fig:negative_template-r3}}, we first give the background in the prompt and then clarify the task of modifying knowledge for the LLM, where we can specify which evaluation metrics are not fulfilled. Next, we provide the raw log, the raw positive knowledge, the key points, and the three evaluation requirements in the prompt.
Finally, we require the LLM to give the reason for not fulfilling the evaluation requirements while generating the modified content, which not only improves the reasoning ability of the \textit{Evaluator} but also provides guidance for the revision of the content by \textit{Executor}.
In cases where the LLM-generated negative examples do not capture the characteristics we want to avoid, this can be manually checked, and feedback can be given to the LLM to re-generate negative samples. 
To avoid the higher expense of the longer prompt, we construct one positive knowledge and its corresponding three negative knowledge as reference examples to be provided to the \textit{Evaluator}. 
The contrastive examples we constructed in our experiments are in Fig. 6.}

\item We modify the introduction of collaboration in \textbf{Section III.B}. \\
\uline{\textbf{Section III.B.3), Page 5:}} \textcolor{blue}{After constructing evaluation examples and assigning roles to LLMs, different roles start working to collaborate and interact according to the requirements in the prompt. 
First, the \textit{Director} meticulously analyzes the input logs to discern key points and formulates a plan for comprehending the logs effectively. Subsequently, the \textit{Director} shares these insights with the \textit{Executor} to guide the content generation process. The \textit{Executor} utilizes these key points to create detailed content that aligns with the requirements.
Finally, the detailed content produced by the \textit{Executor} undergoes evaluation by the \textit{Evaluator} to assess its quality. If the content meets the evaluation requirement, it is directly output as expert knowledge. In cases where the evaluation result is unsatisfactory and improvements are needed, the \textit{Evaluator} provides feedback to the \textit{Executor} for refinement.  To rigorously ensure the quality of the generated knowledge, this evaluation and refinement mechanism will be iterative until the content generated by \textit{Executor} meets the evaluation requirement or the maximum number of iterations is reached. We set up 3 iterations to build expert knowledge in our experiments. The pseudocode of the multi-expert collaboration framework is outlined in Algorithm \ref{alg:algorithm-r3}.
} \\
\textcolor{blue}{ This collaborative framework manifests two pivotal advantages:
Firstly, leveraging multiple roles' collective insights and skills enables a multi-perspective analysis of the input log, 
thereby mitigating the one-sidedness and bias inherent in a single model's response acquiring more professional expert knowledge. 
Secondly, through the feedback loop mechanism, the framework enables iterative refinement of content. This iterative process of evaluation, feedback incorporation, and content enhancement promotes continuous improvement, thereby ensuring that the expert knowledge acquired is comprehensive and of high quality.}
\end{enumerate}

\begin{figure}[]
\centering
   \includegraphics[width=\linewidth]{new_fig/luk_prompt_template.pdf}
   \caption{\textcolor{blue}{Prompt template of constructing negative samples, where the underlined portion of the prompt supports user modification based on their own data and intent.}}
   \label{fig:negative_template-r3}
\end{figure}


\begin{algorithm}
\caption{\textcolor{blue}{Pseudocode of multi-expert collaboration.}}
\label{alg:algorithm-r3}
\begin{algorithmic}
\REQUIRE \textcolor{blue}{Input Log $log$, LLM $\mathcal{M}$, Example Knowledge   $K_{pos}$}      %输入条件
\ENSURE \textcolor{blue}{Output Expert Knowledge $k$}
\STATE \textcolor{gray}{\# Construct Contrastive Examples}
\FOR{\textcolor{blue}{$c = 1$ to $C$}}
    \STATE \textcolor{blue}{$K_{neg}^c = \mathcal{M}(Prompt_{Modify}, K_{pos})$}
\ENDFOR
\STATE  \textcolor{blue}{$K_{examples} = K_{pos} \cup \{K_{neg}\}_{c=1} ^ C $}
\STATE \textcolor{gray}{\# Initial Roles}
\STATE $\mathcal{DIRECTOR} = Init\_Role(Prompt_{Dirctor}, \mathcal{M}) $
\STATE $\mathcal{EXECUTOR} = Init\_Role(Prompt_{Executor}, \mathcal{M}) $
\STATE \textcolor{blue}{$Prompt_{Evaluator} = Prompt_{Evaluator}.join(K_{examples})$}
\STATE \textcolor{blue}{ $\mathcal{EVALUATOR} = Init\_Role(Prompt_{Evaluator},  \mathcal{M})$}
\STATE \textcolor{gray}{\# Collaboration}
\STATE \textcolor{blue}{Init: $epoch = 0, feedback = False$}
\STATE $ keypoint = \mathcal{DIRECTOR}(log) $
\STATE $ content = \mathcal{EXECUTOR}(log, keypoint) $
\REPEAT
\STATE \textcolor{blue}{$ epoch = epoch + 1$}
\STATE \textcolor{blue}{$ feedback = \mathcal{EVALUATOR}(log, keypoint, content) $}
\IF{\textcolor{blue}{$feedback == False$}}
\STATE \textcolor{blue}{$ content = \mathcal{EXECUTOR}(content, feedback) $}
\ENDIF
\UNTIL{\textcolor{blue}{$epoch == Epoch$ or $feedback==True$}}
\STATE $k = content$
\RETURN $k$
\end{algorithmic}
\end{algorithm}
    


\textbf{C3:} In the MEC framework, although outputs from Executors are evaluated by Evaluators, the correctness of outputs from both Evaluators and Directors is not guaranteed. Moreover, after receiving the feedback from the Evaluator, the new content generated by the Executor is directly outputted without a correctness check. Given that the MEC framework is crucial for pre-training, ensuring the correctness of its outputs is essential, or at least, MEC's output correctness should be evaluated. Although the manuscript made a qualitative analysis of two examples, my question is: How often does the MEC framework extract correct knowledge, and how often does MEC extract incorrect knowledge?

\textbf{R3:} Thanks for your suggestions.  First, we statistics the proportion of unsatisfactory knowledge in each iteration.
As shown in \textcolor{red}{Fig. \ref{fig:roundn-r3}}, the \textit{Evaluator} ultimately passed with over 95\% knowledge. 

Second, we count distributions of different error categories in
unsatisfactory knowledge according to \textit{Evaluator}’s results.
As shown in \textcolor{red}{Fig. \ref{fig:different_error_precent-r3}}, it can be found that a significant portion of the inadequacies stems from issues related to completeness. 

\begin{figure*}[]
    \centering
    % \vspace{-2mm}
    \subfloat[Anomaly Detection (BGL)]{\label{fig: roundaaa}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/error_round_percent.pdf}}
    \subfloat[MC (Huawei-Switches)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/mc_roundn.pdf}}
    \subfloat[LDSM (Huawei-Switches)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/ldsm_roundn.pdf}}
    \caption{\textcolor{blue}{Figure (a) shows the proportion of unsatisfactory knowledge in each iteration. Figure (b) and (c) show the results of the refined knowledge based on the evaluation feedback each time.}}
    
    % \vspace{-5mm}
    \label{fig:roundn-r3}
\end{figure*}

\begin{figure}[]
    \centering
    % \vspace{-2mm}
    \subfloat[GPT-4o]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.5\linewidth]{new_fig/error_percent_gpt4o.pdf}}    
    \subfloat[LLama3-70B]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.5\linewidth]{new_fig/error_percent_llama3.pdf}}
    
    \caption{\textcolor{blue}{Distributions of error categories in unsatisfactory knowledge.}}
    
    % \vspace{-5mm}
    \label{fig:different_error_precent-r3}
\end{figure}

\uline{Following your suggestions, our main revisions are as follows:}
\begin{enumerate}
    \item We add the ablation studies of the iterative mechanism in \textbf{Section IV.F, Page 15:} \\
    \uline{\textbf{Section IV.F, Page 15:}} \textcolor{blue}{To verify the performance of the iterative evaluation and
refinement mechanism, we first statistics the proportion of
unsatisfactory knowledge in each iteration, and then verify the
performance of the refined knowledge based on the evaluation
feedback each time on the MC and LDSM tasks, where we set
up 3 iterations in our experiment. As shown in Fig. 10, we can
find a consistent decline in the proportion of unsatisfactory
knowledge with each successive iteration. Simultaneously,
the performance of the enhanced model exhibits steady improvement,
underscoring the positive impact of the iterative
evaluation and refinement mechanism within the framework.
Notably, our observations indicate that a significant portion
of knowledge refinement occurs following the initial feedback
round, with subsequent iterations primarily focusing on refining
a smaller fraction of the knowledge. To save costs, we
suggest that the framework can iterate one time as a cost-effective
strategy, effectively balancing performance gains with
resource optimization.}
    \item We add the case analysis of the MEC framework in \textbf{Section V.B.1), Page 16:} \\
    \uline{\textbf{Section V.B.1), Page 16:}} \textcolor{blue}{1) Evaluation and refinement mechanism of the MEC
framework: To intuitively understand the workflow of the
MEC framework and analyze the impact of the evaluation and
refinement mechanism on knowledge generation, we provide
a specific case of expert knowledge construction as shown in Fig. 11, this input log from the Huawei device.
As can be seen from the case, the Director first meticulously
analyzes the input log to give key points, and then the Executor
generates expert knowledge based on the guidance of these key
points. Following knowledge creation, the Evaluator evaluates
the quality of the generated knowledge and provides feedback
to the Executor for refinement. The evaluation feedback shows
that the content generated by the Executor does not fulfill
completeness and consistency. Specifically, the generated
knowledge lacks of an introduction to the procedure step and
the explanation of the severity level is not rigorous. In addition,
there is also an uninformative explanation in the generated
knowledge, which makes it more difficult for the smaller
model to understand the expert knowledge. Finally, the Executor
refines the generated knowledge based on the evaluation
feedback. From the re-generated knowledge, we can find that
the Executor not only supplements the clear introduction of the
procedure step but also modifies the explanation of severity
level to make it more reasonable. Overall, the re-generated
knowledge is more comprehensive and rigorous, which is more
conducive for the smaller model to learn expert knowledge.
To more deeply reveal the issues of knowledge generated by
LLMs. We count distributions of different error categories in
unsatisfactory knowledge according to Evaluator’s results for
GPT-4o and LLama3-70B, respectively. As shown in Fig. 12,
it can be found that a significant portion of the inadequacies
stems from issues related to completeness. The prevalence of completeness-related errors underscores the challenge faced
by the single LLM in producing comprehensive knowledge
autonomously. Moreover, alongside completeness issues, a
smaller yet notable proportion of unsatisfactory knowledge is
attributed to deficiencies in conciseness and consistency. This
finding underscores the significance of collaborative frameworks
that integrate diverse roles, each contributing unique
perspectives and expertise to compensate for the capacity
deficiencies of the single LLM and improve the completeness
and accuracy of generated knowledge.}
\end{enumerate}

\textbf{C4:} The key idea behind word-level token prediction is the knowledge perception module (KPM), which calculates the weights of each token in a given knowledge. However, the attention mechanism also adjusts the weights of tokens within the knowledge. These two objectives appear to overlap. Could the authors explain why using the attention mechanism alone is insufficient and why the additional KPM module is necessary?

\textbf{R4:} Thanks for your comments. The independent attention mechanism can not work for the bi-encoder architecture. 
Without the knowledge perception module (KPM), our proposed word-level pre-training task degenerates into BERT's Masked Language Modeling (MLM) task, where they only perceive their own contextual information with one encoder and cannot integrate external knowledge.

Experimentally,  we also compare it with existing pre-training tasks in the ablation experiment, including BERT's Masked Language Modeling (MLM) task and KnowLog's Abbreviation Prediction (AP) task. 
As shown in \textcolor{red}{Table \ref{tab:ablation-r3}}, results demonstrate the superior capability of our token prediction task in integrating domain knowledge effectively. 

\uline{We add the discussion of the existing pre-training tasks.}
\begin{enumerate}
    \item \uline{\textbf{Section I, Page 2:}} \textcolor{blue}{Since
logs and expert knowledge obtained from LLM are heteroge-
neous data, smaller models with fewer parameters and limited
learning capacity struggle to capture knowledge [48, 49].
Masked Language Modeling (MLM) [31] as the widely used
pre-training task for most pre-trained models, they can only
perceive their own contextual information and cannot incorporate external knowledge.}
    \item We add the ablation experiment of existing pre-training tasks in \textbf{Section IV.F, Page 15:} \\
    \uline{\textbf{Section IV.F, Page 15:}} \textcolor{blue}{To further
verify our proposed word-level Token Prediction (TP) task,
we also compare it with other word-level pre-training tasks,
including BERT’s Masked Language Modeling (MLM) task
and KnowLog’s Abbreviation Prediction (AP) task. The results
demonstrate the superior capability of our token prediction
task in integrating domain knowledge effectively. Unlike MLM
and Abbreviation Prediction tasks, our proposed pre-training
task requires models to not only predict tokens within the
log itself but also dynamically assimilate contextual insights
from domain-specific knowledge using the knowledge perception module. This distinctive aspect sets our approach apart,
as BERT solely relies on internal information and cannot
leverage external knowledge. Conversely, KnowLog is limited
in its scope, focusing solely on abbreviations and failing to
comprehend other critical log elements such as parameters,
conditions, and more, which are essential for a comprehensive
understanding of domain-specific terminology.}
\end{enumerate}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\color{blue}
\caption{\textcolor{blue}{Ablation studies for LUK, where TP and SA represent the pre-training tasks Token Prediction, and Semantic Alignment for LUK, respectively. MLM represents the pre-training task Masked Language Modeling of BERT and AP represents the pre-training task Abbreviation Prediction of KnowLog.}}
\label{tab:ablation-r3}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc|cc}
\toprule[1.5pt]
\multirow{3}{*}{Methods}         & \multicolumn{2}{c|}{MC (Accuracy / Weighted-F1)} & \multicolumn{2}{c}{LDSM (Accuracy / Weighted-F1)} \\ \cmidrule{2-5} 
                                 & \multicolumn{2}{c|}{Huawei}                      & \multicolumn{2}{c}{Huawei}                        \\
                                 & Switches                & Routers                & Switches                & Routers                 \\ \midrule
BERT                             & 82.37 / 81.20           & 81.18 / 79.20          & 93.18 / 93.18           & 90.06 / 90.05           \\
LUK (MEC-GPT4o)                  & \textbf{85.51} / \textbf{85.26}           & \textbf{85.33} / \textbf{84.73}          & \textbf{97.66} / \textbf{97.66}           & \textbf{97.34} / \textbf{97.34}           \\ \midrule
$\vdash$ w/o Evaluator           & 83.77 / 83.26           & 82.30 / 81.08          & 96.57 / 96.57           & 95.53 / 95.53           \\
$\vdash$ w/o Evaluation Examples & 84.38 / 84.17           & 82.13 / 81.06          & 96.64 / 96.64           & 95.63 / 95.63           \\ \midrule
$\vdash$ w/o TP                  & 83.25 / 82.65           & 81.66 / 79.92          & 95.95 / 95.95           & 95.68 / 95.68           \\
$\vdash$ w/o SA                  & 83.77 / 83.19           & 84.14 / 82.92          & 95.25 / 95.25           & 94.68 / 94.68           \\ \midrule
$\vdash$ only with MLM           & 83.24 / 83.25           & 82.36 / 81.19          & 94.19 / 94.19           & 93.62 / 93.61           \\
$\vdash$ only with AP            & 83.60 / 82.89           & 82.72 / 81.68          & 94.39 / 94.39           & 93.97 / 93.97           \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table}


\textbf{C5:} The manuscript lacks a detailed description of datasets used for pre-training, fine-tuning, and evaluating each downstream task. Specifically, RQ2 states, "In this RQ, ... we conduct experiments on downstream tasks beyond the pre-training logs." Does this imply that the evaluation dataset used in RQ1 will also be included in the pre-training and fine-tuning processes?

\textbf{R5:} We apologize for the unclear description of the datasets. 
The evaluation datasets in our experiments include two types: including in the pre-training corpus and not including in the pre-training corpus. 
First, the evaluation datasets of the RQ1 come from the same source as the pre-training data.  Second,  to verify the generalization capability of LUK in RQ2, we collect more logs not included in the pre-training for evaluation. Specifically, for software logs, we collect ThunderBird
and Spirit as the datasets of the Anomaly Detection task from
Loghub \cite{zhu2023loghub}. For network device logs, we collect logs from other vendors (H3C) and devices
(Security) as the datasets.

\uline{Following your suggestions, we clarify the description of the datasets in the revised manuscript. }

\begin{enumerate}
    \item We modify the description of the evaluation datasets in \textbf{Section IV.C, Page 8:} \\
    \uline{\textbf{Section IV.C, Page 8:}} \textcolor{blue}{The evaluation datasets in our experiments include two types: including in the pre-training corpus and not including
in the pre-training corpus. For most datasets, we collect the
evaluation datasets from the same source as the pre-training
data. Moreover, apart from logs involved in pre-training, to
verify the generalization capability of LUK, we collect more
logs that are not included in the pre-training for evaluation.}
    \item We clarify the evaluation dataset of RQ2: \\
    \uline{Section IV.E.RQ2, Page 12:} As the system evolves, many previously unseen logs will be
collected [82], \textcolor{blue}{and it is unrealistic to collect all the real-world
logs for pre-training. In this RQ, to verify the generalization
of LUK, we conduct experiments on downstream tasks where
the logs in these datasets do not appear in the pre-training
phase. Specifically, for software logs, we collect ThunderBird
and Spirit as the datasets of the Anomaly Detection task from
Loghub [38]. For network device logs, as shown in Table
III, we collect logs from other vendors (H3C) and devices
(Security) as the datasets.}
\end{enumerate}


\textbf{C6:}  If the evaluation dataset is included in the pre-training or fine-tuning steps, could this design introduce data leakage issues?

\textbf{R6:} Thanks for your reminder. There is no data leakage in our downstream tasks. During pre-training, the model is only familiarized with the vast original logs and knowledge, and there is no ground-truth of the downstream tasks. In fact, as with existing general pre-trained models \cite{feng2020codebert,zhao2023survey,naveed2023comprehensive,liu2023pre} and log pre-trained models \cite{guo2021logbert,tao2023biglog}, the objective of our pre-trained model is to learn effective contextual representations from massive unlabeled logs and corresponding knowledge optimized
by pre-training tasks.

\textbf{C7:} Please provide the time required for pre-training and fine-tuning a PLM using the LUK framework.

\textbf{R7:} Thanks for your reminder. We provide the time cost for the pre-training in the Section of \textit{Parameters Setting}. It takes 3 hours to pre-train on 2 NVIDIA A100 GPUs.
We provide the time cost for fine-tuning in the experiments section.
As shown in \textcolor{red}{Fig. \ref{fig:time-cost-r3}}, even excluding the fine-tuning time, the average inference speed
of LUK is 718x, and 868x faster than GPT-4o and LLama3-
70B, respectively. 

\begin{figure}[]
    \centering
    % \vspace{-2mm}
    \subfloat[LDSM (Huawei-Switches)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 2.pdf}}
    
    \subfloat[LPCR (Huawei-Switches)]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 1.pdf}}

    \subfloat[Anomaly Detection (BGL)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.95\linewidth]{new_fig/Data 3.pdf}}
    
    \caption{\textcolor{blue}{Time expense of different models during reasoning.}}
    
    % \vspace{-5mm}
    \label{fig:time-cost-r3}
\end{figure}

\textbf{C8:} Although KnowLog can only pre-train PLMs on a limited set of logs with documentation, it would be better if the manuscript could include KnowLog's performance in Tables VII and VIII. Since KnowLog's pipeline is quite similar to that of LUK, understanding the performance differences between these two tools can better illustrate the contributions of LUK.

\textbf{R8:} Thanks for your reminder. We supplement the experiments of KnowLog in the revised manuscript. Experimentally, our experiments and case studies demonstrate that LUK consistently outperforms KnowLog across various metrics, substantiating the efficacy and advancement of our proposed approach.

Theoretically, first, LUK focuses on the challenge of the high cost and inefficiency of reasoning for Large Language Models (LLMs). It introduces a novel framework that reduces the computational overhead of LLMs by distilling knowledge into smaller models, enhancing practicality in log analysis contexts. In contrast, KnowLog's primary emphasis lies in leveraging existing domain knowledge to enhance log understanding.
Second, LUK has an advantage over KnowLog in terms of knowledge acquisition. KnowLog enhances the model based on existing documentation knowledge, however, most logs lack documentation, and the cost of manually constructing knowledge is extremely high, KnowLog cannot work in the absence of documentation. LUK, on the other hand, does not need to rely on existing documentation and obtains sufficient knowledge through the LLM, which is even of higher quality than the documentation knowledge, thus making LUK more practical. Third, LUK proposes a new pre-training task from the word level. KnowLog's abbreviation prediction task only recognizes the abbreviations that are already in the log. It cannot understand other key information within the log's tokens (such as parameters) and cannot perceive useful information from external knowledge to enhance the understanding of domain tokens. And LUK can adaptively perceive useful knowledge to understand tokens in logs, not limited to abbreviations. 

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{new_fig/luk_knowledge_case.pdf}
   % \vspace{-6mm}
   \caption{\textcolor{blue}{Example of knowledge generated by GPT-4o and retrieved from documentation.}}
   % \vspace{-4mm}
   \label{fig:knowledge_case-r3}
\end{figure*}

\begin{figure}[]
\centering
    % \vspace{-2mm}
    \includegraphics[width=\columnwidth]{new_fig/LUK_percentage_1.pdf}    
    
    \caption{\textcolor{blue}{Proportion of unsatisfactory knowledge, where we employ the evaluation criteria of the MEC framework to evaluate the knowledge.}}
    
    % \vspace{-5mm}
    \label{fig:doc-knowledge-analysis-r3}
\end{figure}

\uline{Our main revisions are as follows:}
\begin{enumerate}
\item We add KnowLog as the baseline in our experiments. \\
    \uline{\textbf{Section IV.D.2), Page 10:}} 
    \textcolor{blue}{In addition, KnowLog is the state-of-the-art log pre-trained model in log analysis not only due to pre-training on log corpus but also enhancing the pre-training with documentation knowledge. Referring to KnowLog, we collect the descriptions of logs from the Huawei and Cisco public documentation as background knowledge to enhance the log pre-training in the same way. For fairness, we reproduce Biglog and KnowLog with the same pre-training setting on our log corpus.} 
    \item We add the analysis of the experiments about KnowLog in \textbf{Section IV.E, Page 11-14:} \\
    \uline{\textbf{Section IV.E.RQ1, Page 11:}} \textcolor{blue}{To verify the effectiveness of the expert knowledge obtained
from the LLM, we compare it with the KnowLog, whose
knowledge is obtained from the documentation. Our experimental
findings demonstrate that MEC-based LUK surpasses
KnowLog in performance, more specifically, LUK (MECGPT4o)
improves the average Accuracy on the Cisco and
Huawei datasets regarding the MC and LDSM tasks by 2.38\%
and 1.15\%, respectively. It is noteworthy that Huawei’s documentation
provides more detailed log descriptions compared
to the relatively concise descriptions found in Cisco’s documentation.
This disparity underscores the LLM’s capability
to generate domain knowledge of equal or superior quality to that found in high-quality documentation. Given the scarcity of
documented descriptions for most logs in practice, obtaining
expert knowledge through KnowLog becomes impractical. For
instance, the challenge of sourcing relevant documents for
logs from sources like Loghub [38] significantly hampers
the effectiveness of KnowLog. Our approach, which operates
independently of documentation, consistently yields superior
results, and serves to diminish the reliance on human experts
for intricate knowledge construction processes, offering a more
feasible and practical alternative to traditional documentation-based
methodologies.} \\
    \uline{\textbf{Section IV.E.RQ2, Page 12:}} \textcolor{blue}{
    In comparison to KnowLog, LUK still has a clear advantage
over KnowLog, which takes knowledge from the documentation.
The domain knowledge derived from LLMs offers a deeper
level of comprehension and learning, enabling the PLM to
generalize more effectively to new log datasets. Conversely,
KnowLog, constrained by information within documents, may
not provide sufficiently profound domain insights to support
robust generalization of the PLM to unseen data.} \\
    \uline{\textbf{Section IV.E.RQ3, Page 13:}} \textcolor{blue}{In contrast, KnowLog’s reliance on knowledge
solely extracted from documentation may lead to limitations
in handling the evolving nature of log data.} \\
    \uline{\textbf{Section IV.E.RQ4, Page 14:}} \textcolor{blue}{KnowLog primarily relies on
knowledge extracted from documentation, which may be limited
in scope and quality, especially in low-resource settings.
In contrast, this proves that knowledge acquired by the LLM
has a wider scope and can provide a more comprehensive
and diverse range of information, rather than being limited to
some specific documentation.}
    \item To further verify our proposed word-level Token Prediction (TP) task,
we also compare it with other word-level pre-training tasks \textcolor{red}{Table \ref{tab:ablation-r3}},
including BERT’s Masked Language Modeling (MLM) task
and KnowLog’s Abbreviation Prediction (AP) task. \\
    \uline{\textbf{Section IV.F, Page 14:}} \textcolor{blue}{
    To further verify our proposed word-level Token Prediction (TP) task,
we also compare it with other word-level pre-training tasks,
including BERT’s Masked Language Modeling (MLM) task
and KnowLog’s Abbreviation Prediction (AP) task. The results
demonstrate the superior capability of our token prediction
task in integrating domain knowledge effectively. Unlike MLM
and Abbreviation Prediction tasks, our proposed pre-training
task requires models to not only predict tokens within the
log itself but also dynamically assimilate contextual insights
from domain-specific knowledge using the knowledge perception
module. This distinctive aspect sets our approach apart,
as BERT solely relies on internal information and cannot
leverage external knowledge. Conversely, KnowLog is limited
in its scope, focusing solely on abbreviations and failing to
comprehend other critical log elements such as parameters,
conditions, and more, which are essential for a comprehensive
understanding of domain-specific terminology.}
    \item We add the case study to analyze the quality of the expert knowledge from different sources in \textbf{Section V.B.2), Page 17:} \\
    \uline{\textbf{Section V.B.2), Page 17:}} \textcolor{blue}{Evaluation and refinement mechanism of the MEC
framework: To further intuitively analyze the quality of the expert knowledge constructed with the MEC framework, we compare it with the knowledge collected from documentation and the COT-based approach. As shown in \textcolor{red}{Fig. \ref{fig:knowledge_case-r3}}, we collect a Cisco log as the case and give the corresponding generated knowledge based on the COT and MEC methods.} \\
    \textcolor{blue}{
As can be seen from these cases, the knowledge provided by the documentation is too simple, which provides a generic and limited understanding of the log without delving into specific details or potential causes. Although COT-based knowledge offers a more detailed explanation of the log, compared to MEC-based knowledge, there is still the problem of inadequate knowledge and lack of insight.
In contrast, the knowledge derived from the MEC framework excels in its comprehensive analysis and insights. By explicitly outlining the specifics of the log error, including the MTS queue failure and the placeholders for queue and error message, the MEC-based knowledge provides a deeper understanding of the issue at hand. Furthermore, it goes beyond mere description to identify potential root causes such as network connectivity issues.
The comparison highlights the clear advantage of the MEC framework in expert knowledge generation. Its collaborative nature allows for the integration of diverse expertise and perspectives, resulting in a more comprehensive analysis of complex logs.} \\ 
\textcolor{blue}{
To quantify the differences among the various forms of knowledge, we employ the evaluation criteria of the MEC framework to evaluate the knowledge acquired by the documentation and the knowledge constructed based on COT in the network device logs. The evaluation results are shown in \textcolor{red}{Fig. \ref{fig:doc-knowledge-analysis-r3}}, revealing a notable contrast in quality between the different sources of knowledge. It is apparent from the analysis that a significant proportion of knowledge sourced from documentation falls short of meeting the evaluation requirements. This deficiency can be attributed to the inherent limitations of documentation-derived knowledge, which often lacks depth and detail, offering only the most straightforward description of the logs. Combined with Fig. 10a, this suggests that the knowledge acquired from MEC based on LLMs is comparable or even better than the documentation. Considering the lack of documentation support for most logs and the high cost of manually constructing knowledge, this provides a feasible way to gain a wealth of practical knowledge automatically.}

\end{enumerate}


\textbf{C9:}  RQ1 states, "Comparing MEC with COT, MEC demonstrates superior performance." However, my reading of the experiments is the opposite: MEC appears to provide only marginal improvements and, in some cases, even performs worse, as indicated in Tables VII and VIII. To what extent do you believe the improvements offered by MEC are sufficient?

\textbf{R9:} We apologize for the previous inadequate design and experiments.  After we improve the framework, the latest experimental results gain an improvement over the previous version on all datasets, which is significantly better than the existing baselines.
In particular, as shown in \textcolor{red}{Fig. \ref{fig:low-resource-results-r3}}, LUK is more effective in the challenging log analysis tasks of low-resource scenarios. 
Specifically, we made the following improvements to the original framework:
\begin{itemize}
    \item We employ the more powerful LLM (GPT-4o) as the backbone to build the MEC framework in our experiments;
    \item We refine the design of the MEC framework from the following two aspects, including: 1) Constructing the contrastive examples to improve the Evaluator's evaluation capability under the challenging reference-free setting; and 2) Constructing the evaluation and refinement mechanisms as the iterative framework.
\end{itemize}.

\begin{figure*}[]
    \centering
    % \vspace{-2mm}
    \subfloat[Anomaly Detection (BGL)]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_BGL.pdf}}
    \subfloat[LDSM (Huawei-Security)]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_ldsm.pdf}}
    \subfloat[Fault Phenomenon Identification]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.33\linewidth]{new_fig/low_resouce_fpi.pdf}}
    \caption{Results on different ratios of the training dataset.}
    
    % \vspace{-5mm}
    \label{fig:low-resource-results-r3}
\end{figure*}

\textbf{C10:} Tables and Figures in the Experiments section miss some baselines or datasets. I hope authors can explain the following in the revised manuscript:
\textbf{(1)} In Table II, some datasets (ThunderBird, Spirit) are not included in the pre-training phase.
\textbf{(2)} In RQ1, FPI is not included.
\textbf{(3)} RQ3 does not include LUK (COT-ChatGPT). Since LUK-COT achieves a very comparable performance against LUK (MEC-ChatGPT), I am curious about its performance. Thus I am wondering why it is not included in RQ3?

\textbf{R10:} Thanks for your reminders. We respond to the above three questions as follows:
\begin{enumerate}
    \item  We apologize for the unclear description of the datasets. We exclude some datasets (ThunderBird, Spirit) in the pre-training phase to verify the generalization of the pre-trained model. Considering that it is unrealistic to collect all the real-world logs for pre-training, these logs that do not appear in the pre-training phase are used to evaluate the generalization of the model.  Our findings affirm that LUK excels in its generalization capabilities by adeptly analyzing previously unseen logs. 
    \item  We apologize for not showing the complete baselines on the FPI task. Following your suggestions, we provide the FPI results in \textcolor{red}{Table \ref{tab: network_result2-r3}}. 
    Since the dataset of the FPI is collected from the real world, we cannot evaluate it with proprietary LLMs due to data privacy. 
    \item Following your suggestions, we also provide the complete baselines about RQ3 in \textcolor{red}{Fig. \ref{fig:robust-r3}}.
    It can be seen that LUK performs much better than other baselines.
\end{enumerate}

\begin{figure}[]
    \centering
    \vspace{-2mm}
    \subfloat[Anomaly Detection (BGL)]{\label{fig: system type forgetting}\includegraphics[width=0.95\linewidth]{new_fig/injector_ratio_f1.pdf}}
    
    \subfloat[LDSM (Huawei Switches)]{\label{fig: system type zero}\includegraphics[width=0.95\linewidth]{new_fig/injector_ratio_accuracy.pdf}}
    \caption{\textcolor{blue}{Results on different synthetic datasets of unstable log.}}
    % \vspace{-5mm}
    \label{fig:robust-r3}
\end{figure}

\textbf{C11:}  Regarding LUK (MEC-ChatGPT)'s performance on the MC-Huawei-Routers task, there is an inconsistency between Table XII (83.43/82.49) and Table VIII (83.55/82.41). Please double-check and resolve the inconsistency.

\textbf{R11:} We apologize for displaying the wrong results due to our carelessness. We re-run the experiments for the tasks with our latest framework and check all the results in the revised manuscript. 
The updated experiment results are shown in \textcolor{red}{Table \ref{tab:ablation-r3}.}

\textbf{C12:} Comments on Presentation
Overall, the writing is clear. Here are a few minor issues:

Page 4: Are 'background knowledge' and 'expert knowledge' the same in Section III.C? If so, please make them consistent.
Page 7: this sentence is difficult to parse:
'where the input is a log as a query and an answer candidate set and the output is the ranking result.'

\textbf{R12:} Thanks for your reminder. First, we apologize for the inconsistent presentation of expert knowledge.     `Background knowledge' and `Expert knowledge' are consistent in this work. Following your suggestions, we have unified the presentation in the revised manuscript. Second, we clarify the presentation of the above sentence as follows: 
\textit{Specifically, the input is a log and an answer candidate set, then the model needs to find the most probable causes from the set and rank the candidate set based on the priority as the output. }


==> sections/baselines_revision.tex <==
\subsection{Data preparation}
In this paper, we collect logs from software systems and network devices to construct expert knowledge and the log pre-trained model. Specifically, we collect software system logs from Loghub \cite{zhu2023loghub}, including operating system logs composed of Windows and BGL, as well as distributed system logs composed of HDFS and OpenStack.
Given that these datasets contain a significant proportion of duplicated logs, we employ widely used Drain \cite{he2017drain} to parse these logs and achieve log templates. Subsequently, we only sample one instance log as input that corresponds to each unique template.
In addition, we also collect network device logs from the public documentation of two vendors, Cisco\footnote{\url{https://www.cisco.com/c/en/us/support/all-products.html}} and Huawei\footnote{\url{https://support.huawei.com/enterprise/en/index.html}}, including three devices: Switches, Routers, and WLAN. The detailed statistics are shown in Table \ref{tab:statistics}.


% such as logs on switches of Cisco and Huawei. Specifically, we collected 28,990 log templates from the public documentation of two vendors, Cisco\footnote{\url{https://www.cisco.com/c/en/us/support/all-products.html}} and Huawei\footnote{\url{https://support.huawei.com/enterprise/en/index.html}}, including three devices: switches, routers, and WLAN. The detailed statistics are shown in Table \ref{tab: statistics}. Then we prompt ChatGPT to generate the corresponding background knowledge.

% We use log templates instead of instance logs with specific parameters in our experiments for several considerations. First, these log templates are directly available from the public documentation, reducing the difficulty of data collection. Second, instance logs contain real parameters, which can easily cause the risk of data leakage. Finally, instance logs are often repetitive, increasing the workload of data pre-processing. Some studies have shown that repetitive content degrades the performance of the model. Finally, experiments also show that understanding log templates still has a good generalization to instance logs.


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphic   x}
\begin{table}[h]
\centering
\caption{Statistics of the dataset used for knowledge generation and pre-training.}
% \vspace{-2mm}
\label{tab:statistics}
\begin{tabular}{ll|c}
\toprule[1pt]
\multicolumn{1}{l|}{Datasets}                         & Category           & $\#$ of log templates \\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{Software System}} & Distributed System & 2,292               \\
\multicolumn{1}{l|}{}                                 & Operating System   & 11,947              \\ \midrule
\multicolumn{1}{l|}{\multirow{2}{*}{Network Device}}  & Cisco              & 16,591              \\
\multicolumn{1}{l|}{}                                 & Huawei             & 12,399              \\ \midrule
\multicolumn{2}{c|}{Total}                                                 & 43,229              \\ \bottomrule[1pt]
\end{tabular}%
% \vspace{-3mm}
\end{table}



\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{new_fig/luk_evaluation_examples.pdf}
   \vspace{-3mm}
   \caption{\textcolor{blue}{The contrastive samples constructed in our experiments, where Example 1 represents the positive example, and the remaining three examples are negative examples obtained from the modification of GPT-4o. Colour-marked text indicates that the evaluation requirements are unsatisfied. }}
   \vspace{-3mm}
   \label{fig:evaluation}
\end{figure*}


\subsection{Parameters Setting}
\begin{itemize}
\item  \textcolor{blue}{As for expert knowledge acquisition, we explore different large language models for experiments, including two proprietary LLMs: \textit{gpt-3.5-turbo} (ChatGPT) and \textit{gpt-4o} (GPT-4o), and one open-source model: \textit{Llama-3.3-70B-Instruct } (LLama3-70B) \cite{dubey2024llama}.} To increase the stability of LLM’s output, we set the temperature of LLMs to 0.
\item \textcolor{blue}{
For contrastive examples provided to the \textit{Evaluator}, we show in Fig. \ref{fig:evaluation}.}
% which contains an encoder with 12 layers, 12 self-attention heads, and the hidden size of 768.
\item For pre-training, we use \textit{bert-base-uncased} with 110M parameters in our experiments. During pre-training, we set the batch size as 32, epochs as 40 and the maximum length of the input text as 512. Moreover, the optimizer we adopt is Adam with a learning rate of 5e-5, a weight decay of 0.01, learning rate warmup for 2,000 steps and linear decay of the learning rate after.
\item For fine-tuning, we adopt the cross-entropy loss as the loss function in downstream tasks and we set epoch to 20 and 10 on log-single and log-pair tasks, respectively.
\item \textcolor{blue}{We spend 3 hours pre-training the LUK on 2 NVIDIA A100 GPUs with PyTorch 2.4.0.}
\end{itemize}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Statistics of downstream tasks datasets on software system  (Training/Validation/Testing Size).}
% \vspace{-2mm}
\label{tab:software_statistics}
\begin{tabular}{llcll}
\toprule[1pt]
\multicolumn{1}{l|}{Tasks}                                                                        & Dataset      & \multicolumn{3}{c}{\#Size}        \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Anomaly\\ Detection\end{tabular}}} & BGL          & \multicolumn{3}{c}{30K / 10K / 10K} \\
\multicolumn{1}{l|}{}                                                                             & ThunderBird* & \multicolumn{3}{c}{30K / 10K / 10K} \\
\multicolumn{1}{l|}{}                                                                             & Spirit*      & \multicolumn{3}{c}{30K / 10K / 10K} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Failure \\ Identification\end{tabular}}            & Openstack    & \multicolumn{3}{c}{236 / 80 / 80} \\ \bottomrule[1pt]
\multicolumn{5}{l}{* indicates logs not involved in the pre-training.}                                                                            
\end{tabular}%
% \vspace{-3mm}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[]
\caption{Statistics of downstream tasks datasets on network device (Training/Validation/Testing Size).}
% \vspace{-2mm}
\tabcolsep = 0.07cm
\label{tab:network_statistics}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lllll}
\toprule[1pt]
\multicolumn{1}{l|}{Tasks}                                                                                            &        & Switches             & Routers            & Security*         \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Module\\ Classification\end{tabular}}}                 & Cisco  & 13,495/4,498/4,498   & 7,265/2,422/2,421  & -                 \\
\multicolumn{1}{l|}{}                                                                                                 & Huawei & 3,439/1,146/1,146    & 2,539/846/845      & -                 \\
\multicolumn{1}{l|}{}                                                                                                 & H3C*   & 1,241/413/413        & 1,336/445/444      & -     \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Fault Phenomenon\\ Identification\end{tabular}}                        & Huawei & 362/120/120          & -                  & -                 \\ \midrule
\multicolumn{1}{l|}{\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Log and Description\\ Semantic Matching\end{tabular}}} & Cisco  & 49,954/16,651/16,651 & 26,975/8,992/8,991 & 1,894/631/631     \\
\multicolumn{1}{l|}{}                                                                                                 & Huawei & 7,702/2,567/2,567    & 5,977/1,992/1,991  & 4,485/1,495/1,494 \\
\multicolumn{1}{l|}{}                                                                                                 & H3C*   & 2,606/868/868        & 2,837/946/945      & 2,223/741/740     \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Log and Possible\\ Cause Ranking\end{tabular}}                         & Huawei & 3,851/1,283/1,283    & 3,097/1,032/1,032  & 2,361/787/787     \\ \bottomrule[1pt]
\multicolumn{5}{l}{* indicates logs not involved in the pre-training.}                                                                                                                        
\end{tabular}%
}
% \vspace{-3mm}
\end{table}

\subsection{Downstream tasks}
To explore the performance of LUK on different log analysis domains, we conduct experiments on different downstream tasks, including software system and network device logs. 

Firstly, following existing studies in software system logs \cite{zhu2023loghub,he2021survey}, we evaluate LUK on two widely researched log analysis tasks to validate the representativeness of our approach: anomaly detection and failure identification. 

Secondly, we conduct experiments on network device logs to investigate the model's generalization ability. This domain poses additional challenges due to the presence of various vendors and highly specialized logs. Due to the lack of public tasks on network device logs, we construct four different downstream tasks referring to \cite{ma2024knowlog}. 
These tasks are commonly encountered by engineers and require substantial expert knowledge for effective solutions.


\textcolor{blue}{
The evaluation datasets in our experiments include two types: including in the pre-training corpus and not including in the pre-training corpus. For most datasets, we collect the evaluation datasets from the same source as the pre-training data.
Moreover, 
apart from logs involved in pre-training, to verify the generalization capability of LUK, we collect more logs that are not included in the pre-training for evaluation.}
In Table \ref{tab:software_statistics} - \ref{tab:network_statistics} we provide statistics for different tasks of their datasets. Next, we give an introduction to each task and its evaluation metrics.
\subsubsection{Downstream Tasks of Software System Logs} 


\begin{itemize}
    \item \textbf{Anomaly Detection (AD).} Anomaly detection is a widely researched log analysis task to predict whether anomalies exist within a short period of log messages, where the input is a log sequence and the output is True or False.  Following Biglog \cite{tao2023biglog}, we concatenate each log in the sequence and then input them to the encoder to obtain the representation of the sequence.
    
    \textbf{Dataset and Metric.} Following previous anomaly detection studies \cite{le2021log,le2022log}, we collect datasets from Loghub \cite{zhu2023loghub}. To measure the effectiveness of different models in anomaly detection, we report \textit{Precision}, \textit{Recall}, and \textit{F1} on the True (anomaly) class as evaluation metrics.
    
    \item \textbf{Failure Identification (FI).} Failure identification aims to further discern the type of failure present in the anomaly log. Given the log messages, the model is required to determine what error emerges. 

    \textbf{Dataset and Metric.} This dataset comes from \cite{cotroneo2019bad}, which is an OpenStack dataset including 396 failure tests and 16 kinds of API errors, such as ``network delete error'', ``openstack network create error''. Usually, engineers are interested in whether top-K recommended results contain the correct error, hence, we report the \textit{Recall@K} rate as the evaluation metric.
    
\end{itemize}


\begin{table*}[]
\centering
\caption{Examples of Module Classification (MC) and Fault Phenomenon Identification (FPI).}
\label{tab:tasks}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{l|cl}
\toprule[1pt]
Tasks                & \multicolumn{2}{c}{Example}                                                                                                                                                                                                                                                                                                                                          \\ \midrule
\multirow{4}{*}{MC}  & \textbf{Input}  & \begin{tabular}[c]{@{}l@{}}{[}MASK{]}/6/NOTIFY\_RECV: The router received a NOTIFICATION from the peer. (Peer={[}peer-address{]}, \\ SourceInterface={[}SourceInterface{]}, ErrorCode={[}error-code{]}, SubErrorCode={[}sub-error-code{]}, NotifyInfo={[}notify-info{]},\\ VpnInstance={[}VpnInstance{]}, ErrorData={[}error-data{]})\end{tabular} \\
                     & \textbf{Output} & BGP                                                                                                                                                                                                                                                                                                                                                \\ \cmidrule{2-3} 
                     & \textbf{Input}  & {[}MASK{]}-3-DUPLICATE\_IFINDEX:\%s has \%d duplicate ifIndices.                                                                                                                                                                                                                                                                                   \\
                     & \textbf{Output} & SNMP  \\ \midrule
\multirow{4}{*}{FPI} & \textbf{Input}  & \begin{tabular}[c]{@{}l@{}}OSPF/4/CONFLICT\_ROUTERID\_INTF: OSPF router ID conflict is detected on the interface.(ProcessId=1, RouterId=\\ 10.26.09.101, AreaId=0.0.0.0, InterfaceName=10GE1/0/11, IpAddr=10.26.10.1, PacketSrcIp=10.26.10.2)\end{tabular}                                                                                         \\
                     & \textbf{Output} & Router\_id\_conflict                                                                                                                                                                                                                                                                                                                               \\ \cmidrule{2-3} 
                     & \textbf{Input}  & \begin{tabular}[c]{@{}l@{}}IFNET/2/linkDown\_activ: The interface status changes. (ifName=10GE1/0/11, AdminStatus=DOWN,  OperStatus=\\ DOWN, Reason=The interface is shut down, mainIfname=10GE1/0/11)\end{tabular}                                                                                                                                \\
                     & \textbf{Output} & Trunk\_link\_down \& Physical\_link\_down                                                                                                                                                                                                                                                                                                          \\ \bottomrule[1pt]
\end{tabular}%
}
\end{table*}


\begin{table*}[]
\centering
\caption{Examples of Log and Description Semantic Matching (LDSM) and Log and Possible Cause Ranking (LPCR).}
\label{tab:tasks2}
\resizebox{0.85\textwidth}{!}{%
\begin{tabular}{c|cl}
\toprule[1pt]
\multicolumn{1}{l|}{Tasks}                 & \multicolumn{2}{c}{Example}                                                                                                                                                                                                                                                                                                     \\ \midrule
\multirow{4}{*}{LDSM}                      & \textbf{Input}  & \begin{tabular}[c]{@{}l@{}}{[} ARP/4/ARP\_VLAN\_SPEED\_LMT: The VLAN's ARP packet speed exceeded the configured speed limit value. \\ (SuppressValue={[}SpeedLmtValue{]}, Vlan={[}VlanId{]}) , \\ The transmit rate of ARP packets in a VLAN exceeded the configured rate limit in the VLAN. {]}\end{tabular} \\
                                           & \textbf{Output} & True                                                                                                                                                                                                                                                                                                          \\ \cmidrule{2-3} 
                                           & \textbf{Input}  & \begin{tabular}[c]{@{}l@{}}{[}(ARP/4/ARP\_VLAN\_SPEED\_LMT: The VLAN's ARP packet speed exceeded the configured speed limit value. \\ (SuppressValue={[}SpeedLmtValue{]}, Vlan={[}VlanId{]}) , \\ A received ARP packet was not an ARP reply packet in response to the ARP request packet sent by the device. 
 {]}\end{tabular}       \\
                                           & \textbf{Output} & Fasle                                                                                                                                                                                                                                                                                                         \\ \midrule
\multirow{4}{*}{LPCR}                      & \textbf{Input}  & \begin{tabular}[c]{@{}l@{}}BGP/3/FSM\_UNEXPECT: FSM received an unexpected event. (FSM={[}fsm-name{]}, PreState={[}prev-state{]}, \\ CurrState={[}curr-state{]}, InputEvent={[}input{]})\end{tabular}                                                                                                         \\
                                           & \textbf{Output} & It is caused by an internal error of the system.                                                                                                                                                                                                                                                              \\ \cmidrule{2-3} 
                                           & \textbf{Input}  & \begin{tabular}[c]{@{}l@{}}BGP/2/hwBgpPeerSessionExceed\_clear: The number of BGP peer sessions decreased below the maximum number. \\ (MaximumNumber={[}MaximumNumber{]}, CurrentNumber={[}CurrentNumber{]})\end{tabular}                                                                                    \\
                                           & \textbf{Output} & The number of BGP peer sessions fell below the upper limit.                                                       \\ \bottomrule[1pt]
\end{tabular}%
}
\end{table*}

\subsubsection{Downstream Tasks of Network Device Logs}


To intuitively understand these tasks, we give examples of each task in Table \ref{tab:tasks} - \ref{tab:tasks2}.
\begin{itemize}
    \item \textbf{Module Classification (MC).} MC is a log-single task aiming at identifying which module the log originates from, which input is a log with the masked module name and the output is the corresponding module name. 

    \textbf{Dataset and Metric.} We collect the log from Table \ref{tab:network_statistics} and replace the module name with \textit{[MASK]} as input, the module name in the log as ground truth. Obviously, this is a multi-classification task and the model needs to understand the contextual information of the logs to accurately identify their source.
    As an unbalanced multi-class classification task and considering the importance of different classes, we report \textit{Accuracy} and \textit{Weighted F1} as evaluation metrics.
    
    \item \textbf{Fault Phenomenon Identification (FPI).} FPI is also a log-single task to identify the fault category to which the log belongs. Different from the previous failure identification task, FPI is a multi-label classification task due to a log may appear in more than one fault category.
    
    \textbf{Dataset and Metric.} We collect 602 Huawei switches logs covering 43 fault categories from real-world as the dataset, these logs are annotated by experts. Unlike the multi-class classification task, we report \textit{Average Accuracy} of all samples \cite{sorower2010literature} as the evaluation metric, where the accuracy for each sample is the number of correctly predicted labels.

     
    \item \textbf{Log and Description Semantic Matching (LDSM).} LDSM is a log-pair task aimed at determining whether the semantics of a given log align with the corresponding natural language description, where the input is a log and description pair, and the output is True or False.

    \textbf{Dataset and Metric.} We collect descriptions of logs from the documentation, then we build (log, description) pair as ground truth and randomly select one other description for each log as a negative sample. This task requires the model to accurately understand the semantics of the logs and descriptions. As a binary classification task, both positive and negative cases require attention, we report the \textit{Accuracy} and \textit{Weighed F1} as evaluation metrics.
    
    \item \textbf{Log and Possible Cause Ranking (LPCR).} LPCR is a log-pair ranking task to find the most probable answer from a list of possible causes for a given log. \textcolor{blue}{
    Specifically, the input is a log and an answer candidate set, then the model needs to find the most probable causes from the set and rank the candidate set based on the priority as the output. }

    \textbf{Dataset and Metric.} We collect logs and the corresponding possible causes from the Huawei public documentation and build (log, possible cause) pairs as ground truth. Then we randomly select 15 possible causes of other logs the ground truth as a candidate set. This task necessitates that the model understands the background information of the log to accurately identify its potential causes. As a typical ranking task, following \cite{niu2022spt}, we report \textit{Precision@K} and \textit{Mean Reciprocal Rank} (MRR) as evaluation metrics, where MRR is a statistic measure for evaluating search algorithms. 
\end{itemize}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table*}[]
% \caption{The prompts of ChatGPT and Llama2 used for each task.}
% \centering
% \label{tab:prompts}
% \resizebox{0.85\textwidth}{!}{%
% \begin{tabular}{l|l}
% \toprule[1pt]
% Tasks                                                                            & \multicolumn{1}{c}{Prompt Template}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Anomaly\\ Detection\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}You are a professional Operations Engineer, determine whether an anomaly exists in the given log sequence, \\ and output True if it exists and False if it does not. \\ Input log sequence: \{\}\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Failure \\ Identification\end{tabular}                & \begin{tabular}[c]{@{}l@{}}You are a professional Operations Engineer, identify the 3 most possible causes of the given log from the following\\ 16 error causes. Requirement: the most possible error causes are ranked first. \\ The error causes and their corresponding numbers are as follows:{[}’openstack server add volume’: 0, ’cinder list’: 1,\\ ’openstack volume list’: 2, ’openstack volume create’: 3, ’openstack network set’: 4, ’openstack network create’: 5, \\ ’openstack floating ip create’: 6, ’openstack subnet create’: 7, ’openstack router add subnet’: 8, ’openstack network delete’: 9, \\ ’openstack security group create’: 10, ’openstack domain create’: 11, ’openstack server create’: 12, ’openstack server reboot’: 13, \\ ’nova list’: 14, ’openstack keypair create’: 15{]} \\ Directly outputs the sorted result of the number corresponding to the error cause of the given log, e.g., 3, 10, 6. \\  Input Log: \{\}\end{tabular} \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Module \\ Classification\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}You are a professional Operations Engineer, Please determine which module the log comes from. \\ Requirement: choose one answer to output from all the modules.  All modules:{[} {]}.  \\ Input Logs: \{\}\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Log and Description \\ Semantic Matching\end{tabular} & \begin{tabular}[c]{@{}l@{}}You are a professional Operations Engineer, Please determine whether the given log and the description semantics match, \\ output True if they match, output False if they don’t. \\ Input Log:\{\}, Description: \{\}\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ \midrule
% \begin{tabular}[c]{@{}l@{}}Log and Possible\\ Cause Ranking\end{tabular}         & \begin{tabular}[c]{@{}l@{}}You are a professional Operations Engineer, Please determine the possible causes of the given log. \\ Requirement: Score each of the possible causes out of 100. \\ Input Log: \{\}, Possible Causes: {[}{]}\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ \bottomrule[1pt]
% \end{tabular}%
% }
% \end{table*}

\subsection{Baselines}

\textcolor{blue}{
We categorize baselines for log understanding into four groups according to technology type: traditional deep-learning methods, pre-trained language models, knowledge distillation methods, and large language models. In addition, to ensure a fair comparison, apart from LLMs, we re-produce all baselines from their repositories, and the parameters of baseline models are according to their original settings. } 
% knowledge distillation
% For large language models-based baselines, we 
% , following, we select top-5 examples from
% the training set for each input log and use the same embedding model as ECR to select examples.}
% Considering that ICL suffers from unstable results due to example selection \cite{kaddour2023challenges, lu2022fantastically} and well-designed in-context is not the focus of this paper, to compare with the stable result, we utilize the zero-shot capability of LLMs for log analysis.
\subsubsection{\textcolor{blue}{Traditional deep-learning methods}} 
\textcolor{blue}{Traditional deep-learning methods convert each log message into a vector with the word embedding model and then input the vector to a deep neural network (CNN or BiLSTM) to analyze logs. Following previous works \cite{zhang2019robust, lu2018detecting}, We choose the most widely used \textbf{BiLSTM} and \textbf{CNN} for log analysis as deep neural network building models.}

\subsubsection{\textcolor{blue}{Pre-trained language models}}
\textcolor{blue}{Pre-trained language model-based log analysis methods follow the \textit{pre-train and fine-tune} paradigm, where one pre-trained language model serves as the backbone, and then is fine-tuned on different specific downstream tasks. We select one general pre-trained model (\textbf{BERT \cite{le2021log,lee2023lanobert}}) and two specific pre-trained models for logs (\textbf{Biglog \cite{tao2023biglog}} and \textbf{KnowLog \cite{ma2024knowlog}}) as baselines.
\textbf{Biglog} excels in capturing essential features due to its extensive training on the log corpus. In addition, \textbf{KnowLog} is the state-of-the-art log pre-trained model in log analysis not only due to pre-training on log corpus but also enhancing the pre-training with documentation knowledge. Referring to KnowLog, we collect the descriptions of logs from the Huawei and Cisco public
documentation as background knowledge to enhance the log
pre-training in the same way.
For fairness, we reproduce Biglog and KnowLog with the same pre-training setting on our log corpus. 
}

\subsubsection{\textcolor{blue}{Knowledge distillation methods}}
\textcolor{blue}{
In the era of LLMs, data augmentation (DA) is the prevalent paradigm to achieve knowledge distillation of LLMs, where it prompts the LLM to generate more data tailored to train the student model in a targeted skill or domain \cite{taori2023stanford,xu2024survey}. This reasoning process-oriented distillation method is more effective compared to obtaining labels directly from the teacher model \cite{zhu2024distilling}.
Considering the lack of research on knowledge distillation in the field of log analysis, we select Chain-of-Thought (COT)-based knowledge distillation as the baseline, which has proven to be an effective knowledge distillation method for the reasoning process in the field of NLP \cite{hsieh2023distilling,shridhar2023distilling}.
}

\textcolor{blue}{
Specifically, we select \textbf{T5 \cite{raffel2020exploring}} (\textit{t5-base with 223M parameters})  as the student model, and GPT-4o as the teacher model.  Given the specific log analysis task, we provide the inputs and labels from the training set to the teacher model, then utilize COT prompting to extract rationales from the teacher model. Finally, the student model is trained with the inputs and constructed rationales. }

\subsubsection{\textcolor{blue}{Large language models}}
\textcolor{blue}{LLM-based log analysis methods follow the \textit{in-context learning} paradigm, where LLMs make predictions based on contexts augmented with a few examples without training.
Following previous LLM-based log analysis works \cite{xu2024divlog,xu2024unilog,liu2023logprompt,jiang2023llmparser}, we select top-5 similar examples from the training set for each input log and use \textit{bge-large-en-v1.5} as the embedding model to select examples, due to its excellent performance among all open-source embedding models. Considering the recency bias of LLMs \cite{zhao2021calibrate}, we arrange these examples in ascending order based on the cosine similarity. We select two proprietary LLMs (\textbf{ChatGPT} and \textbf{GPT-4o}) and one powerful open-source LLM (\textbf{LLama3-70B \cite{dubey2024llama}}) as baselines. We utilize HTTP requests to invoke the OpenAI APIs and interact with proprietary LLMs. For open-source LLM, we deploy \textit{Llama-3.3-70B-Instruct} in our environments to analyze logs.}

In addition, since \textbf{COT} prompting \cite{wei2022chain} is verified to improve the performance of LLMs significantly. To verify the effectiveness of multi-expert collaboration, we acquire knowledge with COT and then train the model with the same pre-training tasks for comparison. 
The specific prompt is: \textit{You are an engineer in the maintenance and operation domain, Please help me understand this log, including parameters, description, possible causes and resolution procedures. Let's think step by step.}

==> sections/discussion_revision.tex <==

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Qualitative examples of LUK and baselines. We calculate the cosine similarity as the score to analysis.}
\label{tab:example}
\tabcolsep=0.07cm
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{l|c|l|ll}
\toprule[1.5pt]
Label                    & Index              & \multicolumn{1}{c|}{Examples}                                                                                                & Models & Score          \\ \midrule
\multirow{6}{*}{Match}   & \multirow{3}{*}{1} & \textbf{Log:} \textcolor{blue}{OPSA/3/OPS\_}CLI\_CLOSE\textcolor{blue}{\_FAIL: Failed to} stop the terminal \textcolor{blue}{using the script.}                                             & BERT   & 0.671          \\
                         &                    & (Script={[}script-name{]}, event={[}event-name{]}, instance={[}instance-id{]},terminal={[}cli-id{]})                         & Biglog & 0.624          \\
                         &                    & \textbf{NL Description:} There was a failure in stopping the terminal using a specific script.                                        & LUK    & \textbf{\color{blue}0.740} \\ \cmidrule{2-5} 
                         & \multirow{3}{*}{2} & \textbf{Log:}  SYSTEM/4/SYS\_IMAGE\_ERROR: The next startup image \textcolor{blue}{package is error}. (imageIndex={[}imageIndex{]},                                                  & BERT   & 0.723          \\
                         &                    &  curImageName={[}curImageName{]}, nextImageName={[}nextImageName{]}, errReason={[}errReason{]}) & Biglog & 0.629          \\
                         &                    & \textbf{NL Description:} An error occurred in the next startup image package.                                                         & LUK    & \textbf{\color{blue}0.788}          \\ \midrule
\multirow{6}{*}{UnMatch} & \multirow{3}{*}{1} & \textbf{Log:} \textcolor{blue}{OPSA/3/OPS\_}TERMINAL\_WRITE\textcolor{blue}{\_FAIL: Failed to} display the string on the                                                  & BERT   & 0.657          \\
                         &                    & terminal \textcolor{blue}{using the script.} (Script=xx,event=xx, instance=xx, string=xxx, terminal=xx)                                        & Biglog & 0.646          \\
                         &                    & \textbf{NL Description:} There was a failure in stopping the terminal using a specific script.                                        & LUK    & \textbf{\color{blue}0.514} \\ \cmidrule{2-5} 
                         & \multirow{3}{*}{2} & \textbf{Log:} TRILL/4/TRILL\_RECV\_ERR\_PKT: TRILL-INFO: Drop \textcolor{blue}{error packet.} (PktType={[}PktType{]},                                   & BERT   & 0.671          \\
                         &                    & ProcessId={[}ProcessId{]}, ErrReason={[}ErrReason{]}, ErrCount={[}ErrCount{]}, InterfaceName={[}InterfaceName{]})            & Biglog & 0.486          \\
                         &                    & \textbf{NL Description:} An error occurred in the next startup image package.                                                                         & LUK    & \textbf{\color{blue}0.077}          \\ \bottomrule[1.5pt]
\end{tabular}%
}
\end{table*}

\subsection{Qualitative Analysis}
To show the usefulness of LUK more intuitively,  we select two representative cases for qualitative analysis. Specifically, we employ a pre-trained model to obtain embedding representations of the input log and natural language (NL) description, then calculate cosine similarity as the score to demonstrate their capability of semantic understanding. As shown in Table \ref{tab:example}, to provide a challenge in the case, we deliberately select logs with closer events and then compute their similarity to the description, which is matched only with one log.

From this case, we notice that: For the matched example, BERT demonstrates better performance, whereas Biglog's performance is comparatively weaker when compared to BERT. This suggests that only pre-training on logs makes it challenging to capture log semantics adequately without external knowledge and this may enlarge the semantic differences between logs and natural language. In contrast, LUK achieves the highest similarity score on the matched example and the lowest similarity score on the unmatched example, which can infer that benefiting from expert knowledge, LUK exhibits superior proficiency in capturing log semantics for log understanding. It also verifies the effectiveness of knowledge acquisition from LLMs. For the unmatched example, both BERT and Biglog exhibit significantly weaker performance compared to LUK, which implies that BERT and Biglog have limitations in recognizing log semantics. These results reveal the remarkable performance of LUK in log understanding.


\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{new_fig/luk_evaluation_example.pdf}
   % \vspace{-6mm}
   \caption{\textcolor{blue}{An complete workflow of the MEC framework to construct knowledge.}}
   % \vspace{-4mm}
   \label{fig:evaluation_case}
\end{figure*}

\begin{figure}[]
    \centering
    % \vspace{-2mm}
    \subfloat[GPT-4o]{\label{fig: system type 
    forgetting}
    % \vspace{-5mm}
    \includegraphics[width=0.5\linewidth]{new_fig/error_percent_gpt4o.pdf}}    
    \subfloat[LLama3-70B]{\label{fig: system type zero}
    % \vspace{-5mm}
    \includegraphics[width=0.5\linewidth]{new_fig/error_percent_llama3.pdf}}
    
    \caption{\textcolor{blue}{Distributions of error categories in unsatisfactory knowledge.}}
    
    % \vspace{-5mm}
    \label{fig:different_error_precent}
\end{figure}


\subsection{Case Analysis}
\subsubsection{\textcolor{blue}{Evaluation and refinement mechanism of the  MEC framework}}
\textcolor{blue}{To intuitively understand the workflow of the MEC framework and analyze the impact of the evaluation and refinement mechanism on knowledge generation, we provide a specific case of expert knowledge construction as shown in Fig. \ref{fig:evaluation_case}, this input log from the Huawei device\footnote{\url{https://support.huawei.com/enterprise/en/doc/EDOC1100332302/fb54bda3}}.}

\textcolor{blue}{
As can be seen from the case, the \textit{Director} first meticulously analyzes the input log to give key points, and then the \textit{Executor} generates expert knowledge based on the guidance of these key points. Following knowledge creation, the \textit{Evaluator} evaluates the quality of the generated knowledge and provides feedback to the \textit{Executor} for refinement. The evaluation feedback shows that the content generated by the \textit{Executor} does not fulfill completeness and consistency. Specifically, the generated knowledge lacks of an introduction to the procedure step and the explanation of the severity level is not rigorous. In addition, there is also an uninformative explanation in the generated knowledge, which makes it more difficult for the smaller model to understand the expert knowledge.
Finally, the \textit{Executor} refines the generated knowledge based on the evaluation feedback. From the re-generated knowledge, we can find that the \textit{Executor} not only supplements the clear introduction of the procedure step but also modifies the explanation of severity level to make it more reasonable. Overall, the re-generated knowledge is more comprehensive and rigorous,  which is more conducive for the smaller model to learn expert knowledge.}

\textcolor{blue}{To more deeply reveal the issues of knowledge generated by LLMs. We count the distributions of different error categories in unsatisfactory knowledge according to \textit{Evaluator}'s results for GPT-4o and LLama3-70B, respectively. 
As shown in Fig. \ref{fig:different_error_precent}, it can be found that a significant portion of the inadequacies stems from issues related to completeness. The prevalence of completeness-related errors underscores the challenge faced by the single LLM in producing comprehensive knowledge autonomously. Moreover, alongside completeness issues, a smaller yet notable proportion of unsatisfactory knowledge is attributed to deficiencies in conciseness and consistency. This finding underscores the significance of collaborative frameworks that integrate diverse roles, each contributing unique perspectives and expertise to compensate for the capacity deficiencies of the single LLM and improve the completeness and accuracy of generated knowledge.}

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{new_fig/luk_knowledge_case.pdf}
   % \vspace{-6mm}
   \caption{\color{blue}Example of knowledge generated by GPT-4o and retrieved from documentation.}
   % \vspace{-4mm}
   \label{fig:knowledge_case}
\end{figure*}

\begin{figure}[]
\centering
    % \vspace{-2mm}
    \includegraphics[width=\columnwidth]{new_fig/LUK_percentage_1.pdf}    
    
    \caption{\textcolor{blue}{Proportion of unsatisfactory knowledge, where we employ the evaluation criteria of the MEC framework to evaluate the knowledge.}}
    
    % \vspace{-5mm}
    \label{fig:doc-knowledge-analysis}
\end{figure}

\subsubsection{\textcolor{blue}{Comparison of knowledge from different sources}} 
\textcolor{blue}{To further intuitively analyze the quality of the expert knowledge constructed with the MEC framework, we compare it with the knowledge collected from documentation and the COT-based approach. As shown in Fig. \ref{fig:knowledge_case}, we collect a Cisco log\footnote{\url{https://www.cisco.com/c/en/us/td/docs/switches/datacenter/sw/routing_messages/reference/7k_rout_mess_ref_book/7k_rout_mess_ref_2mess.html}} as the case and give the corresponding generated knowledge based on the COT and MEC methods.}

\textcolor{blue}{
As can be seen from these cases, the knowledge provided by the documentation is too simple, which provides a generic and limited understanding of the log without delving into specific details or potential causes. Although COT-based knowledge offers a more detailed explanation of the log, compared to MEC-based knowledge, there is still the problem of inadequate knowledge and lack of insight.
In contrast, the knowledge derived from the MEC framework excels in its comprehensive analysis and insights. By explicitly outlining the specifics of the log error, including the MTS queue failure and the placeholders for queue and error message, the MEC-based knowledge provides a deeper understanding of the issue at hand. Furthermore, it goes beyond mere description to identify potential root causes such as network connectivity issues.
The comparison highlights the clear advantage of the MEC framework in expert knowledge generation. Its collaborative nature allows for the integration of diverse expertise and perspectives, resulting in a more comprehensive analysis of complex logs.}

\textcolor{blue}{
To quantify the differences among the various forms of knowledge, we employ the evaluation criteria of the MEC framework to evaluate the knowledge acquired by the documentation and the knowledge constructed based on COT in the network device logs. The evaluation results are shown in Fig. \ref{fig:doc-knowledge-analysis}, revealing a notable contrast in quality between the different sources of knowledge. It is apparent from the analysis that a significant proportion of knowledge sourced from documentation falls short of meeting the evaluation requirements. This deficiency can be attributed to the inherent limitations of documentation-derived knowledge, which often lacks depth and detail, offering only the most straightforward description of the logs. Combined with Fig. \ref{fig: roundaaa}, this suggests that the knowledge acquired from MEC based on LLMs is comparable or even better than the documentation. Considering the lack of documentation support for most logs and the high cost of manually constructing knowledge, this provides a feasible way to gain a wealth of practical knowledge automatically.}

\textcolor{blue}{
Despite the advantages of the MEC framework in knowledge generation, domain-specific documentation continues to hold an indispensable role. LLMs remain struggling with knowledge gaps, especially when dealing with customized modules and terminology, leading to misconceptions. In such cases, domain documentation can bridge these gaps, providing essential context and expertise to enhance the understanding of LLMs. This symbiotic relationship allows LLMs to enrich documentation content and, in turn, enables documentation to improve the professionalism and accuracy of LLMs. We will optimize the integration of domain documentation and LLM to further enhance the knowledge acquisition process in the future.}

% From the good case, we can observe that the knowledge generated by MEC is superior to the content retrieved from the documentation. The introduction of logs in the Cisco documentation is extremely rough, whereas the knowledge acquired from MEC is more detailed and accurate, e.g., clarifying the error and adding the information of abbreviations to support understanding logs. This suggests that the knowledge acquired from MEC based on LLMs is comparable or even better than professional documentation, which provides feasibility for acquiring expert knowledge for mostly logs that lack documentation support.

% From the bad case, we also notice that the knowledge acquired by MEC lacks informativeness and has factual errors. This situation generally occurs on domain-customized logs, which do not have consensus in the universal log analysis domain.  Since it belongs to the customized module, there is no knowledge of the relevant content in LLMs, which is difficult to understand by non-specific experts, and this case can only rely on manually constructing knowledge. To mitigate this issue, we consider exploring an LLM-based retrieval-augmented language model to enhance log understanding, which can retrieve relevant information about the logs as references to LLMs and this process reduces manual annotation of knowledge. We will investigate it in future work.
 



\subsection{Threats to Validity}
\subsubsection{Construct Validity}
Since LLMs are black box models, LLMs pose a risk of generating output content that may be unreasonable, potentially impacting the accurate interpretation of logs.
\textcolor{blue}{First, to counteract the inherent randomness in the inference process of LLMs, we set the model temperature to 0. This step ensures that LLMs consistently produce results for the same inputs, mitigating variability in output.}
Second, to mitigate hallucinations of LLMs, we propose a multi-expert collaboration framework, which can work better with the power of cooperation and interaction. In particular, we design an \textit{Evaluator} in this framework, which checks the generated knowledge by evaluating completeness, consistency, and conciseness. 
\textcolor{blue}{In addition, to address the issue of ambiguous and inconsistent evaluations by LLMs under the reference-free setting, we construct contrastive examples consisting of positive and negative knowledge of the same log. By presenting these contrastive examples to the \textit{Evaluator} as reference examples, we steer the evaluation of LLMs toward our desired objectives. In cases where issues are identified, the \textit{Executor} within the framework revises or refines the generated content based on the feedback received. This iterative process helps improve the quality and reliability of the generated knowledge. We also verify the importance of the \textit{Evaluator} for acquiring high-quality knowledge in ablation studies.}


% The key of the \textit{generate-pretrain-predict} paradigm is to enhance log pre-training with the knowledge generated by the large language model. In the experiment of RQ2, we find that the background knowledge generated by different prompts has different effects on improving the log understanding. In our experiments, the large language model is a black box model, and we can not control the output of the large language model, thus there is a risk of the unreasonable content of the output, which can affect the understanding of the logs. In order to reduce the risk of errors and obtain reasonable generation, we propose a generation-selection strategy, which selects the final answer from the output of multiple prompts that are close to the majority of the content, and the effectiveness of this strategy has been demonstrated in experiments. The drawback of this strategy is that it is difficult to choose the optimal result if there is a significant difference in the generation of each prompt, which is caused by the large uncertainty of the model output. One way to solve this challenge is to incorporate expert feedback based on the active learning strategy to obtain the optimal generation, which we will research in future work.

\subsubsection{Internal Validity}
It is widely agreed that the performance of DL models is significantly affected by hyperparameters. Due to the limited computation resources, we do not search for the optimal hyperparameter settings, and instead follow the empirical settings. We acknowledge that further fine-tuning of these hyperparameters may yield better results. 

% In addition, we only collected 43,229 logs for pre-training, and more data would yield better results according to the scaling law criteria \cite{kaplan2020scaling}.

\subsubsection{External Validity}
From the perspective of enterprises, utilizing external LLMs to acquire expert knowledge may cause leakage of user privacy and internal information in logs. To alleviate this issue, on the one hand, we propose to remove sensitive information from logs and utilize log templates after log parsing to acquire knowledge. On the other hand, LUK is a general framework that can combine any LLMs, and users can also employ their own LLMs to acquire knowledge to enhance a small model for solving a specific problem. 
\textcolor{blue}{For example, apart from invoking the proprietary LLMs, we also verify the effectiveness of LUK by deploying LLama3-70B in our experiments, which is an open-source LLM.}

==> sections/introduction_revision.tex <==
\section{Introduction}
\IEEEPARstart{W}{ith} the increasing complexity and scale of IT systems,  the maintenance and operation of large-scale systems become more challenging. Logs record the valuable runtime status, they play a crucial role in troubleshooting and enable engineers to monitor system health effectively. However, the increasing volume of logs has made manual analysis a harder task \cite{zhang2021onion}. Consequently, numerous automated log analysis methods utilizing machine learning (ML) or deep learning (DL) models have been proposed to automatically analyze logs, encompassing various tasks such as log parsing \cite{zhu2019tools,dai2020logram,nedelkoski2021self,liu2022uniparser}, anomaly detection \cite{du2017deeplog,meng2019loganomaly,li2020swisslog,nedelkoski2020self,huang2020hitanomaly,han2021unsupervised,le2022log}, root cause analysis \cite{lu2017log,wang2020root,soldani2022anomaly}, failure prediction \cite{zhang2018prefix,gao2020task,cotroneo2019bad}, etc. In particular, with the recent success of pre-trained language models (PLMs) in natural language processing (NLP), especially the advent of large language models (LLMs) represented by ChatGPT and GPT-4 \cite{achiam2023gpt},  language models (LMs) have garnered significant attention in log understanding and these LM-based approaches \cite{zhu2021unilog,tao2023biglog,ma2024knowlog, le2023log, lee2023lanobert,almodovar2024logfit, xu2024divlog,xu2024unilog,liu2023logprompt,jiang2023llmparser,guo2024lemur} achieve tremendous achievements in automated log analysis due to their outstanding performance. 

% PLM-based approaches rely on annotated data to \textit{fine-tune} the model and update the parameters for a specific task, enabling them to specialize in the given task. 
% Due to the emergence capability of LLMs \cite{wei2022emergent,lu2023emergent}, the LLM-based approaches do \textit{not fine-tune} the model but leverage the in-context learning (ICL) paradigm to solve the task without updating the parameters. Currently, PLM and LLM-based approaches are two mainstream methods for understanding logs due to their outstanding performance.

% Essentially, the improvement of these methods comes from the advancements in the model's capability of log understanding.

% These PLMs are first pre-trained on a large corpus to efficiently capture contextual information in natural language and then adapted to specific tasks through fine-tuning. 

% which improves the performance of log analysis tasks These PLMs are first pre-training on a large corpus and then fine-tuning on specific tasks.
% These methods perform log analysis tasks by understanding the information in the logs. 

\begin{figure}[]
\centering
   \includegraphics[width=\linewidth]{Fig/example.pdf}
   \vspace{-3mm}
   \caption{Example of prompting ChatGPT to help understand log, which can provide detailed background information and terminology explanations and solutions. Without knowledge, the beginner fails to understand RSSI value.}
   \vspace{-3mm}
   \label{fig:understand}
\end{figure}

As language models increase in scale and gain enhanced capabilities, two mainstream paradigms have emerged for utilizing LMs in log understanding. The first one is based on PLMs, which follows the \textit{pre-train \& fine-tune} paradigm, such as BERT \cite{devlin2019bert}, fine-tuning a PLM with task-specific data and enabling it to specialize in the given task. 
Considering the need for fine-tuning with limited computational resources and cost savings, LMs in this paradigm are typically smaller in size, such as BERT with 110M parameters.
The second one is based on LLMs \textcolor{blue}{with vast scale and complexity}\footnote{We use LLM to specifically refer to the large language models over 10B parameters that utilize the ICL paradigm without fine-tuning the parameters.}\textcolor{blue}{, which can tackle a diverse array of tasks with remarkable proficiency.} The LLM-based methods follow the \textit{In-Context Learning} (ICL) paradigm \cite{dong2022survey,lu2022fantastically}, learning from a few examples in the context without updating the parameters. 

\textcolor{blue}{
Despite the powerful performance of LLMs, limited accessibility and higher costs present significant challenges in leveraging the full potential of LLMs. 
These LLMs often come with substantial
usage fees and have restricted access to data privacy and security. Even if the LLM is deployed locally, it still may face resource constraints, making LLMs
less attainable for individuals and smaller organizations.  
In addition, due to their
complex autoregressive architectures and a large number of parameters, LLM-based methods are computationally
inefficient.
Considering that modern software systems can produce several petabytes per day \cite{wang2022spine,li2024logshrink}, directly employing LLMs for log analysis is impractical due to the significant overhead of querying LLMs, such as inference time and network latency \cite{jiang2023llmparser,wang2023tabi}. 
In contrast, smaller PLMs with smaller parameters, requiring limited resource costs, are more efficient than LLMs \cite{ma2024llmparser}. 
Hence, we argue that the smaller PLM is more practical in extensive log analysis scenarios \cite{le2023log,lee2023lanobert,almodovar2024logfit}.
}




% With the advent of emergent capabilities of LMs with billions of parameters \cite{wei2022emergent,lu2023emergent}, 

% Considering the need for fine-tuning with limited computational resources and cost savings, models in this paradigm are typically smaller pre-trained models, making them more practical in real-world scenarios.

% the cost of employing LLMs is becoming an increasingly critical issue \cite{kaddour2023challenges,zhao2023survey}. 
% LLMs with billions of parameters require huge computing
% resources to fine-tune, the in-context learning (ICL) paradigm of LLMs is 
% the mainstream method to analysis logs without updating the parameters \cite{xu2024divlog,xu2024unilog,liu2023logprompt,jiang2023llmparser,guo2024lemur}.
% Nevertheless, given that modern software systems can produce several petabytes per day \cite{wang2022spine,li2024logshrink}, directly employing LLMs for log analysis is impractical due to the significant overhead of querying LLMs, such as inference time and network latency \cite{jiang2023llmparser,wang2023tabi}. Hence, employing the smaller language model in log analysis scenarios becomes essential \cite{le2023log,lee2023lanobert,almodovar2024logfit}, which requires much fewer computation resources and is more cost-saving. 

% The significant advantage of PLMs is their ability to effectively utilize annotated data from specific tasks for fine-tuning the model, making it more suitable for the given task. Compared to LLMs, many studies \cite{yang2023supervised,juneja2023small} have shown that fine-tuning can make models focus more on the specific task and outperform LLMs. In addition, these smaller PLMs have fewer parameters, resulting in more efficient fine-tuning and lower computational costs for prediction. However, PLM-based approaches have faced a bottleneck in log understanding owing to insufficient availability of expert knowledge. Due to a scarcity of rich sources for knowledge acquisition (e.g. almost unable to find relevant documents for logs coming from Loghub \cite{zhu2023loghub}), these PLMs are solely pre-trained on general or log corpora, and without knowledge including background information and terminology descriptions, it is difficult to understand valuable information from logs like experts. 

% For example, as shown in Figure \ref{fig:understand}, a beginner fails to understand RSSI values in a Mac log. 


% Despite the efficient fine-tuning of models using annotated log data, PLM-based approaches have encountered a bottleneck in log understanding owing to the inadequacy of expert knowledge. Logs are inherently concise and highly specialized terminology, expert knowledge such as the description of background and terminology, can enhance models to extract valuable information from logs like experts. For example, in a Mac log ``ARPT: 621131.293163: wl0: Roamed or switched channel, reason $\#$8, bssid 5c:50:15:4c:18:13, last RSSI -64'', without expert knowledge, a novice faces challenges in understanding RSSI values. These PLMs have relatively small parameter sizes and are solely pre-trained on general or log corpora, lacking expert knowledge to understand logs effectively.

% The current way of constructing knowledge for log analysis relies on manual construction \cite{du2016spell,he2017drain,meng2021logclass,huo2023semparser} and collection of documentation \cite{ma2024knowlog}. However, manual construction is inefficient and not all logs are documented, how to automatically obtain sufficient expert knowledge to improve log understanding is still an open question.

However, the smaller PLM encounters a bottleneck in log understanding due to the inadequacy of expert knowledge. 
Logs inherently employ concise and highly specialized terminology, 
the smaller PLM struggles to understand valuable information from logs like experts \cite{ma2024knowlog}. 
\textcolor{blue}{This issue can be attributed to the lack of rich sources for knowledge acquisition. Although KnowLog proposes to acquire expert knowledge from documentation \cite{ma2024knowlog}, most logs lack professional documentation (e.g. almost unable to find relevant documents for logs coming from Loghub \cite{zhu2023loghub}) and the manual construction of knowledge is costly and inefficient, which significantly hinders the availability of the model.
}

% (2) smaller models with fewer parameters struggle to capture knowledge \cite{wei2022emergent,lu2023emergent}.  
% Masked Language Modeling (MLM) \cite{devlin2019bert} as the widely used pre-training task for most pre-trained models, they can only perceive their own contextual information and cannot capture external knowledge.}. 

Fortunately, LLMs with extensive knowledge can understand logs comprehensively, attributing to training on massive textual data related to code \cite{peng2023generative} and logging \cite{mastropaolo2022using,li2023exploring}. For example, as depicted in Fig. \ref{fig:understand}, ChatGPT can better assist in understanding the Mac log. \textcolor{blue}{Consequently, LLMs such as GPT-4 compensate for the lack of knowledge of the smaller PLM, which can analyze logs more efficiently and professionally.}




% Fortunately, LLMs are trained on massive textual data related to code \cite{peng2023generative} and logging \cite{mastropaolo2022using,li2023exploring}, which endows LLMs with rich knowledge for understanding logs comprehensively. For example, as depicted in Figure \ref{fig:understand}, ChatGPT can assist in understanding this Mac log better. However, the direct use of LLMs for log analysis has two notable drawbacks.
% (1) High Computational Costs: utilizing LLMs for prediction is computationally expensive (e.g., deployment of the GPT3-175B model requires 326GB of GPU memory \cite{frantar2022optq}).
% (2) Unstable Performance: LLMs may generate unstable answers due to sensitivity to prompts and occurrence of hallucinations \cite{mundler2023self,manakul2023selfcheckgpt,li2023halueval}. 


% LLMs are trained by vast amounts of text data related to code
% and logging, thus having the potential to understand log messages comprehensively.
% Due to the rich implicit knowledge and powerful reasoning capabilities, LLMs show strong performance in log understanding. Many recent log analysis studies \cite{xu2024divlog,xu2024unilog,liu2023logprompt,jiang2023llmparser,guo2024lemur} employ this implicit knowledge in solving specific log tasks through the ICL  of LLMs. Despite its effectiveness, there are also two notable drawbacks associated with directly utilizing LLMs for log analysis. (1) High Computational Costs: utilizing LLMs for prediction is computationally expensive (e.g., deployment of the GPT3-175B model requires 326GB of GPU memory \cite{frantar2022optq}).
% (2) Unstable Performance: LLMs may generate unstable answers due to problems of sensitivity to prompts and hallucinations \cite{mundler2023self,manakul2023selfcheckgpt,li2023halueval}. 

% However, there is still a wealth of knowledge in LLMs, as depicted in Fi'ge'w \ref{fig:understand}, with the help of ChatGPT, we can understand this Mac log better.
% How to harness this wealth of information effectively to improve log understanding is still an open question.

To more effectively harness the knowledge embedded within LLMs for log understanding, we argue that expert knowledge can be elicited from LLMs and subsequently utilized to empower the smaller PLM, making the smaller model understand logs like experts.  However, two main challenges exist in enhancing log understanding with expert knowledge from LLMs. 
(1) \textbf{Effective Knowledge Acquisition:} 
\textcolor{blue}{Although LLMs have shown remarkable capabilities in various tasks, LLMs still have difficulty in acquiring complete and accurate knowledge due to hallucination, which may result in not covering all the depth of knowledge and there may be misunderstandings when dealing with domain-specific data \cite{mundler2023self,manakul2023selfcheckgpt}. 
In addition, in the era of LLMs, knowledge distillation (KD) \cite{xu2024survey} emerges as a pivotal methodology for transferring advanced capabilities from LLMs to smaller models. 
Compared to obtaining answers directly from the teacher's model, distillation towards the reasoning process has proved to be a more effective method \cite{xu2024survey,zhu2024distilling}.
However, current knowledge distillation methods, such as COT-based KD \cite{hsieh2023distilling,shridhar2023distilling}, struggle to acquire expert knowledge, instead imitating the teacher’s reasoning forms and ignoring the premise that reasoning requires expert knowledge. These distillation methods, which emphasize the process of reasoning and outcome, still hardly compensate for the lack of expert knowledge.}
(2) \textbf{Knowledge Enhancement:} 
\textcolor{blue}{Since logs and expert knowledge obtained from LLM are heterogeneous data, smaller models with fewer parameters and limited learning capacity struggle to capture knowledge \cite{wei2022emergent,lu2023emergent}. 
Masked Language Modeling (MLM) \cite{devlin2019bert} as the widely used pre-training task for most pre-trained models, they can only perceive their own contextual information and cannot incorporate external knowledge. In addition, KnowLog proposes an abbreviation prediction task specialized for log understanding. However, its ability only to enhance the knowledge of abbreviations in the logs is limited. It cannot adaptively perceive other important information from the knowledge to understand logs, such as the parameter knowledge of logs.
}


To overcome the above-mentioned challenges, we propose a novel knowledge enhancement framework to empower log understanding on a smaller PLM, called \textbf{LUK}. Rather than utilizing LLMs to solve specific tasks directly, LUK first acquires expert knowledge from LLMs, then enhances the log pre-training with the corresponding expert knowledge, and finally the knowledge-enhanced PLM for logs can be fine-tuned to solve downstream log analysis tasks efficiently.
\textcolor{blue}{This framework can maximize the advantages of both LLM and smaller PLMs.}


Specifically, to solve the first issue, we design a multi-expert collaboration framework to acquire expert knowledge from LLMs. Motivated by the waterfall model \cite{petersen2009waterfall} in software engineering, we build a professional team consisting of \textit{Director}, \textit{Executor}, and \textit{Evaluator}, and define the identity and responsibility of the roles through prompt, enabling LLMs to think and handle tasks just like role play. 
Then the team cooperates and interacts to construct expert knowledge.
To solve the second issue, we propose two novel pre-training tasks with knowledge enhancement to incorporate and perceive knowledge into the pre-trained model: word-level token prediction and sentence-level semantic alignment.

% construct three roles based on LLMs, and define the identity and responsibility of the roles through prompt, enabling LLMs to think and handle tasks just like role play. Second, the different roles cooperate as a team to generate expert knowledge.


To evaluate the effectiveness of LUK, we conduct experiments on the software system and network device logs, including six log analysis downstream tasks.
The experiment results show that LUK can harness knowledge from LLMs more effectively to improve log understanding and achieve state-of-the-art results on different log analysis tasks. In addition, LUK exhibits remarkable generalization and robustness in log analysis, with notable advantages in low-resource scenarios.

Our main contributions can be summarized as follows:
\begin{itemize}
    \item We propose a novel knowledge enhancement framework dubbed LUK, which leverages expert knowledge from LLMs to empower log understanding on a smaller PLM. To the best of our knowledge, we are the first to elicit expert knowledge of logs from LLMs to empower log understanding, offering a new perspective on log analysis.
    \item We design a multi-expert collaboration framework to acquire expert knowledge from LLMs automatically. Moreover, we propose two novel pre-training tasks to enhance the log pre-training on a smaller PLM with knowledge, which requires less computation costs to predict than solving specific tasks with LLM directly.
    \item LUK achieves state-of-the-art results on different log understanding tasks proving the effectiveness of acquiring knowledge from LLMs to empower log understanding. Moreover, LUK demonstrates significant generalization and robustness in log analysis, particularly showcasing distinct advantages in low-resource scenarios.
\end{itemize}
% \IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
% for IEEE journal papers produced under \LaTeX\ using
% IEEEtran.cls version 1.8b and later.
% % You must have at least 2 lines in the paragraph with the drop letter
% % (should never be an issue)
% I wish you the best of success.

% \hfill mds
 
% \hfill August 26, 2015





\section{Related Work and Motivation}

\subsection{\textcolor{blue}{Pre-trained Language Models for Log Analysis}}
Pre-training is the key to the success of the PLMs and LLMs, where a language model is first trained on the extensive corpus with effective pre-training tasks to capture general knowledge and then be adapted to solve different downstream tasks \cite{bai2021pre,niu2022spt}. 
The emergence of BERT \cite{devlin2019bert} heralds the success of the \textit{pre-train \& fine-tune} paradigm in natural language. Such language models improve the model's ability on a specific task by fine-tuning using task-specific objective functions after pre-training. 
Many studies \cite{gu2021domain,beltagy2019scibert,gururangan2020don} have demonstrated that pre-training on domain corpus and fine-tuning with supervised data can improve performance on a specific task, even outperforming LLMs \cite{yang2023supervised,juneja2023small}.
In the field of log analysis, many studies including pre-training on log corpus \cite{zhu2021unilog,tao2023biglog,ma2024knowlog,guo2021logbert} and fine-tuning on log analysis tasks \cite{lee2023lanobert,almodovar2024logfit} have demonstrated the effectiveness of the pre-trained model for log analysis. 

However, training solely on general or log corpus struggles to further improve log understanding due to the lack of expert knowledge. KnowLog \cite{ma2024knowlog} firstly proposes to enhance log understanding by integrating expert knowledge during the pre-training phase. Nevertheless, KnowLog's usage scenarios are limited as it heavily relies on documentation created by human experts to acquire knowledge. In contrast, this work addresses more generalized log analysis scenarios where logs are available without accompanying expert knowledge.
\textcolor{blue}{
In addition, these pre-trained models rely on the existing Masked Language Modeling (MLM) as the pre-training task, they only perceive their own contextual information and are unable to integrate external knowledge.
Although KnowLog also proposes the abbreviation prediction task, this method cannot adaptively perceive other knowledge than the abbreviation. Considering the abundance of knowledge required for log understanding, hence, we also investigate making the PLM adaptive in perceiving useful information from the knowledge during pre-training.}

% In this paper, following the \textit{pre-training \& fine-tuning} paradigm, we pre-train on log corpus with a smaller language model and design novel pre-training tasks to incorporate expert knowledge into the model. In addition, this log PLM can be fine-tuned on downstream tasks with less computational costs compared to LLMs.

\subsection{\textcolor{blue}{Large Language Model for Log Analysis}}
\textcolor{blue}{Large language models (LLMs), representing a remarkable advancement in artificial intelligence, have been trained on diverse corpora, enabling them to generate human-like text and provide accurate responses to queries \cite{kasneci2023ChatGPT}. Notably, the recent introduction of transformative models like ChatGPT and GPT-4, characterized by their enormous scale and alignment with human feedback, presents a novel opportunity for enhancing software engineering tasks \cite{white2023prompt,le2023log,feng2024prompting,wang2024software}.
}
LLMs can learn from the prompt context without training the model, which is called In-context Learning (ICL) \cite{brown2020language}. Furthermore, research has shown that augmenting the size of LLMs significantly boosts their capacity for knowledge encoding and reasoning \cite{wei2022chain, wei2022emergent}.
Due to the outstanding abilities of LLMs, many recent studies \cite{xu2024divlog,xu2024unilog,liu2023logprompt,jiang2023llmparser,guo2024lemur} utilize the ICL paradigm of LLMs for different log analysis tasks without fine-tuning the model and make tremendous achievements in log analysis tasks. 

\textcolor{blue}{However, restricted accessibility, higher costs, and computational inefficiency limit the widespread use of LLM in real-world scenarios. For example, the GPT-3 model with 175 billion parameters requires 326GB of GPU memory to deploy \cite{frantar2022optq}. Given the enormous data volumes produced by modern software systems daily, the overhead of querying LLMs, including inference time and network latency, renders direct application of LLMs for log analysis impractical. In contrast, small PLMs with smaller parameters are more efficient compared to LLMs \cite{ma2024llmparser}.} We argue that the smaller PLM can make predictions better in log analysis tasks given sufficient expert knowledge. In this paper, we guide LLMs as domain experts with prompts and explore how to effectively acquire and utilize expert knowledge from LLMs to empower log understanding. 



% However, the computational costs associated with making predictions using LLMs remain challenging in real-world application scenarios. For example, the GPT-3 model with 175 billion parameters requires 326GB of GPU memory to deploy \cite{frantar2022optq}. In addition, the results generated by LLM may be unreliable due to the inherent hallucination problem. Rather than directly utilizing LLMs for specific log analysis tasks, we argue that the smaller PLM can make predictions better in log analysis tasks given sufficient expert knowledge.  In this paper, we guide LLMs as domain experts with prompts and explore how to effectively acquire and utilize expert knowledge from LLMs to empower log understanding.

==> sections/methods_revision.tex <==
\begin{figure}[]
\centering
   \includegraphics[width=\linewidth]{Fig/overview.pdf}
   \vspace{-3mm}
   \caption{Conceptual overview of LUK.}
   \vspace{-3mm}
   \label{fig:overview}
\end{figure}


\section{Method}

\subsection{Overview}
Fig. \ref{fig:overview} shows the conceptual overview of LUK, which consists of three phases: knowledge acquisition, knowledge-enhanced pre-training, and fine-tuning with downstream tasks.
Specifically, in the first stage, we collect various logs as input, and then we design a multi-expert collaboration framework based on LLMs to acquire expert knowledge of logs.
In the second stage, we take the raw logs and the corresponding expert knowledge as input. To effectively leverage expert knowledge to empower log understanding on a smaller model, we enhance the log pre-training with knowledge based on BERT-base and propose two pre-training tasks on word level and sentence level.
Finally, a specific PLM for logs is obtained, which can be fine-tuned on downstream tasks to solve log analysis tasks.  
In the following sections, we describe the details of LUK.

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{Fig/expert-framework.pdf}
   \vspace{-3mm}
   \caption{\textcolor{blue}{Framework of multi-expert collaboration, which consists of three experts. First, the \textit{Director} meticulously analyzes the input logs to discern key points. Subsequently, the \textit{Executor} utilizes these key points
to create detailed content. Finally, the \textit{Evaluator} evaluates the quality of the generated content. In cases where the evaluation result is unsatisfactory and improvements are needed, the \textit{Evaluator} provides feedback to the \textit{Executor} for refinement. }}
   \vspace{-3mm}
   \label{fig:multi-expert}
\end{figure*}



% cognitive synergy 
\subsection{Multi-Expert Collaboration Framework}
\textcolor{blue}{Hallucination is an inherent flaw of LLMs, which may lead to incomplete or incorrect generation, ultimately failing to fulfill
the intended requirements. To construct comprehensive and accurate expert knowledge with LLM,} motivated by \textit{cognitive synergy} \cite{goertzel2009cognitive} and \textit{teamwork theory} \cite{katzenbach2015wisdom}, humans can leverage the power of collaboration and interaction to solve complex problems. As shown in Fig. \ref{fig:multi-expert},  we design a multi-expert collaboration (MEC) framework, where we assign LLMs to different roles, and these roles collaborate to generate effective expert knowledge.

\subsubsection{Role Design}
Based on the classical waterfall model \cite{petersen2009waterfall} in software engineering, we design a similar waterfall model to analyze logs consisting of three stages: analysis, execution, and evaluation. Thus, we build a professional team based on LLMs and define clear goals for each role, comprising a \textit{Director}, \textit{Executor} and \textit{Evaluator}. 

\textcolor{blue}{
It is widely acknowledged that one key capability of LLMs is to follow input natural language instructions or prompts \cite{zhou2023instruction,li2024evaluating}, hence they can customize the output to the specific needs of the user.
As shown in Fig. \ref{fig:multi-expert}, the prompt design methodology involves the pre-definition of role cards to allocate distinct roles and responsibilities to LLMs. These role cards encompass character identity, task objectives, requirements, and input queries. Initially, the LLM is assigned a character identity to emulate a specific expert role. This step enables the model to adjust its output to match the expertise and responsibilities associated with the designated role. Subsequently, the task objective is delineated to direct the LLM towards fulfilling the corresponding responsibilities aligned with the assigned character identity. Moreover, the requirement outlines the anticipated outcome or characteristics that the generated content must exhibit. These criteria may encompass aspects such as reasoning strategies, informativeness, or other pertinent factors crucial to the task at hand. Lastly, the inclusion of an input query or data serves to contextualize the task for the LLM by presenting specific information or scenarios that the model should engage with or respond to.
}

\textcolor{blue}{
By integrating these components into the prompt design framework, we can effectively guide the LLM in generating responses that are tailored to specific roles, tasks, and desired outcomes.}
These three different roles are assigned the following tasks: 
\begin{itemize}
    \item \textbf{\textit{\textcolor{blue}{Director}}.} 
    \textcolor{blue}{The \textit{Director}'s primary objective is to establish a comprehensive high-level framework aimed at providing a strategic overview to drive the team's efforts in understanding logs. This role outlines the key points essential for log understanding, thus ensuring that essential insights are highlighted and comprehensively addressed.}
    \item \textbf{\textit{\textcolor{blue}{Executor}}.} \textcolor{blue}{As the central role of this team, the \textit{Executor} is tasked with the detailed execution of the log analysis process. By receiving key points from the Director and feedback from the Evaluator, the Executor undertakes content generation and refinement two critical responsibilities.  Firstly, the Executor generates content intricately aligned with the outlined key points. Secondly, the Executor refines and polishes the content based on feedback, enhancing the knowledge quality.}
    \item \textbf{\textit{\textcolor{blue}{Evaluator}}.} \textcolor{blue}{The Evaluator assumes the crucial responsibility of ensuring the quality and adherence of generated content to predefined requirements. 
    We define three evaluation requirements for the \textit{Evaluator} to scrutinize the Executor's generation on three fundamental aspects: completeness, consistency, and conciseness. By evaluating content against these criteria, the Evaluator validates the accuracy and completeness of the generated knowledge.}

\end{itemize}

% We specialize the LLM into different roles by prompting. Specifically, 





\subsubsection{\textcolor{blue}{Dehallucination with Self-Evaluation}}
\textcolor{blue}{LLM Hallucinations seriously affect the accuracy and quality of outputs \cite{dhuliawala2023chain,huang2023survey}. Given the propensity of LLM-generated content to exhibit deficiencies in comprehensiveness and informativeness, ensuring the superior quality of directly generated knowledge poses a significant challenge.
To mitigate the hallucination of LLM and ensure the quality of expert knowledge, we build the role of an \textit{Evaluator} in the MEC framework and define three evaluation aspects to evaluate the quality of generated knowledge automatically,
which encourages the LLM to actively seek more detailed suggestions from the self-evaluation before delivering a formal response.
However, the MEC framework runs under the challenging reference-free setting and the evaluation requirements cannot be directly quantified through metrics, the LLM tends to generate ambiguous and inconsistent evaluations without fine-grained distinguishability, causing unsatisfactory evaluation performance \cite{zheng2023judging,ke2024critiquellm}.
}

\textcolor{blue}{
To address the evaluation weaknesses of the LLM, we provide evaluation examples as the reference in the \textit{Evaluator} prompt. 
By providing specific examples, the \textit{Evaluator} uses them as the basis for evaluation, thus better steering the evaluation of LLMs towards our desired goals.
Considering that the single type of example makes the LLM biased, motivated by contrastive learning techniques \cite{gao2020dialogue,radford2021learning}, we construct \textbf{contrastive examples} consisting of positive and negative knowledge of the same log to \textit{Evaluator} as reference examples, where the positive example showcases the desired knowledge, while the negative example highlights the unsatisfactory knowledge that should be avoided.  
By analyzing both types of examples before generating the evaluation, the \textit{Evaluator} can reason about our evaluation requirements and make a more informed decision about how to evaluate. }

\textcolor{blue}{
Specifically, we select one log $L$ with high-quality knowledge $K_{pos}$ as the positive example, which can be manually constructed by experts or generated from the LLM and manually confirmed. Considering that negative examples $\{K_{neg}\}_{c=1} ^ C, C=3$ of the log $L$ are unavailable directly, to construct the negative examples automatically, we propose to prompt the LLM to modify the positive knowledge making it unsatisfactory for evaluation.
As shown in Fig. \ref{fig:negative_template}, we first give the background in the prompt and then clarify the task of modifying knowledge for the LLM, where we can specify which evaluation metrics are not fulfilled. Next, we provide the raw log, the raw positive knowledge, the key points, and the three evaluation requirements in the prompt.
Finally, we require the LLM to give the reason for not fulfilling the evaluation requirements while generating the modified content, which not only improves the reasoning ability of the \textit{Evaluator} but also provides guidance for the revision of the content by \textit{Executor}.
In cases where the LLM-generated negative examples do not capture the characteristics we want to avoid, this can be manually checked, and feedback can be given to the LLM to re-generate negative samples. 
To avoid the higher expense of the longer prompt, we construct one positive knowledge and its corresponding three negative knowledge as reference examples to be provided to the \textit{Evaluator}. 
The contrastive examples we constructed in our experiments are in Fig. \ref{fig:evaluation}.
}



\begin{figure}[]
\centering
   \includegraphics[width=\linewidth]{new_fig/luk_prompt_template.pdf}
   \caption{\textcolor{blue}{Prompt template of constructing negative samples, where the underlined portion of the prompt supports user modification based on their own data and intent.}}
   \label{fig:negative_template}
\end{figure}

\subsubsection{Collaboration}
\textcolor{blue}{After constructing evaluation examples and assigning roles to LLMs, different roles start working to collaborate and interact according to the requirements in the prompt. 
First, the \textit{Director} meticulously analyzes the input logs to discern key points and formulates a plan for comprehending the logs effectively. Subsequently, the \textit{Director} shares these insights with the \textit{Executor} to guide the content generation process. The \textit{Executor} utilizes these key points to create detailed content that aligns with the requirements.
Finally, the detailed content produced by the \textit{Executor} undergoes evaluation by the \textit{Evaluator} to assess its quality. If the content meets the evaluation requirement, it is directly output as expert knowledge. In cases where the evaluation result is unsatisfactory and improvements are needed, the \textit{Evaluator} provides feedback to the \textit{Executor} for refinement.  To rigorously ensure the quality of the generated knowledge, this evaluation and refinement mechanism will be iterative until the content generated by \textit{Executor} meets the evaluation requirement or the maximum number of iterations is reached. We set up 3 iterations to build expert knowledge in our experiments. The pseudocode of the multi-expert collaboration framework is outlined in Algorithm \ref{alg:algorithm}.
}

\textcolor{blue}{ This collaborative framework manifests two pivotal advantages:
Firstly, leveraging multiple roles' collective insights and skills enables a multi-perspective analysis of the input log, 
thereby mitigating the one-sidedness and bias inherent in a single model's response acquiring more professional expert knowledge. 
Secondly, through the feedback loop mechanism, the framework enables iterative refinement of content. This iterative process of evaluation, feedback incorporation, and content enhancement promotes continuous improvement, thereby ensuring that the expert knowledge acquired is comprehensive and of high quality.}

\begin{algorithm}
\caption{\textcolor{blue}{Pseudocode of multi-expert collaboration.}}
\label{alg:algorithm}
\begin{algorithmic}
\REQUIRE \textcolor{blue}{Input Log $log$, LLM $\mathcal{M}$, Example Knowledge   $K_{pos}$}      %输入条件
\ENSURE \textcolor{blue}{Output Expert Knowledge $k$}
\STATE \textcolor{gray}{\# Construct Contrastive Examples}
\FOR{\textcolor{blue}{$c = 1$ to $C$}}
    \STATE \textcolor{blue}{$K_{neg}^c = \mathcal{M}(Prompt_{Modify}, K_{pos})$}
\ENDFOR
\STATE  \textcolor{blue}{$K_{examples} = K_{pos} \cup \{K_{neg}\}_{c=1} ^ C $}
\STATE \textcolor{gray}{\# Initial Roles}
\STATE $\mathcal{DIRECTOR} = Init\_Role(Prompt_{Dirctor}, \mathcal{M}) $
\STATE $\mathcal{EXECUTOR} = Init\_Role(Prompt_{Executor}, \mathcal{M}) $
\STATE \textcolor{blue}{$Prompt_{Evaluator} = Prompt_{Evaluator}.join(K_{examples})$}
\STATE \textcolor{blue}{ $\mathcal{EVALUATOR} = Init\_Role(Prompt_{Evaluator},  \mathcal{M})$}
\STATE \textcolor{gray}{\# Collaboration}
\STATE \textcolor{blue}{Init: $epoch = 0, feedback = False$}
\STATE $ keypoint = \mathcal{DIRECTOR}(log) $
\STATE $ content = \mathcal{EXECUTOR}(log, keypoint) $
\REPEAT
\STATE \textcolor{blue}{$ epoch = epoch + 1$}
\STATE \textcolor{blue}{$ feedback = \mathcal{EVALUATOR}(log, keypoint, content) $}
\IF{\textcolor{blue}{$feedback == False$}}
\STATE \textcolor{blue}{$ content = \mathcal{EXECUTOR}(content, feedback) $}
\ENDIF
\UNTIL{\textcolor{blue}{$epoch == Epoch$ or $feedback==True$}}
\STATE $k = content$
\RETURN $k$
\end{algorithmic}
\end{algorithm}




% In order to obtain background knowledge of logs from the LLM to help understand logs, we need to prompt a large language model to a given log. We can directly input  ``Please help me understand this log: \{Input\_Log\}'' to the LLM, then LLM will generate the corresponding background knowledge. This prompt has no extra information, such as domain-specific information and specific output content, which we call Raw prompt. However, prompts are not unique, different experts may provide different prompts. As shown in Table \ref{tab:prompts}, to explore the effect of different prompts on the results and further mine LLM's ability of log understanding, apart from raw prompt, we also propose two prompts: domain-specific prompt (DSP) and specific output prompt (SOP). 

% DSP refers to providing explicit domain scenarios in the prompt. LLMs are pre-trained on a broad corpus rather than focusing on a specific domain.
% We argue that the absence of specific information makes a gap between LLM and specific domains, which can limit its capability. To alleviate this gap and enable LLM to understand logs like a domain expert, we specify domain information in the prompt. Specifically, we prepend ``You are an engineer in the maintenance and operation domain'' to the prompt. 

% SOP refers to providing explicit output content in the prompt, which makes LLM generate more detailed background knowledge. We argue that more detailed content is better for understanding logs. Therefore, we specify the output of the LLM in the prompt. Specifically, we provide the required output in the prompt, including explanations of parameters, descriptions of logs, possible causes and resolution steps.

\begin{figure*}[]
\centering
   \includegraphics[width=\textwidth]{Fig/framework.pdf}
   \vspace{-3mm}
   \caption{The overview of LUK pre-training framework. LUK includes two novel pre-training objectives on word level and sentence level. The word-level object is designed from the perspective of domain token understanding, while the sentence-level objective is designed from overall semantic alignment.}
   % \vspace{-3mm}
   \label{fig:framework}
\end{figure*}


\subsection{Pre-Training with Knowledge Enhancement}
The overall pre-training framework is shown in Fig. \ref{fig:framework}, the input of the pre-training framework is a batch of pairs consisting of logs and the corresponding expert knowledge, then these pairs are fed into two encoders to obtain log representations and knowledge representations through two encoders respectively, \textcolor{blue}{where two encoders are initialized with the same pre-trained model. } 
Finally, \textcolor{blue}{
based on the structural characteristics of the log, we propose two pre-training tasks at word-level and sentence-level:} (1) token prediction and (2) semantic alignment, to incorporate expert knowledge for improving log understanding. 
% Since log and expert knowledge are all text, both encoders are initialized with the same pre-trained language model but do not share parameters.





%Different from MLM in BERT, TP can also perceive knowledge from $K$ for prediction. For example, in a switch log ``ERROR-DOWN/4/hwErrordown\_active: Error-down occurred. (Ifindex=[IfIndex], Ifname=[IfName], Cause=[Cause])'', suppose $Ifindex$ is masked, it is difficult to predict the semantics of $Ifindex$ from the log itself. While with external knowledge, the model can perceive that this token refers to the index of an interface, and thus can further infer that the error described by this log occurred on the interface.
%



\subsubsection{Word-Level Token Prediction}
Logs contain many domain terminologies, to sufficiently understand these domain terminologies, we propose a token prediction pre-training task (TP). Unlike existing word-level tasks of traditional PLMs only utilizing local context to predict tokens, our proposed word-level task requires models to aggregate context and knowledge for predicting tokens, leading to a knowledgeable pre-trained model.

Specifically, given a log $l$ and expert knowledge $k$ generated from the LLM, we get the corresponding input token sequence $ls= \{l_0,l_1,...,l_n\}, ks = \{k_0,k_1,...,l_m\}$ after tokenization. The token prediction task randomly masks a certain percentage (15\% in our experiments) of the log tokens $l_i$ with a special $[MASK]$ token, and then tries to recover them by perceiving external knowledge. To perceive knowledge, we design a knowledge perception module (KPM). The process of this module can be described in three steps:

Firstly, log encoder and knowledge encoder encode $ls$ and $ks$, respectively, and get the corresponding token representations $\boldsymbol{l} = \{\boldsymbol{l_0},\boldsymbol{l_1},...,\boldsymbol{l_n}\}$ and $\boldsymbol{k} = \{\boldsymbol{k_0},\boldsymbol{k_1},...,\boldsymbol{k_m}\}$.
Secondly, since not all tokens in knowledge contribute equally to the masked token prediction and to measure the importance of each token in knowledge for the token semantic, KPM calculates the semantic similarity between masked token $\boldsymbol{l_i}$ and knowledge $\boldsymbol{k}$, each token in knowledge is assigned a weight to represent its importance:
\begin{equation}
Q = W_Q\boldsymbol{l_i}, K = W_K\boldsymbol{k}, V = W_V\boldsymbol{k},
\end{equation}
\begin{equation}
\alpha = softmax(\frac{QK^T}{\sqrt{d_k}}),  \boldsymbol{k^{'}} = \alpha V,
\end{equation}
where $W_Q$, $W_K$ and $W_V$ are learnable parameter matrices, $d_k$ is the dimension of representation and $\alpha$ refers to the attention distribution. Thirdly, we concatenate the vector $\boldsymbol{l_i}$ of the masked token with $\boldsymbol{k^{'}}$ and use $[\boldsymbol{l_i};\boldsymbol{k^{'}}]$ to predict the original token:
\begin{equation}
\hat{y_i} = softmax(W_f[\boldsymbol{l_i};\boldsymbol{k^{'}}]),
\end{equation}
where $W_f$ is the weight parameter.
At last, the TP objective is to predict the original tokens which are masked out, formulated as follows:
\begin{equation}
    \mathcal{L}_{TP}(\theta) = -log \mathbf{p}(l_i | ls \backslash \{l_i\} ), \label{mlm}
\end{equation}
where $ls \backslash \{l_i\}$ denotes the log tokens sequence $ls$ with token $l_i$ being masked.




\subsubsection{Sentence-Level Semantic Alignment}
Since logs do not conform to the grammatical structure of human language and are always concise, it is difficult to sufficiently capture the semantics of logs. To enrich the semantic context of logs and improve the robustness of log representations, \textcolor{blue}{inspired by KnowLog \cite{ma2024knowlog}, we construct a semantic alignment pre-training task (SA) in the sentence-level} that aligns the semantic representations of logs with the expert knowledge in the semantic space by contrastive learning.

Specifically, we first construct positive and negative examples from a batch $T = \{(l,k)\}$ of input pairs with size $N$. $(l^a,k^a)$ is the $a$-th pair in the batch. We obtain logs $l$ and knowledge $k$ from the same input pairs $\{(l^a,k^b)_{a=b}\}$ as positive examples and different input pairs $\{(l^a,k^b)_{a \neq b}\}$ as negative examples. Then we use $\boldsymbol{l^a}$, $\boldsymbol{k^a}$ to indicate the representations of the log and the knowledge, here the hidden state of the special symbol $[CLS]$ as the sentence representation. To pull closer positive samples and push away negative samples, the training objective of SA is defined as follows:
\begin{equation}
    f(\boldsymbol{l^a,k^b}) = exp(\frac{\boldsymbol{(l^a)}^{\top} \boldsymbol{k^b} }{\lVert \boldsymbol{l^a} \rVert \cdot \lVert \boldsymbol{k^b} \rVert} / \tau ), \label{ct}
\end{equation}

\begin{equation}
    \mathcal{L}_{SA}(\theta)=\frac{1}{N}\sum_{a=1}^N -log\frac{f(\boldsymbol{l^a,k^a})}{f(\boldsymbol{l^a,k^a}) + \sum\nolimits_{b=1}^{N-1} f(\boldsymbol{l^a,k^b})},
\end{equation}
where $\tau$ is the temperature hyper-parameter, which is set to 0.05 empirically in our experiments.

At last, we sum the TP loss and the SA loss, and obtain the overall training objective:
\begin{equation}
\min_{\theta} \mathcal{L}_{TP}(\theta) + \mathcal{L}_{SA}(\theta)
\end{equation}



\subsection{Fine-Tuning with Downstream Tasks}
After pre-training, we fine-tune the log encoder on different downstream tasks. We group all downstream tasks into two categories based on the input type: log-single tasks and log-pair tasks. We use the final hidden state of the first token (the $[CLS]$ token) as the sentence representation. For log-single tasks, we input the output of the language model $l_{CLS}$ into a multi-layer perception network function $f_H$ and obtain the prediction as $f_{H}(l_{CLS})$. For log-pair tasks, we follow sentence-bert \cite{reimers2019sentence} and use the language model to encode two separate sentences $u,v$, then input $u_{CLS},v_{CLS}$ and element-wise difference $|u_{CLS}-v_{CLS}|$ into a multi-layer perception network function $f_{H}$ and obtain the prediction as $f_{H}([u_{CLS};v_{CLS};|u_{CLS}-v_{CLS}|])$. 
